Structured Prediction Cascades

Structured prediction tasks pose a fundamental trade-off between the need for model complexity to increase predictive power and the limited computational resources for inference in the exponentially-sized output spaces such models require. We formulate and develop the Structured Prediction Cascade architecture: a sequence of increasingly complex models that progressively filter the space of possible outputs. The key principle of our approach is that each model in the cascade is optimized to accurately filter and refine the structured output state space of the next model, speeding up both learning and inference in the next layer of the cascade. We learn cascades by optimizing a novel convex loss function that controls the trade-off between the filtering efficiency and the accuracy of the cascade, and provide generalization bounds for both accuracy and efficiency. We also extend our approach to intractable models using tree-decomposition ensembles, and provide algorithms and theory for this setting. We evaluate our approach on several large-scale problems, achieving state-of-the-art performance in handwriting recognition and human pose recognition. We find that structured prediction cascades allow tremendous speedups and the use of previously intractable features and models in both settings.

==> text/aistats/cascades.tex <==
\begin{figure}
  \centering
  \resizebox{1.0\textwidth}{!} {
    \input{figs/pruned_lattice}
  }
\caption{\small Max marginal-based cascade for a CRF based parts model
  as implemented in experiments. {\em Left:} The original dense
  lattice represents all $K$ assignments to all $L$ positions in the
  lattice, with transitions between states representing bigrams. {\em
    Center:} The first pruning function, $r_{\mbf{w}}$, prunes away
  several of the potential assignments to singletons at difference
  positions. {\em Right:} A mapping function $\phi$ maps singletons
  in the sparse unigram lattice (Center) to a sparse set of bigram
  parts in a one-to-many fashion. The set of unpruned edges in this
  final lattice represent a sparse set of unpruned trigrams. This
  process can be repeated to represent quad- or five-grams, if desired.}
  \label{fig:lattice}
\end{figure}

\section{Max-marginal pruning}% cascades for structured outputs}
\label{sec:cascades}

Even given an optimal pruning function, exponentially large
output spaces pose additional difficulties that must be addressed in
order for the pruning function to be of any practical use. First, for
any fixed pruning rate, the output of the pruning
function will be exponential in size if $\mcal{Y}(x)$ is
exponential. Therefore a compact representation must be found to
represent the set of unpruned outputs $r_{\bw}(x, \cY(x))$. Second, we
must be able to efficiently modify our inference procedure to take
advantage of the reduced output space, i.e., to compute
\begin{equation}
  \label{eq:efficient_hyp}
  h_{\mbf{\widetilde{\bw}}}(x) = \argmax_{y\in r_{\bw}(x,\cY(x))} \widetilde{\bw}^\top\mbf{f}(x,y) ,
\end{equation}
for some pruning function $r_{\mbf{w}}(x)$. Finally, as alluded to
earlier, pruning an exponentially large output space by some fixed
proportion will only reduce, but not eliminate, the exponential
complexity of inference. Ideally, our pruning procedure would prune
away an exponentially large portion of the output space of roughly the
same order as the difficulty of the original problem. In this section,
we propose a simple and general pruning procedure that
addresses each of the above difficulties.

%\subsection{Efficient pruning}% with max marginals}
%\label{sec:cascade}

We use a clique-based representation of the feature function to
compactly store an exponential number of unpruned labels. We define
the {\em max marginal} for a clique $c$, an assignment $Y_c = y_c$, and a
parameter vector $\mbf{w}$ as the following,
\begin{equation}
  \label{eq:max_marginal_part}
  s_{\mbf{w}}^\star(x,y_c) \triangleq \max \{\mbf{w}^\top\mbf{f}(x,y')\mid y' \in \cY(x), y'_c = y_c\},
\end{equation}
which is the best possible score for any output $y$ that is consistent
with the assignment $y_c$. Suppose $s_{\mbf{w}}^\star(x,y_c)$ is less
than some desired pruning threshold $\theta$. By definition, the score
of any other output consistent with the assignment $y_c$ cannot be
higher than $s_{\mbf{w}}^\star(x,y_c)$. We can therefore make the
following simple statement: if for any $y \in \mcal{Y}$, there exists
some part $c$ such that $s_{\mbf{w}}^\star(x,y_c) \le \theta$, then
the score $\mbf{w}^\top\mbf{f}(x,y) \le \theta$ as well. Thus, for a
given $\theta$, the following relationship holds:
\begin{equation}
  \label{eq:efficient_pruner}
  r_{\mbf{w}}(x,\cY(x)) \subseteq g_{\mbf{w}}(x,\cY(x)),
    \qquad g_{\mbf{w}}(x,\cY(x)) =  \bigcap_{c \in \mcal{C}}\{y \in \cY(x): s_{\mbf{w}}^\star(x,y_c) > \theta\}.
\end{equation}
That is, we can represent a superset of the output of the pruning function
$r_{\mbf{w}}$, which may be exponential in size, with the max marginal
pruning function $g_{\mbf{w}}$, which is represented locally on cliques.
Note that to efficiently evaluate $g_{\mbf{w}}$, it is only required
to compute and store the max-marginals, which by assumption are
polynomial in the length of the input.
%For a given partial assignment
%$y_c$, we can then query whether any $y$ consistent with $y_c$ is
%pruned by $g_{\mbf{w}}$ in $O(1)$ time.


An illustration of this process for sequences (cliques of size $2$)
appears in Figure~\ref{fig:max_marginals}. The left panel shows three
possible labels, organized in two cliques, both containing the second
vertex. The middle panel shows all possible labelings of this graph,
where each vertex can be labeled as either {\tt a}, {\tt b} or {\tt
  c}. Furthermore, the all the labelings that are consistent with
$y_2=\mathtt{b}$ are marked with bold blue edges. Finally, the right
panel illustrates the maximization operation over all consistent
labelings, which is the value of max-marginal
$s_{\mbf{w}}^\star(x,Y_2=b)$.

\out{
Given an efficient representation for $g_\bw$, we must still find a way
to take advantage of $g_\bw$ when evaluating the next hierarchy of the
cascade. Let $\mcal{C}_t$ be the parts for $\mbf{f}$ used at level $t$
of the cascade hierarchy, and let $\mcal{C}_t(x)$ be the set of max
marginals $\ang{c,\hat{y}_c}$ that are unpruned by $r(x)$ at the
previous level. Since we are using a cascade of models of increasing
complexity, there exists a mapping $\phi_{t}: \mcal{C}_{t} \times
\mathbb{Z}^+ \mapsto \mcal{P}_{t+1} \times \mathbb{Z}^+$ that relates
max marginals in $\mcal{P}_{t}$ to max marginals in $\mcal{P}_{t+1}$,
\begin{equation}
  \label{eq:part_mapping}
  \phi_{t}(p, \hat{y}_p) = \left\{\ang{p',\hat{y}_{p'}} \mid p' \in \mcal{P}_{t+1}, \hat{y}_{p} \subseteq \hat{y}_{p'} \right\}.
\end{equation}
By definition, $\ang{p,\hat{y}_p} \in \mcal{S}_t(x)$ implies that
$\phi(p,\hat{y}_p) \in r(x)$. Therefore, when we compute the maximum
over assignments to some part $p$ during dynamic programming or
message passing at the next level of the cascade, we only need to
consider all assignments $\ang{p,\hat{y}_{p}} \in
\phi(p',\hat{y}_{p'})$ for which $\ang{p',\hat{y}_{p'}} \in
\mcal{S}_t$. If we can evaluate $\phi_{t}$ in constant time, then we
do not pay any amortized overhead for the translation process.
}

Finally, the step of passing the representation of the reduced
assignment space from one level of
the cascade to the next level is illustrated in Figure
\ref{fig:lattice} where we start with all possible labels (left), then
prune vertices using max-marginals (middle), and transfer the labeling graph to a
second order lattice.
%This transformation can be computed efficiently.


%\subsection{Sparse forward-backward inference}

We can incorporate the sparse lattice $\mcal{V}$ into the well-known
forward-backward \cite{rabiner} algorithm for HMM/CRF models with
little difficulty. Let $\mcal{F}_k$ and $\mcal{B}_k$ be the set of
valid forward and backward transitions for the $k$'th state in the
model, respectively. We modify forward-backward as follows:
\begin{packed_enum}
\item At each position $j$, we compute coefficients only over the
  sparse set of valid states $\mcal{V}_j$.
\item For each state $k \in \mcal{V}_j$, we maximize only over the
  intersection $\mcal{F}_K \cap \mcal{V}_{j+1}$ or $\mcal{B}_k \cap
  \mcal{V}_{j-1}$.
\end{packed_enum}
By using a sparse datastructure to store $\mcal{V}$, we can enumerate
all $k \in \mcal{V}_j$ in $O(|\mcal{V}_j|)$ time and enumerate all $k
\in \mcal{F}_k \cap \mcal{V}_{j+1}$ in
$O(\min\{|\mcal{F}_k|,|\mcal{V}_{j+1}|\})$ time. Once the forward and
backward coefficients have been computed, the max marginal
$s_{\mbf{w}}^\star(x,Y_j=k)$ is simply the sum of the forward and
backward coefficients $\delta_j(k) + \beta_j(k)$, respectively.



\begin{algorithm}
  \label{alg:pruning}
  \KwIn{Example $x$, parameter $\alpha$, pruning weights $\mbf{w}^{(d)}$.}
  \KwInit the unpruned lattice: $\forall j, \mcal{V}_j = Y_j$.

  \For{$d = 1$ \KwTo $(D-1)$}{
    \begin{packed_enum}
    \item Run sparse Forward-Backward using $\mbf{w}^{(d)}$ and the
      lattice $\mcal{V}$ to compute $\delta$ and $\beta$.
    \item Compute the pruning threshold $\theta$ from $\delta$, $\beta$, and
      $\mcal{V}$% using Equation \eqref{eq:pruning_forward_backward}.
    \item Remove any vertices corresponding to max marginals
      $\delta_j(k) + \beta_j(k) \le \theta$ from $\mcal{V}_j$.
    \item If $d \ge 1$: Using $\phi$, generate a sparse order-($d+1$) lattice from
      $\mcal{V}$ (e.g., Figure \ref{fig:lattice}).
    \end{packed_enum}
  }
  \KwRet The pruned order-$D$ sparse lattice $\mcal{V}$.

  \caption{Pruning a lattice with the cascade.}
\end{algorithm}

\out{ One simple, general example of a parts-based representation for
  a joint label space $Y = \{Y_1Y_2\dots Y_l\}$ is as follows. At the
  base of the cascade, the cliques consist of the singletons
  $\{Y_1\}$, $\{Y_2\}$, $\dots, \{Y_l|\}$; at each following level $t$
  of the cascade, the parts consist of unique unions of $t$ singleton
  sets. Therefore, we can construct $\phi_t$ as follows: if there are
  $l$ singletons, each part at level $t$ maps to exactly $l-t$ parts
  at level $t+1$. Any max marginal assignment to a part at level $t$
  will therefore have $k(l-t)$ consistent max marginal assignments at
  level $t+1$. In an sequence model such as a CRF or HMM, exactly such
  a parts-based representation is used, with the additional constraint
  that singletons may only be added to a part in sequential order (see
  Figure \ref{fig:lattice}).


To summarize, max marginals allow for a efficient representation of
the unpruned outputs determined by $r_\bw(x)$. Rather than attempting to
store all $y \in r_\bw(x)$, we instead store the set of
max marginals which score greater than the threshold $\theta$. When we
train or evaluate the next level of the cascade, we prune corresponding
parts of the lattice to limit the search space of the dynamic programming
or message passing algorithm of the next stage.
%to only those max marginals consistent with
%$\mcal{S}_t(x)$. If $\phi_t$ requires only constant time to evaluate,
the amortized complexity of this entire procedure is the same as the
original evaluation procedure for some $h(x)$ with the same features.
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nips2009"
%%% End:


==> text/aistats/cascadesB.tex <==
\section{Learning $\mbf{w}$ and $\theta$}
\label{sec:pruning}



\out{
=======
\begin{equation}
  \label{eq:pruning_forward_backward}
  \theta = \alpha \max_{k \in \mcal{V}_L} \delta_L(k) +
  (1-\alpha)\frac{1}{|\mcal{V}|}\sum_{\ang{j,k} \in \mcal{V}}\delta_j(k) + \beta_j(k).
\end{equation}
}

In the pruning learning problem \eqref{eq:pruning_fixederr}, our goal
is to maximize pruning efficiency subject to the constraint that we
maintain a desired level of recall. We have two parameters with which
to optimize our objective: the weights $\mbf{w}$ and the pruning
function $\theta(x,\cY(x))$. The simplest
approach, adopted in~\cite{viola01robustreal},
is to estimate $\bw$ first and then tune $\theta(x,\cY(x))$:
\begin{packed_enum}
\item Optimize $\mbf{w}$ to minimize classification loss.
\item Given $\mbf{w}$, find a pruning threshold function
  $\theta(\mbf{w},x)$ that relaxes the classification problem until a
  given recall $(1-\epsilon)$ is achieved.
\end{packed_enum}

We propose this approach as a baseline and  
%In the interest of using the simplest possible tools to achieve our
%goal, 
use the standard structured perceptron algorithm
~\cite{collins_discriminative_2002} in step 1 to minimize
classification loss. The advantages of the perceptron are that it is
simple and efficient and has shown robust
performance on sequence learning tasks such as those studied in this
paper. However, the standard perceptron training is ignorant of the
goal of pruning and the threshold function, and it does not learn to 
minimize the pruning error in general. In the next section 
%\ref{sec:pruningperceptron}, 
we introduce the
{\em pruning perceptron}, which addresses the goal of pruning more directly.

\subsection{Mean-max pruning loss}
In practice, we have the additional constraint that evaluating the
scores and threshold function must be fast enough that the cumulative
evaluation time at each level of the cascade results in a net gain in
efficiency.  Note that the threshold cannot be defined as an absolute value, but
must depend strongly on $x$ and $\bw$.  We construct our threshold from two ingredients
to anchor our threshold :
the score of the best assignment $s^\star_\bw(x) = \max_{y\in\cY(x)}\bw^\top \bft(x,y)$ and
the mean of the max marginals not pruned by $\cY(x)$, denoted by $\bar s^\star_\bw(x)$.
% = \frac{1}{LK} \sum_{k=1}^K\sum_{n=1}^L s_{\mbf{w}}^\star(x,Y_n=k)$.



%For instance, a threshold function that relies on sorting
%the scores of all max marginals before choosing a threshold (e.g.,
%choosing a fixed proportion or sum-likelihood) will be logarithmically
%less efficient than a threshold function that can be evaluated in
%linear time. As the complexity of the cascade grows exponentially,
%even a sublinear inefficiency will rapidly become intolerable in
%practice.

\begin{figure}
  \centering
  \input{figs/meanmax}
  \caption{\small An illustration of the mean-max pruning threshold
    function. The histogram is the distribution of max marginals. The
    mean-max threshold (solid red line, center) is scaled by $\alpha$
    between the mean and the maximum score (dashed red line,
    right). In this case, the score of the truth lies (green, solid)
    lies in between; the threshold at $\alpha = 0.5$ (dashed line,
    black, center) suffices to prune the majority of max marginals
    while preserving the truth.}
  \label{fig:meanmax}
\end{figure}

We propose the following ``mean-max'' threshold function (Figure
\ref{fig:meanmax}), which sets the pruning threshold between the
max over marginals and the mean for $\alpha \in [0,1]$:
\begin{equation}
  \label{eq:meanmax}
  \theta_{\alpha,\bw}(x,\cY(x)) = (1-\alpha)\bar s^\star_\bw(x) + \alpha s^\star_\bw(x).
\end{equation}
The mean-max threshold is computable in linear time. Furthermore, by
varying $\alpha$ from $0$ to $1$, one can control the trade off
between pruning efficiency and pruning errors: as $\alpha$ approaches
$1$, the $\theta_\alpha$ approaches the argmax, and only the argmax
will survive the threshold. In this case, pruning error is exactly
classification error. On the other hand, when $\alpha = 0$, only max
marginals that are equal to or below the mean max marginal across the
entire sequence will be pruned. If the max marginals are reasonably
distributed, this mean threshold will prune close to $1/2$ of the
max-marginals (in practice, we have observed the $\alpha=0$ threshold
to prune roughly $40\%$). We chose the mean, and not an arbitrary
scaling between argmin and argmax, precisely to provide this
approximate minimum efficiency for the cascade, as well as to ensure
the convexity of our margin constraints below.

\subsection{Pruning perceptron}
\label{sec:pruningperceptron}

It is straightforward to modify the perceptron update to minimize pruning
errors for a given threshold function $\theta_{\alpha,\bw}$ instead of
classification errors. For the $j$'th example, we define a {\em pruning mistake} as a
violation of a threshold constraint:
\begin{equation}
  \label{eq:pruningmistake}
  \mbf{w}^\top\mbf{f}(x^j,y^j) \ge \theta_{\alpha,\mbf{w}}(x^j, \cY(x^j)) + 1.
\end{equation}
Note that each constraint is convex in $\bw$, since it involves maxima over linear constraints.

For each mistake, we use the equivalent perceptron update:
\begin{equation}
  \label{eq:pruningupdate}
  \mbf{w}' \leftarrow \mbf{w} + \lambda \mbf{f}(x^j,y^j) -
  \lambda\left[ (1-\alpha)
  %\left(
      \bar\bft_\bw^\star(x^j)
      %\frac{1}{KL} \sum_{k=1}^K\sum_{n=1}^L \mbf{f}(x,y^\star_{\mbf{w}}(Y_n=k))\right) +
    +\alpha \bft_\bw^\star(x^j)
    %\mbf{f}(x,y^\star_{\mbf{w}}(x)) 
    \right],
\end{equation}
where we have introduced the notation 
$\bft_\bw^\star(x) = \bft(x^j, \argmax_{y\in\cY(x^j)} \bw^\top\bft(x^j,y))$
and similarly 
$\bar \bft_\bw^\star(x^j)$ is the average of the features of the maximizing assignments
for each unpruned max-marginal.

In practice, when we train the pruning perceptron (or the standard
perceptron) as part of the cascade, we use the previously-trained
portion of the cascade to prune the output space during training. This
pruning process is outlined in algorithm \ref{alg:pruning}.
% $y^\star_{\mbf{w}}(x,Y_n=k) = \argmax_{y:y_n=k}
% \mbf{w}^\top\mbf{f}(x,y)$ as the maximizing assigments to the argmax
% and the max marginal for $Y_n=k$, respectively.





% This leads to the following definition of forward coefficients
% $\delta$ and backward coefficients $\beta$. To reduce clutter, we
% shorthand for scores over states and transitions, $s_j(x,k) =
% \mbf{w}^\top\mbf{f}(x,Y_j = k)$ and $s_{j,j'}(x,k,k') =
% \mbf{w}^\top\mbf{f}(x,Y_{jj'}) = kk')$:
% \begin{align}
%   \beta_n(k) & = 0, \qquad \beta_j(k) = \max_{k' \in \mcal{V}_{j+1}
%     \cap \mcal{F}_k} \left[ \beta_{j+1}(k') + s_{j+1}(x,k') +
%     s_{j,j+1}(x, k, k') \right] \\
%   \delta_1(k) & = s_1(x, k) + s_{01}(x, \emptyset, k),
%   \quad \delta_j(k)  = s_j(x,t) + \max_{k' \in \mcal{V}_{j-1} \cap \mcal{B}_k} \left[ \delta_{j-1}(k') + s_{j-1,j}(x,k',k) \right]
% \end{align}

%\subsection{The Pruning Perceptron Cascade}

\begin{algorithm}
  \caption{Pruning Perceptron cascade training.}
  \KwIn{Training set $S$, development set $S_D$, error cap $\epsilon$, depth $D$.}

  \KwInit An empty cascade $C = \{\}$.

  \For{$d = 1$ \KwTo $(D-1)$}{

    \ForEach{$\alpha \in \{0, 0.2, 0.4, 0.6, 0.8\}$}{
        \begin{enumerate}
        \item Train a pruning perceptron $\mbf{w}^{(d)}$ with parameter $\alpha$ as
          described in section \ref{sec:pruningperceptron}.
        \item If the recall of $\mbf{w}^{(d)}$ is less than
          $(1-\epsilon)$, relax $\alpha \rightarrow 0$ until either
          $\alpha = 0$ or the recall reaches the minimum level.
        \end{enumerate}
      }
      \KwUpdate $C_d = \ang{\mbf{w}^{(d)}, \alpha}$
    }
    \KwRet{The cascade $C$.}


  \label{alg:pp}
\end{algorithm}

% One method that has been applied successfully to structured
% classification problems is the perceptron algorithm
% \cite{collins_discriminative_2002}. In the perceptron algorithm, a
% weight vector $\mbf{w}$ is initialized to $0$ and then updated
% incrementally by considering each example $\ang{x^i,y^i} \in S$
% sequentially. If $h_{\mbf{w}}(x) \ne y^i$, then $\mbf{w}$ is updated
% to increase the score of the correct answer and decrease the score of
% the incorrect guess,
% \begin{equation}
%   \label{eq:perceptron_update}
%   \mbf{w}' = \mbf{w} + \lambda\left(\mbf{f}(x^i,y^i) - \mbf{f}(x^i,h_{\mbf{w}}(x^i))\right).
% \end{equation}
% Here, $\lambda$ is a learning rate parameter. In general, the
% algorithm may be improved by decreasing $\lambda$ with each example or
% pass through the training data, thus averaging every $\mbf{w}$ vector
% produced by the algorithm.

% We modify the perceptron algorithm to learn to prune the data. As
% described above, we can encode the pruning function as a binary
% classification task on two examples: $\mbf{f}(x^i,y^i)$ and
% $\bar{\mbf{f}}(x)$. We can therefore use the perceptron algorithm
% exactly as before, but by replacing the classifier's guess
% $\mbf{f}(x^i,h_{\mbf{w}}(x^i))$ with the mean features
% $\bar{\mbf{f}}(x^i)$. This results in the following update,
% \begin{equation}
%   \label{eq:pruning_update}
%   \mbf{w}' = \mbf{w} + \lambda\left(\mbf{f}(x^i,y^i) - \bar{\mbf{f}}(x^i)\right),
% \end{equation}
% which is applied each time $\mbf{w}^\top(\mbf{f}(x^i,y^i) -
% \bar{\mbf{f}}(x^i) \le 1$. The fixed margin of $1$ ensures that we
% choose $\mbf{w}$ to maximize the margin, given on limitations on
% $||\mbf{w}||$ imposed by $\lambda$.

% Aside from training the pruning functions, the most critical issue in
% the pruning cascade is determining how to represent $r(x)$, the set of
% unpruned possible answers according to $r$. If representing $r(x)$
% requires exponential space, then pruning will not provide any
% benefit. We now turn to the task of finding an efficient
% representation for $r(x)$, regardless of how $r(x)$ was trained or
% implemented.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nips2009"
%%% End:


==> text/aistats/conclusion.tex <==
\section{Conclusion}
We presented structured prediction cascades: an efficient, principled
method of tackling the complexity of structured prediction problems.
We proposed and theoretically analyzed a novel loss function that
attempts to balance accuracy and efficiency of the cascade. Using a
simple sub-gradient optimization method, we evaluated our method on
several large-scale datasets. On the handwriting recognition task, we
found that the cascade reduced the state space of a fourth-order
Markov model by five orders of magnitude, allowing the use of higher
order features that tripled the word-level accuracy of predictions. On
the POS task, the cascade increased inference efficiency of trigram
models $100\times$ relative to unfiltered inference without negatively
impacting the accuracy of the final predictor.

While we used sequence models to illustrate the cascades, the methods
described here could be applied to other sets of nested models. For
example, graphical models used for articulated object detection in
vision have a natural coarse-to-fine scale hierarchy. Temporal models
with factored state (e.g., dynamic Bayes nets or factorial CRFs) are
another natural candidate for cascaded learning and inference. Our
approach could also be extended to incorporate intractable models
through the use of approximate inference techniques. Theoretical
analysis of filtering accuracy in the case of approximate inference is
an interesting open question.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cascades_aistats2010"
%%% End:


==> text/aistats/experiment.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluated our approach on three Part of Speech (POS) tagging tasks: English,
Portuguese and Bulgarian.
%To increase the
%difficulty of the problems, we significantly reduced the amount of
%training data available to the learner.
For English, we used volumes
0-4 of the Penn TreeBank~\cite{PennTreebank} Wall Street Journal
corpus for training, volume 18 for development, and volumes 21-24 for
testing. We used the Bulgarian BulTreeBank~\cite{Simov02buildinga} and
the Bosque subset of the Portuguese Floresta
Sinta(c)tica~\cite{floresta}\footnote{http://www.linguateca.pt/Floresta/}
for Bulgarian and Portuguese datasets, respectively. We used a random
40\% sample of the training sets provided with each corpus, divided
again 80-20 into training set and development set, as the input to the
pruning cascades. Finally, to explore a different problem space, we
also evaluated our approach on a modified speech recognition problem
from the TIMIT dataset~\cite{lamel1989sdd} by computing phoneme-level features on frames
already pre-segmented into distinct phonemes. We use 50\% of the TIMIT
training corpus and 20\% of the TIMIT development set for training of
this model.

For each dataset, we trained a standard structured perceptron on an
unpruned trigram model to establish baseline running time and
accuracy. To assess the differences between pruning perceptron
(PP$\alpha$) and structured perceptron (SP) outside of a cascade, we
evaluated both methods for unigram (flat) and bigram models in
isolation. We then evaluated depth-3
(unigram$\rightarrow$bigram$\rightarrow$ trigram) cascades trained
with different minimal recall thresholds $1-\epsilon$. For each
pruning error cap $\epsilon$, we ran two pruning cascades: first,
using the structured perceptron only; second, we applied the pruning
perceptron cascade (Algorithm \ref{alg:pp}) % was ppcascade 
and used a standard
structured perceptron trigram model for the final output.

\subsubsection*{Parameters}

For each level of the cascade, each perceptron (PP$\alpha$ and SP) was
trained for 30 epochs with learning rate $\lambda = 1$. Weight updates
were averaged for voted perceptron, and the epoch with lowest
development set error (classification error for SP, pruning error for
PP$\alpha$) was used as the final classifier after training.

\subsection{Results}
\label{sec:results}

 \begin{figure}
   \centering
   \includegraphics[width=0.33\textwidth,clip=true,trim=0.3in 0.5in 0.5in 0.5in]
   {figs/ptb_small0_alphas}
   \includegraphics[width=0.33\textwidth,clip=true,trim=0.3in 0.5in 0.5in 0.5in]
   {figs/ptb1_alphas}
   \caption{\small Comparison recall-efficiency trade-offs for pruning
     perceptron and structured perceptron on the WSJ dataset (Left:
     flat model, Right: bigram model.) Curves were generated by
     computing the pruning error and pruning efficiency (proportion of
     pruned max marginals) for all possible $\alpha$ relaxations
     available to each method. E.g., PP$\alpha$ trained with $\alpha =
     0.6$ was evaluated for $\alpha \in [0,0.6]$, while PP$\alpha$
     trained with $\alpha = 0$ results in a single point. The
     $\epsilon = 0.05\%$ pruning error cap is marked with a horizontal
     dashed line; intercepts with this line are the efficiencies of
     each method given an error cap of $0.05\%$.}
   \label{fig:pos_eff}
\end{figure}

 \paragraph{Structured vs. pruning perceptron.} On all three POS
 applications, the pruning perceptron had significantly lower pruning
 error than the structured perceptron, and subsequently was able to
 choose larger $\alpha$ and prune more efficiently. For the WSJ
 dataset, the trade-off between pruning error and efficiency is
 visualized in figure \ref{fig:pos_eff}. In many cases, the structured
 perceptron is unable to achieve a pruning error of $\epsilon =
 0.05\%$ for any $\alpha \in [0,1]$; and it is consistently dominated
 in each dataset by the pruning perceptron algorithms.

 \paragraph{Efficiency of structured pruning cascade.} A summary of
 the efficiency of the pruning cascades on each dataset for different
 error caps is in table \ref{tab:bigsummary}. The accuracy is computed
 relative to baseline (Acc). The increase in efficiency is especially
 dramatic for the WSJ dataset due to the large tagset ($K=45$): for
 this data, the PP$\alpha$ cascade resulted in a 27X speedup with
 $0.3\%$ decrease in accuracy $(\epsilon=0.05)$, and a 90X speeded up
 with a $3\%$ decrease in accuracy $(\epsilon=0.1)$. In each dataset,
 the pruning perceptron dominates the standard perceptron cascade in
 terms of efficiency. Finally, since the cascade training proces
 incorporates pruning during training, we also observed a radical
 decrease in training time for all datasets. In the WSJ dataset,
 training time was reduced from over 21 hours to only 31 minutes
 (PP$\alpha$, $\epsilon = 0.1$), a 41-fold reduction, with $3\%$
 decrease in accuracy. With no decrease in accuracy, training time was
 reduced to 1 hour and 16 minutes (PP$\alpha$,$\epsilon=0.05$), a
 16-fold reduction.

We also computed several interesting theoretical metrics for each
cascade. For example, to compare the size of the pruned search space
without taking into account implementation overhead, we computed the
average number of valid states at a given position in the lattice
($|\mcal{V}_j|$) and the average number of valid transitions to be
scored ($|\mcal{F}_k \cap \mcal{V}_j|$). Multiplying these gives the
average number of scoring operations per position, and summing up all
scoring operations in the entire cascade, we can compare the
theoretical efficiency of the Viterbi algorithm (Vit) against the
naive baseline or an approximate inference method such as beam
search. Thus, for the WSJ data the pruning cascade needed 628X fewer
scoring operations than baseline, which we can also compute is roughly
equivalent to the number of scoring operations required if a beam
search was used with only 3 beams ($\approx$Beam).

\begin{table}
  \caption{Cascade efficiency on three Part of Speech (POS) Tagging datasets.}
  \centering
%  \resizebox{1.0\textwidth}{!}{
  \begin{tabular}{ccccccccccc}
    \hline
    & \multicolumn{2}{c}{Pruning $\epsilon$} & & \multicolumn{2}{c}{Efficiency} & & & \multicolumn{3}{c}{Lattice sparsity} \\
    Alg. & Cap & Test & Acc. & ms. & Vit. & $\alpha_0$ & $\alpha_1$ & $\approx$Beam& $|\mcal{V}_j|$ & $|\mcal{F}_k \cap \mcal{V}_{j+1}|$ \\ \hline
    \multicolumn{11}{l}{\em Wall Street Journal (K=45)}\\
    SP & 0.05 &  0.188 & 1.016 &  3.72 & 9.5 & 0.00 & 0.20 & 213.1 & 449.7 & 20.3 \\
    SP & 0.10 & 0.228 & 1.016 &  4.01 & 9.5 & 0.00 & 0.28 & 213.1 & 449.7 & 20.3 \\
    PP$\alpha$ & 0.05 & 0.163 & 1.003 & \bf 27.34 & 109.6 & 0.35& 0.65 & 18.5 & 84.6 & 8.8 \\
    PP$\alpha$ & 0.10 & 0.282 & 1.030 & \bf 89.27 & 628.7 & 0.69& 0.59 & 3.2 & 24.9 & 4.8 \\
    \hline
    \multicolumn{11}{l}{\em Portuguese TreeBank (K=22)}\\
    SP & 0.05 & 0.392 & 0.957 & 5.39 & 19.1 & 0.00 & 0.00 & 27.7 & 70.4 & 8.0 \\
    SP & 0.10 & 0.409 & 0.957 & 5.17 &  19.1 & 0.00 & 0.05 & 27.7 & 70.4 & 8.0 \\
%    SP & 0.20 & 0.529 & 0.957 & 5.34 &  19.1 & 0.00 & 0.24 & 27.7 & 70.4 & 8.0 \\
%    SP & 0.40 & 0.819 & 0.984 & 10.56 & 50.3 & 0.04 & 0.29 & 10.5 & 35.6 & 5.8 \\
    PP$\alpha$ & 0.05 & 0.051 & 0.925 & \bf 5.96 & 21.9 & 0.20& 0.37 & 24.1 & 63.9 & 7.7 \\
    PP$\alpha$ & 0.10 & 0.171 & 0.938 & \bf 11.00 & 64.2 & 0.46& 0.40 & 8.2 & 29.8 & 5.3 \\
 %   PP$\alpha$ & 0.20 & 0.495 & 0.981 & \bf 21.12 & 147.7 & 0.60& 0.38 & 3.6 & 16.6 & 4.0 \\
  %  PP$\alpha$ & 0.40 & 0.938 & 1.000 & \bf 33.23 & 264.6 & 0.75& 0.64 & 2.0 & 10.8 & 3.2 \\ \\
    \hline
    \multicolumn{11}{l}{\em Bulgarian TreeBank (K=12)}\\
    SP & 0.05 & 0.503 & 1.009 & 2.27 & 20.5 & 0.00 & 0.00 & 8.3 & 20.3 & 4.3 \\
    SP & 0.10 & 0.562 & 1.009 & 2.61 & 20.5 & 0.00 & 0.09 & 8.3 & 20.3 & 4.3 \\
    PP$\alpha$ & 0.05 & 0.216 & 0.980 & \bf 2.82 & 11.5 & 0.24& 0.37 & 14.6 & 30.3 & 5.3 \\
    PP$\alpha$ & 0.10 & 0.459 & 0.991 & \bf 4.07 & 30.8 & 0.44& 0.40 & 5.5 & 15.0 & 3.8 \\
    \hline
    \multicolumn{11}{l}{\em TIMIT Pre-Segmented (K=49)}\\
     SP & 0.50 & 0.458 & 0.989 & 4.13 & 6.1 & 0.00 & 0.09 & 393.7 & 715.1 & 26.0 \\
     PP$\alpha$ & 0.50 & 0.542 & 0.995 & \bf 6.34 & 9.5 & 0.28& 0.12 & 252.6 & 526.5 & 22.5 \\
     SP & 4.00 & 7.669 & 0.998 & 219.03 & 632.1 & 0.53 & 0.04 & 3.8 & 29.4 & 5.3 \\
     PP$\alpha$ & 4.00 & 7.502 & 1.010 & 122.90 & 304.6 & 0.79& 0.26 & 7.9 & 50.0 & 6.7 

  \end{tabular}
  \label{tab:bigsummary}
\end{table}


% \begin{table}
%   \centering
%   \begin{tabular}{ccccccccccc}
% Method & $\epsilon_t$ & $\hat{\epsilon}$ & Acc. & Eff. (ms) & Eff. (V) & $\alpha_0$ & $\alpha_1$ & Equiv. Beam& $|\mcal{V}_j|$ & $|\mcal{F}_k \cap \mcal{V}_{j+1}|$\\ \hline

% SP & 1.00 & 1.167 & 0.985 & 17.91 & 31.4 & 0.17 & 0.07 & 76.4 & 234.5 & 15.0 \\
% SP & 2.00 & 3.473 & 0.986 & 67.46 & 140.3 & 0.36 & 0.04 & 17.1 & 84.1 & 9.0 \\

% PP$\alpha$ & 1.00 & 1.403 & 0.993 & 12.76 & 27.7 & 0.47& 0.15 & 86.7 & 254.4 & 15.7 \\
% PP$\alpha$ & 2.00 & 3.668 & 1.000 & 43.29 & 83.3 & 0.68& 0.19 & 28.8 & 121.3 & 10.6
% \end{tabular}
%   \caption{Presegmented TIMIT.}
%   \label{tab:bigsummary}
% \end{table}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "cascades_aistats2010"
%%% End: 


==> text/aistats/intro.tex <==
\section{Introduction}

The trade-off between approximation and estimation error is
fundamental in learning complex prediction models.  In structured
prediction tasks, such as part-of-speech tagging, machine translation and gene prediction, the factor of computation time also plays an important role as models with increasing complexity of inference are
considered. For example, a first order conditional random field
(CRF)~\citep{lafferty01crfs} is fast to evaluate but may not be an
accurate model for phoneme recognition, while a fifth order model is
more accurate, but prohibitively expensive for both learning and  prediction. (Model complexity can also lead to overfitting problems due the sparseness of the training data. We do not specifically address this problem in our paper other than judiciously regularizing model parameters.)

In practice, model complexity is limited by computational constraints at prediction time, either explicitly by the user or implicitly
because of the limits of available computation power. We therefore
need to balance expected error with inference time. A common solution
is to use heuristic pruning techniques or approximate search methods
in order to make higher order models feasible.  While it is natural
and commonplace to prune graphical model state space, the problem of
explicitly learning to control the error/computation tradeoff has not
been addressed. In this paper, we formulate the problem of learning a cascade of models of increasing complexity that progressively filter a given structured output space, minimizing overall error and
computational effort at prediction time according to a desired
tradeoff. The contributions of this paper are:
\vspace{-5mm}
\begin{packed_itemize}
\item A novel convex loss function specifically geared for learning to filter accurately and effectively.
\item A simple online algorithm for minimizing this loss using standard inference methods.
\item Theoretical analysis of generalization of the cascade (in terms of both accuracy and efficiency).
\item Evaluation on two large-scale applications:
  handwriting recognition and part-of-speech tagging.
\end{packed_itemize}
% Our inspiration comes from the cascade classifier model of Viola and
% Jones~\cite{viola01robustreal}, widely used for real-time detection of
% faces in images. In their work~\cite{viola01robustreal}, a window is
% scanned over an image in search for face detections and a cascade of
% very simple binary classifiers is trained to weed out easy and
% frequent negative examples early on.  In the same spirit, we propose
% to learn a cascade of structured models of increasing order that weed
% out easy incorrect assignments early on (Section
% \ref{sec:classification}).  The first key question we address is how
% to efficiently represent and update an exponentially-sized set of
% assignments as it is progressively pruned by the cascade (Section
% \ref{sec:cascades}). The second question is how to learn the
% individual models in the cascade to maximize overall efficiency
% (Section \ref{sec:pruning}). We define a novel loss function that
% balances error and computation and propose an efficient phased online
% algorithm for optimizing (a relaxed version of) the combined loss. We
% evaluate our techniques on three NLP applications: English, Portuguese
% and Bulgarian POS, and one speech-recognition task built on a
% modification of the TIMIT dataset (Section \ref{sec:experiments}).
% The results show that our algorithm is up to $90$ times faster than an
% unpruned baseline, reducing the size of the output space
% several-hundred fold with no decrease in accuracy (Section
% \ref{sec:results}).



% Finally, we then discuss the potential of
% this approach to be further improved and applied to more intractable
% domains (Section \ref{sec:discussion}).

\section{Related Work}

Heuristic methods for pruning the search space of outputs have been exploited in many natural language processing and computer vision tasks.  For part-of-speech tagging, perhaps the simplest method is
to limit the possible tags for each word to those only seen as its
labels in the training data. For example, the MXPOST tagger \citep{ratnaparkhi1996maximum} and many others use this technique.  In our experiments, we compare to this simple trick and show that our method is much more accurate and effective in reducing the output space. In parsing, the several works \citep{charniak2000maximum,carreras2008tag,petrov:PhD} use a ``coarse-to-fine'' idea closely related to ours: the marginals of a simple context free grammar or dependency model are used to prune the parse chart for a more complex grammar.  We also compare to this idea in our experiments.  The key difference with our work is that we explicitly learn a sequence of models tuned specifically to filter the space accurately and effectively.  Unlike the work of ~\cite{petrov:PhD}, however, we do not learn the structure of the hierarchy of models but assume it is given by the designer.

\out{Several recent works have considered the trade-off between error and
computation at \textit{estimation} time in large-scale classification
using stochastic/online methods,
notably~\citep{shalevshwartz2008soi,bottou-bousquet-2008}.  The issue
of controlling computation at \textit{prediction} time as well as
estimation time comes up in kernelized classifiers, where prediction
speed depends on the number of ``support vectors''.  Several
algorithms~\citep{Crammer03onlineclassification,dekel2008forgetron,cavallanti2007tbh},
including the Forgetron and Randomized Budget Perceptron are designed
to maintain a limited active set of support vectors in an online
fashion while minimizing error.}

It is important to distinguish the approach proposed here, in which we use {\em exact} inference in a {\em reduced} output space, with other
{\em approximate} inference techniques that operate in the full output space (e.g., \cite{druck_learning_2007}, \cite{pal_sparse_2006}). Because our approach is orthogonal to such approximate inference techniques, it is likely that the structured pruning cascades we propose could be combined with existing methods to perform approximate inference in a reduced output space.

Our inspiration comes partly from the cascade classifier model of~\cite{viola2002robust}, widely used for real-time detection of
faces in images. In their work, a window is
scanned over an image in search of faces and a cascade of
very simple binary classifiers is trained to weed out easy and
frequent negative examples early on.  In the same spirit, we propose
to learn a cascade of structured models of increasing order that weed
out easy incorrect assignments early on.

%\subsection{Structured Classification}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cascades_aistats2010"
%%% End:


==> text/aistats/learning.tex <==
\begin{figure}
  \centering
  \input{figs/exp_factors}
  \caption{\small An example of a series of CRF models of exponentially
    increasing complexity. Inference in the models requires searching
    over unique assignments to each factor (blue square). As the order
    of the model grows, the number of unique assignments grows
    exponentially. The goal of the pruning cascade is to reduce the
    exponential growth by pruning away a large portion of possible
    assignments with each increase in complexity of the model.}
\end{figure}

\iffalse
\begin{figure}
  \centering
  \resizebox{0.35\textheight}{!} {
    \input{figs/exp_factors}
  }
  \caption{\small An example of a series of sequence models of
    increasing complexity. Inference in the models requires searching
    over unique assignments to each factor (blue square). As the order
    of the model grows, the number of unique assignments grows
    exponentially with model order. The goal of the pruning cascade is to reduce the
    exponential growth by pruning away a large portion of possible
    assignments with each increase in complexity of the model.}
\end{figure}
\fi
\section{Structured Prediction}
\label{sec:classification}

Given an input space $\cX$, output space $\cY$, and a training set $S
= \{\ang{x^1,y^1},\dots,\ang{x^m,y^m}\}$ of $m$ independent and
identically-distributed ({i.i.d.}) random samples from a joint
distribution $D$, the standard prediction task is to learn a
hypothesis $h: \cX \mapsto \cY$ that minimizes the expected loss
$\E{D}{ \ell\left(h(x) , y\right)}$ for some non-negative function
$\ell : \cY \times \cY \rightarrow \reals^+$.

We consider the case of structured classification where $\cY = \cY_1
\times \dots \times \cY_L$.
% and $\cY_i \subseteq\{1, \dots, k\}$.
The linear hypothesis class we consider is of the form:
\begin{equation}
  \label{eq:linear_classifiers}
  h_{\bw}(x) = \argmax_{y\in\cY} \bw^\top\bft(x,y)
\end{equation}
where $\bw \in \mathbb{R}^d$ is a vector of parameters and $\bft:
\cX\times\cY\mapsto\mathbb{R}^d$ is a function mapping $(x,y)$ pairs
to a set of $d$ real-valued features. By choosing $\bft$ to depend on
subsets of $x$ and $y$, this hypothesis class can represent arbitrary
interactions between the components of $x$ and $y$.  In general,
evaluating $h_{\mbf{w}}(x)$ is not always tractable, and limits the
expressiveness of the features that can be used.  For a given $y \in
\cY$, we denote the components of $y$ as $y_1, \dots, y_L$, where $y_j
\in \{1,\dots,K\}$. In this case, $|\mcal{Y}|$ is bounded by $K^L$,
which grows exponentially with $L$. Typically, $\mbf{f}(x,y)$ can be
decomposed into separate feature functions on the set of cliques $C$
of $x$ and $y$,
\begin{equation}
  \label{eq:feature_sep}
  \mbf{w}^\top\mbf{f}(x,y) = \sum_{c \in C} \mbf{w}^\top\mbf{f}_c(x_c,y_c), \qquad x_c \subseteq x, \quad y_c \subseteq y.
\end{equation}
%We have deliberately left the definition of the set of ``parts,''
%$\mcal{P}(x,y)$, vague. For each application or problem,
%$\mcal{P}(x,y)$ represents the subsets of $x$ and $y$ that directly
%interact with one another.
For instance, in a log-linear pairwise
Markov network on a graph $G$, the cliques consist of sets of individual
vertices or pairs of vertices connected by an edge in $G$.
%\cite{Taskar:1210}.
By limiting the graph to a sequence (or a tree), it is then
possible to use dynamic programming or message passing
%other linear decoding algorithm on the associated graph
to evaluate Eq.~\eqref{eq:linear_classifiers} in linear time in $L$.
As we include higher order interactions between variables in $y$
inference becomes impractical. For example, the inference of a Markov
models of order $q$ is $O(K^{q+1}L)$ which is infeasible even moderate
values of $K$.
%\cite{Taskar:1210,druck_learning_2007}.
Several structured prediction methods have been proposed
for learning $h_\bw$, such as conditional random fields~\cite{lafferty01crfs},
structured perceptron~\cite{collins_discriminative_2002},
hidden Markov support vector machines~\cite{altun03hmsvm} and
max-margin Markov networks~\cite{taskar03max}, to name a few.  Our focus here is on learning a cascade of increasingly higher order models that can balance
error and computation for large values of $K$ and $q$.

% In practice, however, polynomial time does not necessarily translate
% into feasibility for large scale problems. For example, one of the
% nsimplest sequential models is the Hidden Markov Model (HMM), in which
% $x$ is a sequence of observations and $y$ a sequence of hidden
% states. We model a HMM using \eqref{eq:feature_sep} by defining the
% parts to be sets of $\{y_j,x_j\}$ (observations) and $\{y_{j-1},y_j\}$
% (state transitions). We can then evaluate
% \eqref{eq:linear_classifiers} in a order-$d$ HMM using the standard
% forward-backward Viterbi algorithm with complexity
% $O(k^{(d+1)}n)$. Although this complexity is polynomial in $k$ and
% $l$, the ``hidden'' exponential growth in $d$--even for this simple
% model--limits most large-scale applications to tri-gram HMMs ($d = 2$)
% or to approximate inference algorithms instead
% \cite{druck_learning_2007}. For certain applications, such as complex
% computer vision models, speech recognition, or natural language
% processing, the exponential cost of searching for complex interactions
% is prohibitively expensive.

\subsection{Learning to prune}
Consider building a cascade of models of increasing complexity that given an input $x$, progressively prunes the output space $\cY$ to reduce the cost of inference in the consequent models.  For each stage $i$ of the cascade, our goal is to learn a {\em pruning function} $r_i$, which takes as input $x$ and its current state-space $\cY^i(x)$ and produces a reduced state space $\cY^{i+1}(x) \subset \cY^i(x)$, that is, $r_i: \cX \times \mbf{2}^\cY \mapsto \mbf{2}^\cY$.
%Let $\cZ = \mbf{2}^\cY$ be the set of subsets of the output space.

We would like $r_i$ to eliminate as large a portion of the output space as possible without eliminating the correct answer.  We can formulate this goal as
 \begin{equation}
   \label{eq:pruning_fixederr}
   \min_{r_i} \E{D}{|r_i(x,\cY^i(x))|} \quad \textrm{s.t.} \;\;
   \E{D}{\mbf{1}(y\notin r_i(x,\cY^i(x))} \le \epsilon.
 \end{equation}
%This approach more closely mirrors the practical motivation behind
%pruning in the first place.
%In practice, given some approximation, we
Above, we accept a recall hit in order to make the pruning
function algorithm as efficient as
possible (e.g., $\epsilon$ no more than $1\%$).   Given direct
access to $D$, the optimal $r_i(x,\cY(x)$ would sort $\cY(x)$
by $P(y\mid x)$ and pick the top assignments to fulfill the
recall requirement of $1-\epsilon$.  Clearly, we do not have
access to $D$, but would like to
estimate $r_i$ from the sample data $S$.

\subsection{Linear pruning functions}
%In practice, of course, $P(Y|X)$ is never known to the learning
%algorithm, and we can instead only approximate it with training
%samples. Furthermore, we must
We restrict the class of pruning functions that we consider to a simple
and tractable set:
%. In this paper we therefore
%consider the problem of learning
linear pruning functions of similar
form to linear hypotheses for structured classification. These
functions use a weight vector $\mbf{w}$ to reject any output $y$ that
scores less than a given threshold, $\theta_{\bw}(x, \cY(x))$, which depends
on the input $x$ we will specify below:
\begin{equation}
  \label{eq:lin_pruning_func}
  r_{\mbf{w}}(x,\cY(x)) = \left\{y \in \cY(x): \mbf{w}^\top\mbf{f}(x,y) > \theta(x, \cY(x))\right\}.
\end{equation}
The pruning learning problem \eqref{eq:pruning_fixederr} is then an
estimation problem for two parameters: the weight vector $\mbf{w}$ and
the threshold function $\theta$. However, since the set $\cY(x)$ is
exponentially sized, we first need to consider compact representations
of $r_{\mbf{w}}(x, \cY(x))$.

% We can then express the learning problem \eqref{eq:pruning_fixederr}
% in terms of minimizing the empirical {\em pruning inefficiency} (the
% number of unpruned outputs) on a training set, subject to a constraint
% on the {\em pruning error} (the rate at which the correct answer is
% incorrectly pruned).

\begin{figure}
  \centering
 \resizebox{1.0\textwidth}{!} {
    \input{figs/max_marginals}
  }
  \caption{\small An illustration of the computation of max marginals
    for a (left) length $3$ sequence and
    $\cY=\{\mathtt{a},\mathtt{b},\mathtt{c}\}^3$ (middle) where the
    label of the second vertex is fixed to $b$. This involves
    computing the maximum over all 9 unique paths passing through $Y_2
    = b$; if the vertex $Y_2 = b$ can be pruned, all 9 paths must
    score lower than $s_{\mbf{w}}^\star(x,Y_2=b)$ and can be safely
    pruned as well.}
\label{fig:max_marginals}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cascades_aistats2010"
%%% End:


==> text/aistats/sec_casades.tex <==

\begin{figure}
  \centering
  \resizebox{1.0\textwidth}{!} {
    \input{figs/pruned_lattice}
  }
\caption{\small Max marginal-based cascade for a CRF based parts model
  as implemented in experiments. {\em Left:} The original dense
  lattice represents all $K$ assignments to all $L$ positions in the
  lattice, with transitions between states representing bigrams. {\em
    Center:} The first pruning function, $r_{\mbf{w}}$, prunes away
  several of the potential assignments to singletons at difference
  positions. {\em Right:} A mapping function $\phi$ maps singletons
  in the sparse unigram lattice (Center) to a sparse set of bigram
  parts in a one-to-many fashion. The set of unpruned edges in this
  final lattice represent a sparse set of unpruned trigrams. This
  process can be repeated to represent quad- or five-grams, if desired.}
  \label{fig:lattice}
\end{figure}

\section{Structured Prediction Cascades}
\label{sec:cascades}

Even given an optimal pruning function, exponentially large
output spaces pose additional difficulties that must be addressed in
order for the pruning function to be of any practical use. First, for
any fixed pruning rate, the output of the pruning
function will be exponential in size if $\mcal{Y}(x)$ is
exponential. Therefore a compact representation must be found to
represent the set of unpruned outputs $r_{\bw}(x, \cY(x))$. Second, we
must be able to efficiently modify our inference procedure to take
advantage of the reduced output space, i.e., to compute
\begin{equation}
  \label{eq:efficient_hyp}
  h_{\mbf{\widetilde{\bw}}}(x) = \argmax_{y\in r_{\bw}(x,\cY(x))} \widetilde{\bw}^\top\mbf{f}(x,y) ,
\end{equation}
for some pruning function $r_{\mbf{w}}(x)$. Finally, as alluded to
earlier, pruning an exponentially large output space by some fixed
proportion will only reduce, but not eliminate, the exponential
complexity of inference. Ideally, our pruning procedure would prune
away an exponentially large portion of the output space of roughly the
same order as the difficulty of the original problem. In this section,
we propose a simple and general pruning procedure that
addresses each of the above difficulties.

%\subsection{Efficient pruning}% with max marginals}
%\label{sec:cascade}

We use a clique-based representation of the feature function to
compactly store an exponential number of unpruned labels. We define
the {\em max marginal} for a clique $c$, an assignment $Y_c = y_c$, and a
parameter vector $\mbf{w}$ as the following,
\begin{equation}
  \label{eq:max_marginal_part}
  s_{\mbf{w}}^\star(x,y_c) \triangleq \max \{\mbf{w}^\top\mbf{f}(x,y')\mid y' \in \cY(x), y'_c = y_c\},
\end{equation}
which is the best possible score for any output $y$ that is consistent
with the assignment $y_c$. Suppose $s_{\mbf{w}}^\star(x,y_c)$ is less
than some desired pruning threshold $\theta$. By definition, the score
of any other output consistent with the assignment $y_c$ cannot be
higher than $s_{\mbf{w}}^\star(x,y_c)$. We can therefore make the
following simple statement: if for any $y \in \mcal{Y}$, there exists
some part $c$ such that $s_{\mbf{w}}^\star(x,y_c) \le \theta$, then
the score $\mbf{w}^\top\mbf{f}(x,y) \le \theta$ as well. Thus, for a
given $\theta$, the following relationship holds:
\begin{equation}
  \label{eq:efficient_pruner}
  r_{\mbf{w}}(x,\cY(x)) \subseteq g_{\mbf{w}}(x,\cY(x)),
    \qquad g_{\mbf{w}}(x,\cY(x)) =  \bigcap_{c \in \mcal{C}}\{y \in \cY(x): s_{\mbf{w}}^\star(x,y_c) > \theta\}.
\end{equation}
That is, we can represent a superset of the output of the pruning function
$r_{\mbf{w}}$, which may be exponential in size, with the max marginal
pruning function $g_{\mbf{w}}$, which is represented locally on cliques.
Note that to efficiently evaluate $g_{\mbf{w}}$, it is only required
to compute and store the max-marginals, which by assumption are
polynomial in the length of the input.
%For a given partial assignment
%$y_c$, we can then query whether any $y$ consistent with $y_c$ is
%pruned by $g_{\mbf{w}}$ in $O(1)$ time.


An illustration of this process for sequences (cliques of size $2$)
appears in Figure~\ref{fig:max_marginals}. The left panel shows three
possible labels, organized in two cliques, both containing the second
vertex. The middle panel shows all possible labelings of this graph,
where each vertex can be labeled as either {\tt a}, {\tt b} or {\tt
  c}. Furthermore, the all the labelings that are consistent with
$y_2=\mathtt{b}$ are marked with bold blue edges. Finally, the right
panel illustrates the maximization operation over all consistent
labelings, which is the value of max-marginal
$s_{\mbf{w}}^\star(x,Y_2=b)$.

\out{
Given an efficient representation for $g_\bw$, we must still find a way
to take advantage of $g_\bw$ when evaluating the next hierarchy of the
cascade. Let $\mcal{C}_t$ be the parts for $\mbf{f}$ used at level $t$
of the cascade hierarchy, and let $\mcal{C}_t(x)$ be the set of max
marginals $\ang{c,\hat{y}_c}$ that are unpruned by $r(x)$ at the
previous level. Since we are using a cascade of models of increasing
complexity, there exists a mapping $\phi_{t}: \mcal{C}_{t} \times
\mathbb{Z}^+ \mapsto \mcal{P}_{t+1} \times \mathbb{Z}^+$ that relates
max marginals in $\mcal{P}_{t}$ to max marginals in $\mcal{P}_{t+1}$,
\begin{equation}
  \label{eq:part_mapping}
  \phi_{t}(p, \hat{y}_p) = \left\{\ang{p',\hat{y}_{p'}} \mid p' \in \mcal{P}_{t+1}, \hat{y}_{p} \subseteq \hat{y}_{p'} \right\}.
\end{equation}
By definition, $\ang{p,\hat{y}_p} \in \mcal{S}_t(x)$ implies that
$\phi(p,\hat{y}_p) \in r(x)$. Therefore, when we compute the maximum
over assignments to some part $p$ during dynamic programming or
message passing at the next level of the cascade, we only need to
consider all assignments $\ang{p,\hat{y}_{p}} \in
\phi(p',\hat{y}_{p'})$ for which $\ang{p',\hat{y}_{p'}} \in
\mcal{S}_t$. If we can evaluate $\phi_{t}$ in constant time, then we
do not pay any amortized overhead for the translation process.
}

Finally, the step of passing the representation of the reduced
assignment space from one level of
the cascade to the next level is illustrated in Figure
\ref{fig:lattice} where we start with all possible labels (left), then
prune vertices using max-marginals (middle), and transfer the labeling graph to a
second order lattice.
%This transformation can be computed efficiently.


%\subsection{Sparse forward-backward inference}

We can incorporate the sparse lattice $\mcal{V}$ into the well-known
forward-backward \cite{rabiner} algorithm for HMM/CRF models with
little difficulty. Let $\mcal{F}_k$ and $\mcal{B}_k$ be the set of
valid forward and backward transitions for the $k$'th state in the
model, respectively. We modify forward-backward as follows:
\begin{packed_enum}
\item At each position $j$, we compute coefficients only over the
  sparse set of valid states $\mcal{V}_j$.
\item For each state $k \in \mcal{V}_j$, we maximize only over the
  intersection $\mcal{F}_K \cap \mcal{V}_{j+1}$ or $\mcal{B}_k \cap
  \mcal{V}_{j-1}$.
\end{packed_enum}
By using a sparse datastructure to store $\mcal{V}$, we can enumerate
all $k \in \mcal{V}_j$ in $O(|\mcal{V}_j|)$ time and enumerate all $k
\in \mcal{F}_k \cap \mcal{V}_{j+1}$ in
$O(\min\{|\mcal{F}_k|,|\mcal{V}_{j+1}|\})$ time. Once the forward and
backward coefficients have been computed, the max marginal
$s_{\mbf{w}}^\star(x,Y_j=k)$ is simply the sum of the forward and
backward coefficients $\delta_j(k) + \beta_j(k)$, respectively.


\begin{algorithm}
  \label{alg:pruning}
  \KwIn{Example $x$, parameter $\alpha$, pruning weights $\mbf{w}^{(d)}$.}
  \KwInit the unpruned lattice: $\forall j, \mcal{V}_j = Y_j$.

  \For{$d = 1$ \KwTo $(D-1)$}{
    \begin{packed_enum}
    \item Run sparse Forward-Backward using $\mbf{w}^{(d)}$ and the
      lattice $\mcal{V}$ to compute $\delta$ and $\beta$.
    \item Compute the pruning threshold $\theta$ from $\delta$, $\beta$, and
      $\mcal{V}$% using Equation \eqref{eq:pruning_forward_backward}.
    \item Remove any vertices corresponding to max marginals
      $\delta_j(k) + \beta_j(k) \le \theta$ from $\mcal{V}_j$.
    \item If $d \ge 1$: Using $\phi$, generate a sparse order-($d+1$) lattice from
      $\mcal{V}$ (e.g., Figure \ref{fig:lattice}).
    \end{packed_enum}
  }
  \KwRet The pruned order-$D$ sparse lattice $\mcal{V}$.

  \caption{Pruning a lattice with the cascade.}
\end{algorithm}

\out{ One simple, general example of a parts-based representation for
  a joint label space $Y = \{Y_1Y_2\dots Y_l\}$ is as follows. At the
  base of the cascade, the cliques consist of the singletons
  $\{Y_1\}$, $\{Y_2\}$, $\dots, \{Y_l|\}$; at each following level $t$
  of the cascade, the parts consist of unique unions of $t$ singleton
  sets. Therefore, we can construct $\phi_t$ as follows: if there are
  $l$ singletons, each part at level $t$ maps to exactly $l-t$ parts
  at level $t+1$. Any max marginal assignment to a part at level $t$
  will therefore have $k(l-t)$ consistent max marginal assignments at
  level $t+1$. In an sequence model such as a CRF or HMM, exactly such
  a parts-based representation is used, with the additional constraint
  that singletons may only be added to a part in sequential order (see
  Figure \ref{fig:lattice}).


To summarize, max marginals allow for a efficient representation of
the unpruned outputs determined by $r_\bw(x)$. Rather than attempting to
store all $y \in r_\bw(x)$, we instead store the set of
max marginals which score greater than the threshold $\theta$. When we
train or evaluate the next level of the cascade, we prune corresponding
parts of the lattice to limit the search space of the dynamic programming
or message passing algorithm of the next stage.
%to only those max marginals consistent with
%$\mcal{S}_t(x)$. If $\phi_t$ requires only constant time to evaluate,
the amortized complexity of this entire procedure is the same as the
original evaluation procedure for some $h(x)$ with the same features.
}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "cascades_aistats2010"
%%% End: 


==> text/aistats/sec_cascades.tex <==

% \begin{figure}
%   \centering
%   \resizebox{1.0\textwidth}{!} {
%     \input{figs/pruned_lattice}
%   }
% \caption{\small Max marginal-based cascade for a CRF based parts model
%   as implemented in experiments. {\em Left:} The original dense
%   lattice represents all $K$ assignments to all $L$ positions in the
%   lattice, with transitions between states representing bigrams. {\em
%     Center:} The first pruning function, $r_{\mbf{w}}$, prunes away
%   several of the potential assignments to singletons at difference
%   positions. {\em Right:} A mapping function $\phi$ maps singletons
%   in the sparse unigram lattice (Center) to a sparse set of bigram
%   parts in a one-to-many fashion. The set of unpruned edges in this
%   final lattice represent a sparse set of unpruned trigrams. This
%   process can be repeated to represent quad- or five-grams, if desired.}
%   \label{fig:lattice}
% \end{figure}

\section{Structured Prediction Cascades}
\label{sec:cascades}

% Our inspiration comes from the cascade classifier model
% of~\cite{viola01robustreal}, widely used for real-time detection of
% faces in images. In their work, a window is scanned over an image in
% search of faces and a cascade of very simple binary classifiers is
% trained to weed out easy and frequent negative examples early on.
% In the same spirit, we propose to learn a cascade of structured
% models of increasing order that weed out easy incorrect assignments
% early on.
%
%\subsection{Structured Classification}

Given an input space $\cX$, output space $\cY$, and a training set $S
= \{\ang{x^1,y^1},\dots,\ang{x^n,y^n}\}$ of $n$ independent and
identically-distributed ({i.i.d.}) random samples from a joint
distribution $D(X,Y)$, the standard supervised learning task is to learn a
hypothesis $h: \cX \mapsto \cY$ that minimizes the expected loss
$\E{D}{ \cL\left(h(x) , y\right)}$ for some non-negative loss function
$\cL : \cY \times \cY \rightarrow \reals^+$.

We consider the case of structured classification where $Y$ is a $\ell$-vector of variables and $\cY = \cY_1
\times \dots \times \cY_\ell$.  In many settings, the number of
random variables $Y$ differs depending on input $X$ (for example, length of the sentence in part of speech tagging), but for simplicity of notation, we assume a fixed number $\ell$ here.
We denote the components of $y$ as $y = \{y_1, \dots, y_\ell\}$, where $y_i \in \{1, \dots, K\}$.
The linear hypothesis class we consider is of the form:
\begin{equation}
  \label{eq:linear_classifiers}
  \hbw(x) = \argmax_{y\in\cY} \bw^\top\bft(x,y)
\end{equation}
where $\bw \in \reals^p$ is a vector of parameters and $\bft:
\cX\times\cY\mapsto\reals^p$ is a function mapping $(x,y)$ pairs to a
set of $p$ real-valued features. We further assume that $\bft$
decomposes over a set of cliques $\cC \subseteq \bbP\{X, Y\}$
(where $\bbP$ is a powerset):
\begin{equation}
  \label{eq:feature_sep}
  \bw^\top\bft(x,y) = \sum_{c \in \cC} \bw^\top\bft_c(x,y_c).
\end{equation}
Above, $y_c$ is an assignment to the subset of $Y$ variables in the clique $c$ and we will use $\cY_c$ to refer to the set all assignments to the clique. By considering different cliques over $X$ and $Y$, $\bft$ can represent arbitrary interactions between the components of $x$ and $y$. Thus, evaluating $\hbw(x)$ is not always tractable, and
computational resources limit the expressiveness of the features that
can be used.

For example, a first order Markov sequence model has cliques $\{Y_i,
Y_{i+1}, X\}$ to score features depending on emissions $\{X,Y_i\}$ and
transitions $\{Y_i, Y_{i+1}\}$:
\begin{equation}
\bw^\top\bft(x,y) = \sum_{i=1}^{\ell} \bw^\top\bft_i(x,y_i,y_{i+1}).
\end{equation}
For the first order model, evaluating \eqref{eq:linear_classifiers}
requires $O(K^2\ell)$ time using the Viterbi decoding algorithm. For
an order-$d$ Markov model, with cliques over $\{y_i, \dots, y_{i+d},
x\}$, inference requires $O(k^{d+1}\ell)$ time.

Several structured prediction methods have been proposed for learning
$\bw$, such as conditional random fields~\citep{lafferty01crfs},
structured perceptron~\citep{collins_discriminative_2002}, hidden
Markov support vector machines~\citep{altun03hmsvm} and max-margin
Markov networks~\citep{taskar03max}.  Our focus here is instead on
learning a cascade of increasingly complex models in order to
efficiently construct models that would otherwise be intractable.

\subsection{Cascaded inference with max-marginals}

We will discuss how to learn a cascade of models in Section 4, but
first we describe the inference procedure.  The basic notion behind
our approach is very simple: at each level of the cascade, we receive
as input a set of possible clique assignments corresponding to the
cliques of the current level. Each level further filters this set of
clique assignments and generates a set of possible clique assignments
which are passed as input to the next level. Note that each level is
able to prune further than the preceding level because it can consider
higher-order interactions. At the end of the cascade, the most complex
model chooses a single prediction as usual, but it needs only consider
the clique assignments that have not already been pruned. Finally,
pruning is done using clique max-marginals, for reasons which we
describe later in this section.

An example of a cascade for sequential prediction using Markov models
is shown is Figure \ref{fig:schematic}. A $d$-order Markov model has
maximal cliques $\{X, Y_i, Y_{i+1}, \dots, Y_{i+d}\}$. We can consider
a cascade of sequence models of increasing order as a set of bigram
models where the state space is increasing exponentially by a factor
of $K$ from one model to the next.  Given a list of valid assignments
$\cV^i$ in a $d$-order model, we can generate an expanded list of
valid assignments $\cV^{i+1}$ for a $(d+1)$-order model by
concatenating the valid $d$-grams with all possible additional states.

% For example, a $1$st-order (bigram) model scores cliques $\{X,Y_i,
% Y_{i+1}\}$, while a $2$nd-order (trigram) mode scores cliques $\{X,
% Y_i, Y_{i+1}, Y_{i+2}\}$. hus, we can consider a cascade of sequence
% models of increasing order as a set of bigram models where the state
% space is increasing exponentially by a factor of $K$ from one model to
% the next.  Given a list of valid assignments $\cV^i$ in a $d$-order
% model, we can generate an expanded list of valid assignments
% $\cV^{i+1}$ for a $(d+1)$-order model by concatenating the valid
% $d$-grams with all possible additional states.
% % We will discuss how to learn such a cascade in section
% \ref{sec:learning}, but first, we define its operation at inference
% time. The basic notion behind our approach is very simple: at each
% level of the cascade, we start with the output space filtered by a
% simpler model in the previous level and further filter the space by
% considering higher-order interactions. At the end of the cascade, a
% standard structured prediction model with the most complex
% interactions chooses an assignment over the final filtered space. A
% filtered space of outputs is represented by a set of valid clique
% assignments and the decision to prune a clique assignment is based on
% its max-marginal: the score of the best assignment consistent with
% this clique assignment.  The reason for using max-marginals is explained below.

More generally, for a given input $x$, for each maximal clique $c\in
\cC$ in the current level of the cascade, we have a list of valid
assignments $\cV_c \subseteq \cY_c$. Inference is performed only over
the set of valid clique assignments $\cV = \bigcup_{c \in \cC}
\cV_c$. Using the filtering model $\bw$ of the current cascade level,
the clique assignments in $\cV_c$ are scored by their max-marginals,
and a threshold $t$ is chosen to prune any $y_c \in \cV_c$ with a
score less than the threshold. The sets $\cV$ are then passed to the
next level of the cascade, where higher-order cliques consistent with
unpruned cliques are constructed. If we can eliminate at least a
fraction of the entries in $\cV$ on each round of the cascade, then
$|\cV|$ decreases exponentially fast and the overall efficiency of
inference is controlled.

Thus, to define the cascade, we need to define: (1) the set of models
to use in the cascade, and (2) a procedure to choose a threshold
$t$. In the remainder of this section we discuss our approach to these
decisions.

\begin{figure}
  \centering
  \includegraphics[width=0.45\textwidth]{figs/exp_factors_sparse.png}
  \vskip -2mm
  \caption{\small Schematic of a structured prediction cascade using
    unigram, bigram, and trigram Markov sequence models. Models are
    represented as factor graphs; as order increases, the state space
    grows, but the size of the filtered space remains small (filled
    area).}
  \label{fig:schematic}
\end{figure}

First, to define a set of models for the cascade, we require only that
the sets of cliques of the models form a nesting sequence. The cliques
of the models must satisfy the relation,
\begin{equation}
  \label{eq:nested}
  \cC^1 \subseteq \cC^2 \subseteq \dots \subseteq \cC^d,
\end{equation}
where $\cC^i$ is the set of cliques of the $i$'th model of the
cascade. In other words, every clique assignment $y_c$ of the $i$'th
model is contained in at least one clique assignment $y_c'$ of the
$(i+1)$'th model. This property allows for the use of increasingly
complex models as the depth of the cascade increases. As long as
\eqref{eq:nested} holds, a simple and intuitive mapping from the set
of valid cliques of the $i$'th model $\cV^i$ to a corresponding set of
valid cliques of the $(i+1)$'th model, $\cV^i$:
\begin{equation}
  \label{eq:cliquemapping}
  \cV^{i+1}_c = \{ y_c \in \cY_c \mid \forall c' \in \cC^i, c' \subseteq c, y_{c'} \in \cV_{c'}^i\}
\end{equation}
This is the set of clique assignments $y_c$ in the $(i+1)$'th model
for which all consistent clique assignments $y_{c'}$ for subcliques
$c' \in \cC^i$ have not been pruned by the $i$'th
model.

In order to filter clique assignments, we use their
\textit{max-marginals}.  We introduce the shorthand $\score{y} =
\bw^\top\bft(x,y)$ for the cumulative score of an output $y$, and
define the max marginal $\mmarg{y_c}$ as follows:
$$\mmarg{y_c} \triangleq \max_{y'\in \cY} \;\;\{ \score{y'} : y'_c = y_c\}.$$
Computing max-marginals can be achieved using the same dynamic
programming inference procedures in factor graphs as would be used to
evaluate \eqref{eq:linear_classifiers}. Most importantly, max
marginals satisfy the following simple property:
\begin{lem} [Safe Filtering]
  \label{prop:pruning}
  If $\score{y} > \mmarg{y'_c}$ for some $c$, then $y_c \ne y'_c $.
\end{lem}
Lemma \ref{prop:pruning} states that if the score of the true label
$y$ is greater than the max marginal of a clique assignment $y'_c$,
then that clique assignment $y'_c$ must be inconsistent with the truth
$y$. The lemma follows from the fact that the max marginal of any
clique assignment $y_c$ consistent with $y$ is at least the score of
$y$.

A consequence of Lemma \ref{prop:pruning} is that on training data, a sufficient
condition for the target output $y$ not to be pruned is that the
threshold $t$ is lower than the score $\score{y}$. Note that a similar
condition does not generally hold for standard sum-product marginals
of a CRF (where $p(y|x)\propto e^{\score{y}}$), which motivates our
use of max-marginals.

The next component of the inference procedure is choosing a threshold
$t$ for a given input $x$.  Note that the threshold cannot be defined
as a single global value but should instead depend strongly on the
input $x$ and $\score{\cdot}$ since scores are on different scales. We
also have the constraint that computing a threshold function must be
fast enough such that sequentially computing scores and thresholds for
multiple models in the cascade does not adversely effect the
efficiency of the whole procedure. One might choose a quantile
function to consistently eliminate a desired proportion of the max
marginals for each example. However, quantile functions are
discontinuous in the score function, and we instead approximate a
quantile threshold with a more efficient {\em mean-max} threshold
function, defined as a convex combination of the mean of the max
marginals and the maximum score $\scoremax = \max_y \score{y}$,
\begin{equation}
  \label{eq:meanmax}
  \thr = \alpha \scoremax + (1-\alpha)\frac{1}{|\cV|} \sum_{c\in\cC, y_c\in V_c} \mmarg{y_c}.
\end{equation}
Choosing a mean-max threshold is therefore choosing $\alpha \in
[0,1)$. Note that $\thr$ is a convex function of $\score{\cdot}$ (in
fact, piece-wise linear), which combined with Lemma
\ref{prop:pruning} will be important for learning the filtering models
and analyzing their generalization. In our experiments, we found that
the distribution of max marginals was well centered around the mean,
so that choosing $\alpha \approx 0$ resulted in $\approx50\%$ of max
marginals being eliminated on average. As $\alpha$ approaches $1$, the
number of max marginals eliminated rapidly approaches $100\%$. We used
cross-validation to determine the optimal $\alpha$ in our experiments
(section \ref{sec:experiments}).

%by concatenating each state $y_j \in \cV^i$ with
%the set of values $\{1, \dots, k\}$. For example, given $\cV^i$ for a
%bigram model, the resulting trigram set is $\cV^i' = \{ y_jy_k\dots
%y_j \in \cV^i, y_k \in \{1, \dots, k\}\}$. Note that the $0$-order
%(unigram) and bigram models share the same state space. Furthermore,
%given the lists of valid states $\cV$, it is straightforward to modify the Viterbi algorithm to search only over the set of unpruned
%labels.

\out{
For sequence models, we can now summarize the cascaded inference
process for a given input $x$ as follows: first, we initialize $\cV_i
= \{1, \dots, K\}$ for each position $Y_i$ in the input. We then
repeat for each model in our cascade:
\begin{packed_itemize}
\item Compute the (possibly expanded) sets of valid assignments $\cV'$
  for the the $(d+1)$-order model that are consistent with the sets $\cV$
  of the previous $d$-order model.
\item Comptute $\mmarg{y_j}$ for all $y_j \in \cV$ using the
  forward-backward algorithm.
\item Compute $\thr$ and eliminate any max marginals
  that score below threshold from $\cV$.
\item Pass $\cV$ to the next model in the cascade.
\end{packed_itemize}

To terminate the cascade, we simply evaluate the argmax
\eqref{eq:linear_classifier} instead of copmuting max marginals, and
return.
}


% Our inspiration is the

% Even given an optimal pruning function, exponentially large
% output spaces pose additional difficulties that must be addressed in
% order for the pruning function to be of any practical use. First, for
% any fixed pruning rate, the output of the pruning
% function will be exponential in size if $\mcal{Y}(x)$ is
% exponential. Therefore a compact representation must be found to
% represent the set of unpruned outputs $r_{\bw}(x, \cY(x))$. Second, we
% must be able to efficiently modify our inference procedure to take
% advantage of the reduced output space, i.e., to compute
% \begin{equation}
%   \label{eq:efficient_hyp}
%   h_{\mbf{\widetilde{\bw}}}(x) = \argmax_{y\in r_{\bw}(x,\cY(x))} \widetilde{\bw}^\top\mbf{f}(x,y) ,
% \end{equation}
% for some pruning function $r_{\mbf{w}}(x)$. Finally, as alluded to
% earlier, pruning an exponentially large output space by some fixed
% proportion will only reduce, but not eliminate, the exponential
% complexity of inference. Ideally, our pruning procedure would prune
% away an exponentially large portion of the output space of roughly the
% same order as the difficulty of the original problem. In this section,
% we propose a simple and general pruning procedure that
% addresses each of the above difficulties.

% %\subsection{Efficient pruning}% with max marginals}
% %\label{sec:cascade}

% We use a clique-based representation of the feature function to
% compactly store an exponential number of unpruned labels. We define
% the {\em max marginal} for a clique $c$, an assignment $Y_c = y_c$, and a
% parameter vector $\mbf{w}$ as the following,
% \begin{equation}
%   \label{eq:max_marginal_part}
%   s_{\mbf{w}}^\star(x,y_c) \triangleq \max \{\mbf{w}^\top\mbf{f}(x,y')\mid y' \in \cY(x), y'_c = y_c\},
% \end{equation}
% which is the best possible score for any output $y$ that is consistent
% with the assignment $y_c$. Suppose $s_{\mbf{w}}^\star(x,y_c)$ is less
% than some desired pruning threshold $\theta$. By definition, the score
% of any other output consistent with the assignment $y_c$ cannot be
% higher than $s_{\mbf{w}}^\star(x,y_c)$. We can therefore make the
% following simple statement: if for any $y \in \mcal{Y}$, there exists
% some part $c$ such that $s_{\mbf{w}}^\star(x,y_c) \le \theta$, then
% the score $\mbf{w}^\top\mbf{f}(x,y) \le \theta$ as well. Thus, for a
% given $\theta$, the following relationship holds:
% \begin{equation}
%   \label{eq:efficient_pruner}
%   r_{\mbf{w}}(x,\cY(x)) \subseteq g_{\mbf{w}}(x,\cY(x)),
%     \qquad g_{\mbf{w}}(x,\cY(x)) =  \bigcap_{c \in \mcal{C}}\{y \in \cY(x): s_{\mbf{w}}^\star(x,y_c) > \theta\}.
% \end{equation}
% That is, we can represent a superset of the output of the pruning function
% $r_{\mbf{w}}$, which may be exponential in size, with the max marginal
% pruning function $g_{\mbf{w}}$, which is represented locally on cliques.
% Note that to efficiently evaluate $g_{\mbf{w}}$, it is only required
% to compute and store the max-marginals, which by assumption are
% polynomial in the length of the input.
% %For a given partial assignment
% %$y_c$, we can then query whether any $y$ consistent with $y_c$ is
% %pruned by $g_{\mbf{w}}$ in $O(1)$ time.


% An illustration of this process for sequences (cliques of size $2$)
% appears in Figure~\ref{fig:max_marginals}. The left panel shows three
% possible labels, organized in two cliques, both containing the second
% vertex. The middle panel shows all possible labelings of this graph,
% where each vertex can be labeled as either {\tt a}, {\tt b} or {\tt
%   c}. Furthermore, the all the labelings that are consistent with
% $y_2=\mathtt{b}$ are marked with bold blue edges. Finally, the right
% panel illustrates the maximization operation over all consistent
% labelings, which is the value of max-marginal
% $s_{\mbf{w}}^\star(x,Y_2=b)$.

\out{
Given an efficient representation for $g_\bw$, we must still find a way
to take advantage of $g_\bw$ when evaluating the next hierarchy of the
cascade. Let $\mcal{C}_t$ be the parts for $\mbf{f}$ used at level $t$
of the cascade hierarchy, and let $\mcal{C}_t(x)$ be the set of max
marginals $\ang{c,\hat{y}_c}$ that are unpruned by $r(x)$ at the
previous level. Since we are using a cascade of models of increasing
complexity, there exists a mapping $\phi_{t}: \mcal{C}_{t} \times
\mathbb{Z}^+ \mapsto \mcal{P}_{t+1} \times \mathbb{Z}^+$ that relates
max marginals in $\mcal{P}_{t}$ to max marginals in $\mcal{P}_{t+1}$,
\begin{equation}
  \label{eq:part_mapping}
  \phi_{t}(p, \hat{y}_p) = \left\{\ang{p',\hat{y}_{p'}} \mid p' \in \mcal{P}_{t+1}, \hat{y}_{p} \subseteq \hat{y}_{p'} \right\}.
\end{equation}
By definition, $\ang{p,\hat{y}_p} \in \mcal{S}_t(x)$ implies that
$\phi(p,\hat{y}_p) \in r(x)$. Therefore, when we compute the maximum
over assignments to some part $p$ during dynamic programming or
message passing at the next level of the cascade, we only need to
consider all assignments $\ang{p,\hat{y}_{p}} \in
\phi(p',\hat{y}_{p'})$ for which $\ang{p',\hat{y}_{p'}} \in
\mcal{S}_t$. If we can evaluate $\phi_{t}$ in constant time, then we
do not pay any amortized overhead for the translation process.
}

\out{
Finally, the step of passing the representation of the reduced
assignment space from one level of
the cascade to the next level is illustrated in Figure
\ref{fig:lattice} where we start with all possible labels (left), then
prune vertices using max-marginals (middle), and transfer the labeling graph to a
second order lattice.
%This transformation can be computed efficiently.


%\subsection{Sparse forward-backward inference}

We can incorporate the sparse lattice $\mcal{V}$ into the well-known
forward-backward \citep{rabiner} algorithm for HMM/CRF models with
little difficulty. Let $\mcal{F}_k$ and $\mcal{B}_k$ be the set of
valid forward and backward transitions for the $k$'th state in the
model, respectively. We modify forward-backward as follows:
\begin{packed_enum}
\item At each position $j$, we compute coefficients only over the
  sparse set of valid states $\mcal{V}_j$.
\item For each state $k \in \mcal{V}_j$, we maximize only over the
  intersection $\mcal{F}_K \cap \mcal{V}_{j+1}$ or $\mcal{B}_k \cap
  \mcal{V}_{j-1}$.
\end{packed_enum}
By using a sparse datastructure to store $\mcal{V}$, we can enumerate
all $k \in \mcal{V}_j$ in $O(|\mcal{V}_j|)$ time and enumerate all $k
\in \mcal{F}_k \cap \mcal{V}_{j+1}$ in
$O(\min\{|\mcal{F}_k|,|\mcal{V}_{j+1}|\})$ time. Once the forward and
backward coefficients have been computed, the max marginal
$s_{\mbf{w}}^\star(x,Y_j=k)$ is simply the sum of the forward and
backward coefficients $\delta_j(k) + \beta_j(k)$, respectively.


\begin{algorithm}
  \label{alg:pruning}
  \KwIn{Example $x$, parameter $\alpha$, pruning weights $\mbf{w}^{(d)}$.}
  \KwInit the unpruned lattice: $\forall j, \mcal{V}_j = Y_j$.

  \For{$d = 1$ \KwTo $(D-1)$}{
    \begin{packed_enum}
    \item Run sparse Forward-Backward using $\mbf{w}^{(d)}$ and the
      lattice $\mcal{V}$ to compute $\delta$ and $\beta$.
    \item Compute the pruning threshold $\theta$ from $\delta$, $\beta$, and
      $\mcal{V}$% using Equation \eqref{eq:pruning_forward_backward}.
    \item Remove any vertices corresponding to max marginals
      $\delta_j(k) + \beta_j(k) \le \theta$ from $\mcal{V}_j$.
    \item If $d \ge 1$: Using $\phi$, generate a sparse order-($d+1$) lattice from
      $\mcal{V}$ (e.g., Figure \ref{fig:lattice}).
    \end{packed_enum}
  }
  \KwRet The pruned order-$D$ sparse lattice $\mcal{V}$.

  \caption{Pruning a lattice with the cascade.}
\end{algorithm}
}

\out{ One simple, general example of a parts-based representation for
  a joint label space $Y = \{Y_1Y_2\dots Y_l\}$ is as follows. At the
  base of the cascade, the cliques consist of the singletons
  $\{Y_1\}$, $\{Y_2\}$, $\dots, \{Y_l|\}$; at each following level $t$
  of the cascade, the parts consist of unique unions of $t$ singleton
  sets. Therefore, we can construct $\phi_t$ as follows: if there are
  $l$ singletons, each part at level $t$ maps to exactly $l-t$ parts
  at level $t+1$. Any max marginal assignment to a part at level $t$
  will therefore have $k(l-t)$ consistent max marginal assignments at
  level $t+1$. In an sequence model such as a CRF or HMM, exactly such
  a parts-based representation is used, with the additional constraint
  that singletons may only be added to a part in sequential order (see
  Figure \ref{fig:lattice}).


To summarize, max marginals allow for a efficient representation of
the unpruned outputs determined by $r_\bw(x)$. Rather than attempting to
store all $y \in r_\bw(x)$, we instead store the set of
max marginals which score greater than the threshold $\theta$. When we
train or evaluate the next level of the cascade, we prune corresponding
parts of the lattice to limit the search space of the dynamic programming
or message passing algorithm of the next stage.
%to only those max marginals consistent with
%$\mcal{S}_t(x)$. If $\phi_t$ requires only constant time to evaluate,
the amortized complexity of this entire procedure is the same as the
original evaluation procedure for some $h(x)$ with the same features.
}
\out{
\begin{table}
  \centering
\small
\begin{tabular}{|rll|}
  \hline {\bf Function} & {\bf Map} & {\bf Definition} \\ \hline
%  $\ssp$ & $\cX \mapsto \reals^m$ &
%  $\left\{ \forall c \in \cC, \forall y_c \::\: \bw \cdot \bft_c(x,y_c) \right\}$ \\
  $\score{y}$ & $\cX \times \cY \mapsto \reals$ & $\bw^\top \bft(x,y)$ \\
  $\scoremax$ & $\cX \mapsto \reals$ & $\max_y \score{y}$ \\
  $\mmarg{y_c}$ & $\cX \times \cY_\cC \mapsto \reals$ & $\max_{y': y_c = y_c'} \score{y'}$ \\
  $\wit{y_c}$ &  $\cX \times \cY_\cC \mapsto \cY$ & $\argmax_{y': y_c = y_c'} \score{y'}$\\
  \hline
\end{tabular}
\caption{\small Summary of notation.}
\end{table}
}
% For a
% given $y \in \cY$, we denote the components of $y$ as $y_1, \dots,
% y_\ell$, where $y_j \in \{1,\dots,K\}$. In this case, $|\cY|$ is
% bounded by $K^\ell$, which grows exponentially with $L$. Typically,
% $\mbf{f}(x,y)$ can be decomposed into separate feature functions on
% the set of cliques $C$ of $x$ and $y$,
%We have deliberately left the definition of the set of ``parts,''
%$\mcal{P}(x,y)$, vague. For each application or problem,
%$\mcal{P}(x,y)$ represents the subsets of $x$ and $y$ that directly
%interact with one another.
% For instance, in a log-linear pairwise
% Markov network on a graph $G$, the cliques consist of sets of individual
% vertices or pairs of vertices connected by an edge in $G$.
% %\citep{Taskar:1210}.
% By limiting the graph to a sequence (or a tree), it is then
% possible to use dynamic programming or message passing
% %other linear decoding algorithm on the associated graph
% to evaluate Eq.~\eqref{eq:linear_classifiers} in linear time in $L$.
% As we include higher order interactions between variables in $y$
% inference becomes impractical. For example, the inference of a Markov
% models of order $q$ is $O(K^{q+1}L)$ which is infeasible even moderate
% values of $K$.
% %\citep{Taskar:1210,druck_learning_2007}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cascades_aistats2010"
%%% End:


==> text/aistats/sec_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\paragraph{Handwriting Recognition.} We first evaluated the accuracy
of the cascade using the handwriting recognition dataset from
\citet{taskar03max}. This dataset consists of 6877 handwritten words,
with avereage length of $\sim$8 characters, from 150 human subjects,
from the data set collected by \citet{Kassel_Thesis}. Each word was
segmented into characters, each character was rasterized into an image of 16 by 8 binary pixels. The dataset is divided into 10 folds; we used 9 folds for training and a single withheld for testing (note that
\citet{taskar03max} used 9 folds for testing and 1 for training due to
computational limitations, so our results are not directly
comparable). Results are averaged across all 10 folds.

Our objective was to measure the improvement in predictive accuracy as
higher order models were incorporated into the cascade. The final
cascade consisted of four Markov models of increasing order. Pixels
are used as features for the lowest order model, and 2,3, and 4-grams
of letters are the features for the three higher order models,
respectively. The maximum filter loss threshold $\epsilon$ was set to
1\%, 2\%, and 4\% (this avoids over-penalizing higher order models),
and we trained structured cascades (SC) using $\alpha$'s from the candidate set $\{0,
0.25, 0.5\}$. To simplify training, we fixed $\eta = 1$, $\lambda =
0$, and used an early-stopping procedure to choose $\bw$ that achieved
optimal tradeoff according to \eqref{eq:cascade_learning}.

Results are summarized in Table \ref{tab:ocr}. We found that the use
of higher order models dramatically increased accuracy of the
predictions, raising accuracy at the character above 90\% and more
than tripling the word-level accuracy. Furthermore, the cascade
reduced the search space of the 4-gram model by 5 orders of magnitude,
while incurring only 3.41\% filtering error.

\paragraph{Part-of-Speech Tagging.} We next evaluated our approach on
several part of speech (POS) tagging tasks. Our objective was to
rigorously compare the efficacy of our approach to alternative methods
on a problem while reproducing well-established benchmark prediction
accuracy. The goal of POS tagging is to assign a label to each word in
a sentence. We used three different languages in our experiments:
English, Portuguese and Bulgarian. For English, we used volumes 0-17
of the Wall Street Journal portion of the Penn
TreeBank~\citep{PennTreebank} for training, volumes 18-20 for
development, and volumes 21-24 for testing. We used the Bulgarian
BulTreeBank~\citep{Simov02buildinga} and the Bosque subset of the
Portuguese Floresta Sinta(c)tica~\citep{floresta}
%\footnote{http://www.linguateca.pt/Floresta/}
for Bulgarian and Portuguese datasets, respectively.

For these experiments, we focused on comparing the efficiency of our
approach to the efficiency of several alternative approaches. We again
used a set of Markov models of increasing order; however, to increase
filtering efficiency, we computed max marginals over subcliques
representing $(d-1)$ order state assignments rather than $d$-order
cliques representing transitions. Thus, the bigram model filters
unigrams and the trigram model filters bigrams, etc. Although we ran
the cascades up to 5-gram models, peak accuracy was reached with
trigrams on the POS task.

\out{We used a held-out development set to
estimate the losses $\cL_e$ and $\cL_f$ during training and thus to
enforce the constraint $\cL_f \le \epsilon$.}\out{we used early-stopping For perceptron
algorithms, we used early-stopping over 30 passes in randomized order
through the training data, and taking the average $\bw$ over all
epochs and steps through the training data (averaged perceptron).}
 \out{If the constraint $\cL_f \le \epsilon$
was still violated after solving for $\bw$, we fixed $\bw$ and relaxed
the $\alpha$ until either $\alpha = 0$ or the constraint was satisfied
on the held-out data. We conducted two separate experiments with the
algorithms.}
%Words that
%occurred less than 10 times in the training data were replaced by
%``rare'' tokens.

We compared our SC method to two baselines: the standard structured
perceptron (SP) and a maximum a posteriori CRF. All methods used the
same standard set of binary features: namely, a feature each
(word,tag) pair $\ind{X_t = x_t, Y_t = y_t}$ and feature for each
$d$-gram in the model. For the baseline methods, we trained to
minimize classification error (for SP) or log-loss (for CRF) and then
chose $\alpha \in [0,1]$ to achieve minimum $\cL_e$ subject to $\cL_f
\le \epsilon$ on the development set. For the CRF, we computed
sum-product marginals $P(y_c|x) = \sum_{y': y'_c = y_c} P(y'|x)$, and
used the threshold $\thr = \alpha$ to eliminate all $y_c$ such that
$P(y_c|x) \le \alpha$. For all algorithms, we used grid search over
several values of $\eta$ and $\lambda$, in addition to early stopping,
to choose the optimal $\bw$ based on the development set.  For
SC training, we considered initial $\alpha$'s from the candidate set
$\{0, 0.2, 0.4, 0.6, 0.8\}$.

We first evaluated our approach on the WSJ dataset.  \out{We took the
  optimal $\bw$ over $\eta \in \{1.0, 0.1, 0.001, 0.0001\}$, selecting
  on the development set.} To ensure accuracy of the final predictor,
we set a strict threshold of $\epsilon = 0.01$\%. All methods were
trained using a structured perceptron for the final classifier. The
results are summarized in Table \ref{tab:fullwsj}. SC was compared to
CRF, an unfiltered SP model (Full), and a heuristic baseline in which
only POS tags associated with a given word in the training set were
searched during inference (Tags). SC was two orders of magnitude
faster than the full model in practice, with the search space reduced
to only $\approx 4$ states per position in inference (roughly the
complexity of a greedy approximate beam search with 4 beams.)  SC
also outperformed CRF by a factor of 2.6 and the heuristic by a factor
of 6.8. Note that because of the trade-off between accuracy and
efficiency, CRF suffered less filter loss relative to SC due to
pruning less aggressively, although neither method suffered enough
filtering loss to affect the accuracy of the final
classifier. Finally, training the full trigram POS tagger with exact
inference is extremely slow and took several days to train; training
the SC cascade took only a few hours, despite the fact that more
models were trained in total.

% Although CRF suffered less filter loss than
% SCP, we established In figure~\ref{fig:times}, we plot test set
% runtime improvement over unfiltered trigram model for the three
% different filtering methods.

\begin{table}
  \centering
  {\small
    \begin{tabular}{|l|cccc|}
    \hline {\bf Model Order:} & {\bf 1} & {\bf 2} & {\bf 3} & {\bf 4} \\
    \hline
    Accuracy, Char. (\%) & 77.44 & 85.69 & 87.95 & 92.25 \\
    Accuracy, Word (\%) & 26.65 & 49.44 & 73.83 & 84.46 \\
    Filter Loss (\%) & 0.56 & 0.99 & 3.41 & --- \\
    Avg. Num $n$-grams & 26.0 & 123.8 & 88.6 & 5.4\\
    \hline
  \end{tabular}}
\caption{\small {Summary of handwriting recognition results.} For each level of the
  cascade, we computed prediction accuracy (at character and word
  levels) using a standard voting
  perceptron algorithm as well as the filtering loss and average
  number of unfiltered $n$-grams per position for the SC on the test set.}
  \label{tab:ocr}
\end{table}
\begin{table}

  \centering
  {\small
  \begin{tabular}{|l|cccc|}
    \hline {\bf Model:} & {\bf Full} & {\bf SC} & {\bf CRF} & {\bf Tags} \\
    \hline
    Accuracy (\%) & 96.83 & 96.82& 96.84 & --- \\
    Filter loss (\%) & 0& 0.121 & {\bf 0.024} & 0.118 \\
    Test Time (ms) & 173.28 & {\bf 1.56} & 4.16 & 10.6 \\
    Avg. Num States & 1935.7 & {\bf 3.93} & 11.845 & 95.39 \\
    \hline
  \end{tabular}}
\caption{\small Summary of WSJ Results.
  Accuracy is the accuracy of the final trigram model.
  Filter loss is the number of incorrectly pruned bigrams at the end of the cascade.
  The last row is the average number of states considered at each position in the test set.}
  \label{tab:fullwsj}
\end{table}


% \begin{figure}
%   \centering
%   \includegraphics[width=0.50\textwidth]{figs/exp2-effs-trans.jpg}
%   \caption{\small Full WSJ runtime efficiency on the test set. Blue
%     (`o') is SCP, green (`x') is CRF, and orange
%     (`{\tiny $\Delta$}') is a tag-list heuristic. Points
%     represent test set runtime improvement over unfiltered trigram model
%     (y-axis) as a function of sentence length (x-axis).}
%   \label{fig:times}
% \end{figure}

% We tried fitting $\bw$ with all combinations of $\eta \in \{0.1,
% 0.01, 0.001\}$ and (due to the reduced training set size) a
% $\ell_2$-norm regularization parameter $\lambda \in \{1, 0.1, 0.01,
% 0.001\}$, taking the $\bw$ with optimal performance over all
% combinations.

We next investigated the efficiency vs. filtering accuracy trade-off
of SC compared to the SP and CRF baselines on all three
languages. For each of the three languages, we generated 10 different
training sets from 40\% of the full training datasets. Randomization
was taken with the same 10 seeds for each dataset/algorithm pair. For
all methods, we trained bigram models under two conditions: first, as
the initial step of a cascade (e.g., no prior filtering), and second,
as the second step of a cascade after initial filtering by the SC
algorithm with $\epsilon = 0.05$\%, and analyzed the resulting
trade-off between efficiency and accuracy.

The results are presented in Figure \ref{fig:tradeoff}. The figures
were generated by computing for each $\epsilon$ along the x-axis the
corresponding {\em test} efficiency $\cL_e$ when the constraint on
filter loss ($\cL_f \le \epsilon$) is enforced using {\em development}
set data. Points for which the constraint could not be enforced (even
with $\alpha=0$) are not shown. SC handily beats the competitors in
both the filtered and unfiltered case. Note that in the unfiltered
condition, the CRF is unable to achieve significant pruning efficiency
for any $\epsilon$, while the SP cannot achieve filtering accuracy for
small $\epsilon$. However, because SC and SP become equivalent as
$\alpha$ approaches 1, we observe that the performance
of SC and SP converge as $\epsilon$ increases.

\out{In the unfiltered
condition, SC is significantly more efficient than CRF and SP for a
given $\epsilon$. In the filtered condition, SC was the only method
to have a smooth trade-off between filtering accuracy and
efficiency. The SP algorithm reaches minimum $\cL_f$ around $\epsilon
= 0.1\%$ and cannot increase accuracy further, while the sum-product
marginals in the CRF are simply unable to prune more than 30\% of
marginals, regardless of $\epsilon$.}

\begin{figure}
  \centering
  {\tiny \bf Unfiltered Bigram}
  % files got accidentally switched
  \includegraphics[width=0.50\textwidth]{figs/exp1-filtered.png}
  {\tiny
    \vskip -2mm Development Set Filter Loss Threshold $\epsilon$ (\%)}

  {\tiny \bf Filtered Bigram}
  \includegraphics[width=0.48\textwidth]{figs/exp1-unpruned.png}
  {\tiny
    \vskip -2mm Development Set Filter Loss Threshold $\epsilon$ (\%)}

  \caption{\small Efficiency vs. accuracy trade-off for unfiltered
    (top) and filtered (bottom) bigram models on POS tagging task. Blue
    (darkest) is SC, green (lighter) is CRF, and orange is SP
    (lightest). Shaded region shows standard error over 10 different
    random training sets. The y-axis show the test set efficiency when
    fitting to enforce the constraint $\cL_f \le \epsilon$ (x-axis) on
    development data.}
  \label{fig:tradeoff}
\end{figure}


%  \begin{figure}
%    \centering
%    \includegraphics[width=0.33\textwidth,clip=true,trim=0.3in 0.5in 0.5in 0.5in]
%    {figs/ptb_small0_alphas}
%    \includegraphics[width=0.33\textwidth,clip=true,trim=0.3in 0.5in 0.5in 0.5in]
%    {figs/ptb1_alphas}
%    \caption{\small Comparison recall-efficiency trade-offs for pruning
%      perceptron and structured perceptron on the WSJ dataset (Left:
%      flat model, Right: bigram model.) Curves were generated by
%      computing the pruning error and pruning efficiency (proportion of
%      pruned max marginals) for all possible $\alpha$ relaxations
%      available to each method. E.g., PP$\alpha$ trained with $\alpha =
%      0.6$ was evaluated for $\alpha \in [0,0.6]$, while PP$\alpha$
%      trained with $\alpha = 0$ results in a single point. The
%      $\epsilon = 0.05\%$ pruning error cap is marked with a horizontal
%      dashed line; intercepts with this line are the efficiencies of
%      each method given an error cap of $0.05\%$.}
%    \label{fig:pos_eff}
% \end{figure}

% We also computed several interesting theoretical metrics for each
% cascade. For example, to compare the size of the pruned search space
% without taking into account implementation overhead, we computed the
% average number of valid states at a given position in the lattice
% ($|\mcal{V}_j|$) and the average number of valid transitions to be
% scored ($|\mcal{F}_k \cap \mcal{V}_j|$). Multiplying these gives the
% average number of scoring operations per position, and summing up all
% scoring operations in the entire cascade, we can compare the
% theoretical efficiency of the Viterbi algorithm (Vit) against the
% naive baseline or an approximate inference method such as beam
% search. Thus, for the WSJ data the pruning cascade needed 628X fewer
% scoring operations than baseline, which we can also compute is roughly
% equivalent to the number of scoring operations required if a beam
% search was used with only 3 beams ($\approx$Beam).


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cascades_aistats2010"
%%% End:


==> text/aistats/sec_learning.tex <==
\section{Learning the cascade}
\label{sec:learning}

We now turn to the problem of finding the best parameters $\bw$ and
the corresponding best tuning of the threshold $\alpha$ for each level of the cascade. 
When learning a cascade, we have two competing objectives that we must trade off:\\
%\begin{packed_itemize}
%\item {\em Accuracy:}
{\em $\bullet$ Accuracy:} Minimize the number of errors incurred by each
  level of the cascade to ensure an accurate inference process in
  subsequent models.\\
%\item {\em Efficiency:}
{\em $\bullet$ Efficiency:} Maximize the number of filtered max marginals at
  each level in the cascade to ensure an efficient inference process in subsequent models.
%\end{packed_itemize}

We quantify this trade-off by defining two loss functions. We
define the {\em filtering loss} $\cL_f$ to be a 0-1 loss indicating a mistakenly eliminated correct assignment. The {\em efficiency loss}
$\cL_e$ is the proportion of unfiltered clique assignments.

\begin{defn}[Filtering loss] Let $\ssp$ be the scoring function in the current level of the cascade. A filtering error occurs when a max-marginal of a clique assignment of the correct output $y$ is pruned.
%When $\score{y} > \thr$ no error occurs, however, when $\score{y} \le \thr$ a filtering error could occur.
We define filtering loss as $\cL_f(y, \ssp) = \ind{\score{y} \le \thr}$.
\end{defn}
\begin{defn}[Efficiency loss] Let $\ssp$ be defined as above.
%, where  $\ssp \in \reals^m$.
  The efficiency loss is the proportion of unpruned clique assignments  $\cL_e(y,\ssp) = \frac{1}{|\cV|}\sum_{c\in C, y_c\in \cV_c} \ind{\mmarg{y_c} \ge \thr}$.
\end{defn}

Note that we can trivially minimize either of these at the
expense of maximizing the other. If we set ($\bw,\alpha$) to achieve
a minimal threshold such that no assignments are ever filtered, then
$\cL_f = 0$ and $\cL_e = 1$. Alternatively, if we choose a threshold
to filter every assignment, then $\cL_f = 1$ while $\cL_e = 0$. To
learn a cascade of practical value, we can minimize one loss while constraining the 
other below a threshold $\epsilon$. Since the ultimate goal of the cascade is accurate 
classification, we focus on the problem of
minimizing efficiency loss while constraining the filtering loss to be
below a desired tolerance $\epsilon$.

We can express the cascade learning objective as a joint optimization
over $\bw$ and $\alpha$:
\begin{equation}
  \label{eq:cascade_learning}
  \min_{\bw,\alpha}\;\; \bbE\left[ \cL_e(Y,\sspRV)\right] \textrm{ s.t. } \bbE\left[ \cL_f(Y,\sspRV)\right] \le \epsilon,
\end{equation}
%where $l(x^i)$ is the length of the $i$'th example. 
We solve this problem with a two-step procedure. First, we define a convex
upper-bound on the filter error $\cL_f$, making the problem of
minimizing $\cL_f$ convex in $\bw$ (given $\alpha$). We learn $\bw$ to
minimize filter error for several settings of $\alpha$ (thus
controlling filtering efficiency). Second, given $\bw$, we optimize the
objective \eqref{eq:cascade_learning} over $\alpha$ directly, using
estimates of $\cL_f$ and $\cL_e$ computed on a held-out development
set. In section \ref{sec:theory} we present a theorem bounding the
deviation of our estimates of the efficiency and filtering loss from
the expectation of these losses.

% \subsection{Structured Filter Learning}
% One approach to learning $\bw$ would be
% to solve the following convex margin optimization problem (for a fixed
% $\alpha$):
% \begin{eqnarray*} \inf_{\bw,\xi\ge 0} && \frac{1}{2}||\bw||^2 +
% \sum_i^n \xi_i \\ {\rm s.t. }\;\;\; && \bw^\top\bft(x^i,y^i) \ge \thri + 1 - \xi_i, \;\;\;
% \end{eqnarray*}

To learn one level of the structured cascade model $\bw$ for a fixed $\alpha$, we pose the
following convex margin optimization problem:
\begin{equation}
  \label{eq:convex_opt}
\mathbf{SC:}\;\;\;\;  \inf_{\bw} \;\;\;\ \frac{\lambda}{2}||\bw||^2 + \frac{1}{n}\sum_i H(\bw;(x^i,y^i)),
\end{equation}
where $H$ is a convex upper bound on the filter loss $\cL_f$,
\begin{equation*}
  H(\bw;(x^i,y^i)) = \max\{0, \ell + \thri - \bw^\top\bft(x^i,y^i)\}.
\end{equation*}
The upper-bound $H$ is a hinge loss measuring the margin between the
filter threshold $\thri$ and the score of the truth
$\bw^\top\bft(x^i,y^i)$; the loss is zero if the truth scores above
the threshold by margin $\ell$ (in practice, the length $\ell$ can
vary by example).  We solve \eqref{eq:convex_opt} using stochastic
sub-gradient descent. Given a sample $(x,y)$, we apply the following
update if $H(\bw;(x,y))$ (i.e., the sub-gradient) is non-zero:
\begin{equation}
  \begin{split}
    \label{eq:spf_update}
    \bw' & \leftarrow (1-\lambda)\bw + \eta \bft(x,y) - \eta \alpha \bft(x,y^\star)   \\
    & \quad - \eta(1-\alpha) \frac{1}{|\mcal{V}|} \sum_{c \in \cC, y_c} \bft(x,\wit{y_c}).
  \end{split}
\end{equation}
Above, $\eta$ is a learning rate parameter, $y^\star = \argmax_{y'}
\score{y'}$ and $\wit{y_c} = \argmax_{y': y_c = y_c'} \score{y'}$.
The key distinguishing feature of the this update as compared to
structured perceptron is that it subtracts features included in all
max marginal assignments $\wit{y_c}$.

Note that because \eqref{eq:convex_opt} is $\lambda$-strongly convex,
if we chose $\eta_t = 1/(\lambda t)$ and add a projection step to keep 
$\bw$ in a closed set, the update would correspond to the Pegasos
update with convergence guarantees of $\tilde{O}(1/\epsilon)$ iterations for
$\epsilon$-accurate solutions
\citep*{conf/icml/Shalev-ShwartzSS07}.

%  In this paper, we use a
% sub-gradient chose instead to find $\bw$ using an online, perceptron
% style algorithm that can be seen as an approximate solver for the
% above problem. We start with an initial estimate $\bw^{(0)} = 0$. In
% the standard structured perceptron algorithm
% \citep{collins_discriminative_2002}, one would decode the $\argmax$
% assignment $y^\star$ using current weights $\bw$ for each training
% example $(x,y)$ and update $\bw' \leftarrow \bw + \eta \bft(x,y) -
% \eta \bft(x,y^\star)$ if the mistake $\ind{y^\star \ne y}$ occurs. The
% parameter $\eta$ is a learning rate. Our Structured Cascade Perceptron
% (SCP) algorithm instead defines mistakes to solve convex margin
% optimization problem for fixed $\alpha$. Thus, we define mistakes as
% $\ind{\score{y} < \thr + 1}$. Our update \eqref{eq:spf_update} is
% therefore similar to the perceptron update except that instead of
% subtracting $\bft(x,y^\star)$ from $\bw$ after a mistake, we need to
% subtract all the features used to compute $\thr$:

%We use the following iterative procedure to optimize
%\eqref{eq:cascade_learning}.
%, which we call the {\bf S}tructured {\bf
%  P}erceptron {\bf F}ilter (SPF).
%A high level summary is as
%follows.
%We first choose an initial $\alpha$ to determine the
%``aggressiveness'' of the filtering step and a filtering loss
%constraint $\cL_f \le \epsilon$. With $\alpha$ fixed, we then find the
%$\bw$ with minimal filtering loss on training data using the online
%algorithm above \eqref{eq:spf_update}.
%If the minimal
%$\bw$ does not satisfy the constraint $\cL_f \le \epsilon$, we relax
%$\alpha$ until either $\alpha = 0$ or the constraint is
%satisfied.

% {\em THE FOLLOWING IS ALL OLD.}

% In the pruning learning problem \eqref{eq:pruning_fixederr}, our goal
% is to maximize pruning efficiency subject to the constraint that we
% maintain a desired level of recall. We have two parameters with which
% to optimize our objective: the weights $\mbf{w}$ and the pruning
% function $\theta(x,\cY(x))$. The simplest
% approach, adopted in~\cite{viola01robustreal},
% is to estimate $\bw$ first and then tune $\theta(x,\cY(x))$:
% \begin{packed_enum}
% \item Optimize $\mbf{w}$ to minimize classification loss.
% \item Given $\mbf{w}$, find a pruning threshold function
%   $\theta(\mbf{w},x)$ that relaxes the classification problem until a
%   given recall $(1-\epsilon)$ is achieved.
% \end{packed_enum}

% We propose this approach as a baseline and
% %In the interest of using the simplest possible tools to achieve our
% %goal,
% use the standard structured perceptron algorithm
% ~\cite{collins_discriminative_2002} in step 1 to minimize
% classification loss. The advantages of the perceptron are that it is
% simple and efficient and has shown robust
% performance on sequence learning tasks such as those studied in this
% paper. However, the standard perceptron training is ignorant of the
% goal of pruning and the threshold function, and it does not learn to
% minimize the pruning error in general. In the next section
% %\ref{sec:pruningperceptron},
% we introduce the
% {\em pruning perceptron}, which addresses the goal of pruning more directly.

% \subsection{Mean-max pruning loss}
% In practice, we have the additional constraint that evaluating the
% scores and threshold function must be fast enough that the cumulative
% evaluation time at each level of the cascade results in a net gain in
% efficiency.  Note that the threshold cannot be defined as an absolute
% value, but must depend strongly on $x$ and $\bw$.  We construct our
% threshold from two ingredients to anchor our threshold : the score of
% the best assignment $s^\star_\bw(x) = \max_{y\in\cY(x)}\bw^\top
% \bft(x,y)$ and the mean of the max marginals not pruned by $\cY(x)$,
% denoted by $\bar s^\star_\bw(x)$.
% % = \frac{1}{LK} \sum_{k=1}^K\sum_{n=1}^L s_{\mbf{w}}^\star(x,Y_n=k)$.

% %For instance, a threshold function that relies on sorting
% %the scores of all max marginals before choosing a threshold (e.g.,
% %choosing a fixed proportion or sum-likelihood) will be logarithmically
% %less efficient than a threshold function that can be evaluated in
% %linear time. As the complexity of the cascade grows exponentially,
% %even a sublinear inefficiency will rapidly become intolerable in
% %practice.

% % \begin{figure}
% %   \centering
% %   \input{figs/meanmax}
% %   \caption{\small An illustration of the mean-max pruning threshold
% %     function. The histogram is the distribution of max marginals. The
% %     mean-max threshold (solid red line, center) is scaled by $\alpha$
% %     between the mean and the maximum score (dashed red line,
% %     right). In this case, the score of the truth lies (green, solid)
% %     lies in between; the threshold at $\alpha = 0.5$ (dashed line,
% %     black, center) suffices to prune the majority of max marginals
% %     while preserving the truth.}
% %   \label{fig:meanmax}
% % \end{figure}

% We propose the following ``mean-max'' threshold function (Figure
% \ref{fig:meanmax}), which sets the pruning threshold between the
% max over marginals and the mean for $\alpha \in [0,1]$:
% \begin{equation}
%   \label{eq:meanmax}
%   \theta_{\alpha,\bw}(x,\cY(x)) = (1-\alpha)\bar s^\star_\bw(x) + \alpha s^\star_\bw(x).
% \end{equation}
% The mean-max threshold is computable in linear time. Furthermore, by
% varying $\alpha$ from $0$ to $1$, one can control the trade off
% between pruning efficiency and pruning errors: as $\alpha$ approaches
% $1$, the $\theta_\alpha$ approaches the argmax, and only the argmax
% will survive the threshold. In this case, pruning error is exactly
% classification error. On the other hand, when $\alpha = 0$, only max
% marginals that are equal to or below the mean max marginal across the
% entire sequence will be pruned. If the max marginals are reasonably
% distributed, this mean threshold will prune close to $1/2$ of the
% max-marginals (in practice, we have observed the $\alpha=0$ threshold
% to prune roughly $40\%$). We chose the mean, and not an arbitrary
% scaling between argmin and argmax, precisely to provide this
% approximate minimum efficiency for the cascade, as well as to ensure
% the convexity of our margin constraints below.

% \subsection{Pruning perceptron}
% \label{sec:pruningperceptron}

% It is straightforward to modify the perceptron update to minimize
% pruning errors for a given threshold function $\theta_{\alpha,\bw}$
% instead of classification errors. For the $j$'th example, we define a
% {\em pruning mistake} as a violation of a threshold constraint:
% \begin{equation}
%   \label{eq:pruningmistake}
%   \mbf{w}^\top\mbf{f}(x^j,y^j) \ge \theta_{\alpha,\mbf{w}}(x^j, \cY(x^j)) + 1.
% \end{equation}
% Note that each constraint is convex in $\bw$, since it involves maxima over linear constraints.

% For each mistake, we use the equivalent perceptron update:
% \begin{equation}
%   \label{eq:pruningupdate}
%   \mbf{w}' \leftarrow \mbf{w} + \lambda \mbf{f}(x^j,y^j) -
%   \lambda\left[ (1-\alpha)
%   %\left(
%       \bar\bft_\bw^\star(x^j)
%       %\frac{1}{KL} \sum_{k=1}^K\sum_{n=1}^L \mbf{f}(x,y^\star_{\mbf{w}}(Y_n=k))\right) +
%     +\alpha \bft_\bw^\star(x^j)
%     %\mbf{f}(x,y^\star_{\mbf{w}}(x))
%     \right],
% \end{equation}
% where we have introduced the notation
% $\bft_\bw^\star(x) = \bft(x^j, \argmax_{y\in\cY(x^j)} \bw^\top\bft(x^j,y))$
% and similarly
% $\bar \bft_\bw^\star(x^j)$ is the average of the features of the maximizing assignments
% for each unpruned max-marginal.

% In practice, when we train the pruning perceptron (or the standard
% perceptron) as part of the cascade, we use the previously-trained
% portion of the cascade to prune the output space during training. This
% pruning process is outlined in algorithm \ref{alg:pruning}.
% % $y^\star_{\mbf{w}}(x,Y_n=k) = \argmax_{y:y_n=k}
% % \mbf{w}^\top\mbf{f}(x,y)$ as the maximizing assigments to the argmax
% and the max marginal for $Y_n=k$, respectively.





% This leads to the following definition of forward coefficients
% $\delta$ and backward coefficients $\beta$. To reduce clutter, we
% shorthand for scores over states and transitions, $s_j(x,k) =
% \mbf{w}^\top\mbf{f}(x,Y_j = k)$ and $s_{j,j'}(x,k,k') =
% \mbf{w}^\top\mbf{f}(x,Y_{jj'}) = kk')$:
% \begin{align}
%   \beta_n(k) & = 0, \qquad \beta_j(k) = \max_{k' \in \mcal{V}_{j+1}
%     \cap \mcal{F}_k} \left[ \beta_{j+1}(k') + s_{j+1}(x,k') +
%     s_{j,j+1}(x, k, k') \right] \\
%   \delta_1(k) & = s_1(x, k) + s_{01}(x, \emptyset, k),
%   \quad \delta_j(k)  = s_j(x,t) + \max_{k' \in \mcal{V}_{j-1} \cap \mcal{B}_k} \left[ \delta_{j-1}(k') + s_{j-1,j}(x,k',k) \right]
% \end{align}

%\subsection{The Pruning Perceptron Cascade}

% \begin{algorithm}
%   \caption{Pruning Perceptron cascade training.}
%   \KwIn{Training set $S$, development set $S_D$, error cap $\epsilon$, depth $D$.}

%   \KwInit An empty cascade $C = \{\}$.

%   \For{$d = 1$ \KwTo $(D-1)$}{

%     \ForEach{$\alpha \in \{0, 0.2, 0.4, 0.6, 0.8\}$}{
%         \begin{enumerate}
%         \item Train a pruning perceptron $\mbf{w}^{(d)}$ with parameter $\alpha$ as
%           described in section \ref{sec:pruningperceptron}.
%         \item If the recall of $\mbf{w}^{(d)}$ is less than
%           $(1-\epsilon)$, relax $\alpha \rightarrow 0$ until either
%           $\alpha = 0$ or the recall reaches the minimum level.
%         \end{enumerate}
%       }
%       \KwUpdate $C_d = \ang{\mbf{w}^{(d)}, \alpha}$
%     }
%     \KwRet{The cascade $C$.}


%   \label{alg:pp}
% \end{algorithm}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cascades_aistats2010"
%%% End:


==> text/aistats/sec_theory.tex <==
\section{Generalization Analysis}
\label{sec:theory}

In this section, we give generalization bounds on the filtering and
efficiency loss functions for a single level of a cascade. These bounds depend on Lipschitz dominating
cost functions $\phi_f$ and $\phi_e$ that upper bound $\cL_f$ and
$\cL_e$. To formulate these functions, we define the the scoring
function $\ssp: \mcal{X} \mapsto \reals^m$ where $m=\sum_{c\in\cC} |\cY_c|$ to be the set of scores for all possible clique assignments, $\ssp = \{\bw^\top\bft_c(x,y_c) \mid
c \in \cC, y_c \in \cY_c \}.$ Thus, given $\ssp$, the score
$\score{y}$ can be computed as the inner product $\ang{\ssp, y}$,
where we treat $y$ as a $m$-vector of indicators where $y_i = 1$ if the
$i$'th clique assignment appears in $y$. Finally, we define the
auxiliary function $\phi$ to be the difference between the score of
output $y$ and the threshold as $\phi(y, \theta_x) = \score{y} - \thr$. We now state the main result of this section.


\begin{thm}
  \label{thm:gencascade}
  Let $\ssp$, $\cL_e$, $\cL_f$, and $\phi$ be defined as above. Let
  $\Theta$ be the class of all scoring functions $\sspRV$ with
  $||\bw||_2 \le B$, the total number of cliques $\ell$, and
  $||\bft(x,y_c)||_2 \le 1$ for all $x$ and $y_c$. Define the dominating cost functions $\phi_f(y,\sspRV) =
  r_\gamma(\phi(y,\sspRV))$ and $\phi_e(y,\sspRV) = \frac{1}{m}\sum_{c \in
    \cC, y_c} r_\gamma(\phi(\wit{y_c}, -\sspRV))$, where
  $r_\gamma(\cdot)$ is the ramp function with slope $\gamma$. Then for
  any integer $n$ and any $0 < \delta < 1$ with probability $1-\delta$
  over samples of size $n$, every $\sspRV
  \in \Theta$ and $\alpha \in [0,1]$ satisfies:
  \begin{equation}
    \label{eq:gencascade}
    \begin{split}
      \bbE \left[\cL_f(Y, \sspRV)\right] & \le \hat{\bbE}\left[\phi_f(Y, \sspRV)\right] +
      O\left(\frac{m\sqrt{\ell}B}{\gamma\sqrt{n}}\right) \\
      & \quad + \sqrt{\frac{8 \ln (2/\delta)}{n}},
    \end{split}
  \end{equation}
  where $\hat{\bbE}$ is the empirical expectation with respect to
  training data. Furthermore, \eqref{eq:gencascade} holds with
  $\cL_f$ and $\phi_f$ replaced by $\cL_e$ and $\phi_e$.
\end{thm}
This theorem relies on the general bound given in \cite{BartlettM02}, the properties of Rademacher and Gaussian
complexities (also in \cite{BartlettM02}), and the following lemma:
\begin{lem}
  \label{lem:lipschitz}
  $\phi_f(y,\cdot)$ and $\phi_e(y,\cdot)$ are Lipschitz (with respect
  to Euclidean distance on $\reals^m$) with constant
  $\sqrt{2\ell}/\gamma$.
\end{lem}
A detailed proof of Theorem \ref{thm:gencascade} and Lemma
\ref{lem:lipschitz} is given in the appendix.

Theorem \ref{thm:gencascade} provides theoretical justification for
the definitions of the loss functions $\cL_e$ and $\cL_f$ and the structured cascade objective; if we observe a highly accurate and efficient filtering
model $(\bw,\alpha)$ on a finite sample of training data, it is likely
that the performance of the model on unseen test data will not be too
much worse as $n$ gets large. Theorem
\ref{thm:gencascade} is
%to our knowledge the first application of
%Gaussian complexity bounds to the structured prediction setting. In
%addition, it
the first theoretical guarantee on the
generalization of {\em accuracy} and {\em efficiency} of a structured filtering model.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cascades_aistats2010"
%%% End:


==> text/aistats/sec_theoryproof.tex <==
\appendix

\section{Proof of Theorem \ref{thm:gencascade}}

Assume Lemma \ref{lem:lipschitz} holds (that $\phi_f$ and $\phi_e$ are
Lipschitz with constant $\sqrt{2\ell}/\gamma$) as shown below. We now reproduce the
following four facts from \cite{BartlettM02} that we require to prove the theorem.
\begin{thm}[Bartlett and Mendelson, 2002]
  \label{thm:genbound}
  Consider a loss function $\mathcal{L}$ and a dominating cost
  function $\phi$ such that $\cL(y,x) \le \phi(y,x)$. Let $F:
  \mathcal{X} \mapsto \mathcal{A}$ be a class of functions. Then for
  any integer $n$ and any $0 < \delta < 1$, with probability $1 -
  \delta$ over samples of length $n$, every $f$ in $F$ satisfies
  \begin{equation}
    \label{eq:genbound}
    \begin{split}
      \bbE\cL(Y,f(X)) & \le  \hat{\bbE}_n \phi(Y,f(X)) + R_n(\tilde{\phi} \;\circ\; F)\\
      &\quad  + \sqrt{ \frac{8 \ln(2/\delta)}{n} },
    \end{split}
  \end{equation}
  where $\tilde{\phi} \circ F$ is a centered composition of $\phi$
  with $f \in F$, $\tilde{\phi} \circ f = \phi(y,f(X)) - \phi(y,0)$.

  Furthermore, there are absolute constants $c$ and $C$ such that for
  every class $F$ and every integer $n$,
  \begin{equation}
    \label{eq:rad_to_gaus}
    cR_n(F) \le G_n(F) \le C \ln  n R_n(F).
  \end{equation}
  Let $\cA = \reals^m$ and $F: \cX \to \cA$ be a class of functions
  that is the direct sum of real-valued classes $F_1, \dots,
  F_m$. Then, for every integer $n$ and every sample $(X_1,Y_1), \dots,
  (X_n,Y_n)$,
  \begin{equation}
    \label{eq:multi_gaus}
    \hG_n(\tphi \circ F) \le 2L \sum_{i=1}^m \hG_n(F_i).
  \end{equation}
  Let $F = \{x \mapsto \bw^\top\bft(x,\cdot) \mid ||\bw||_2 \le B,
  ||\bft(x,\cdot)||_2 \le 1\}$. Then,
  \begin{equation}
    \label{eq:lingaus}
    \hat{G}_n(F) \le \frac{2B}{\sqrt{n}}.
  \end{equation}
\end{thm}

% \begin{lem}[Barlett \& Mendelson, 2002]
%   \label{lem:rad_to_gaus}
% \end{lem}
% \begin{thm}[Bartlett \& Mendelson, 2002]
%   \label{thm:multi_gaus}
%   $F: \cX \to \cA$ be a class of functions that is the direct sum
%   of real-valued classes $F_1, \dots, F_m$. Assume that $\tphi: \cY
%   \times \cA \to \reals$ is uniformly bounded, passes through
%   the origin, and Lipschitz (with respect to $\ell_2$ distance on
%   $\cA$) with constant $L$.
% \end{thm}

\begin{proof}[Proof of Theorem \ref{thm:gencascade}]
  Let $\cA = \reals^m$ and $F = \Theta_X$.  By \eqref{eq:rad_to_gaus},
  we have that $R_n(\tphi_f \circ F) = O(G_n(\tphi_f \circ F)).$ Since
  $\tphi$ passes through the origin, then by \eqref{eq:multi_gaus},
  $G_n(\tphi_f \circ F) = O(2L(\tphi_f)\sum_i G_n(f_i)) =
  O(mL(\tphi_f)G_n(\mcal{H}))$. With Lemma \ref{lem:lipschitz} and
  $L(\tphi_f) = L(\phi_f)$, we then have that $R_n(\tphi_f \circ F) =
  O(m\gamma^{-1}\sqrt{l}G_n(F_i))$, where $F_i$ is a linear function
  scoring the $i$'th clique assignment. Thus the results follows from
  \eqref{eq:lingaus} and \eqref{eq:genbound}. Finally, because
  $L(\phi_f) = L(\phi_e)$, the same results applies to $\cL_e$ as
  well.
\end{proof}

\subsection{Proof of Lemma \ref{lem:lipschitz}}

To prove Lemma \ref{lem:lipschitz}, we first bound the slope of the
difference $\phi(y,\ssp)$. We observe that we can consider the scores
of output $y$ as the inner product $\ang{y, \ssp}$, where we treat $y$
as a $m$-vector of indicators and $y_i = 1$ if the $i$'th clique
assignment appears in $y$.
\begin{lem}
  \label{lem:trick}
  Let $f(\ssp) = \ang{y,\ssp} - \max_{y'} \ang{y',\ssp}$. Then $f(u) -
  f(v) \le \sqrt{2\ell} ||u -v||_2.$
\end{lem}
\begin{proof}
  Let $y_u = \argmax_{y'} \ang{y',u}$ and $y_v = \argmax_{y'} \ang{y',
    v}$. Then we have,
  \begin{align*}
    f(u) - f(v) & = \ang{y,u} - \ang{y_u,u} + \ang{y_v,v} - \ang{y,v} \\
    & = \ang{y_v - y,v}  + \ang{y - u_u,u} + \ang{y_v,u} - \ang{y_v,u} \\
    & = \ang{y_v - y, v - u} + \ang{u, y_v - y_u} \\
    & \le \ang{y_v - y, v - u} \\
    & \le ||y_v - y||_2 ||u - v||_2 \le \sqrt{2\ell} ||u-v||_2.
  \end{align*}
  The last two steps follow from the fact that $y_u$ maximizes
  $\ang{y_u,u}$ (so $\ang{u,y_v-y_u}$ is negative), application of
  Cauchy-Schwarz, and from the fact that there are at most $\ell$ cliques appear, each of which can contribute a single non-zero entry in $y$ or $y_v$.
\end{proof}
\begin{lem}
  \label{lem:mmargdiff}
  Let $f'(\ssp) = \ang{y,\ssp} - \frac{1}{m}\sum_{c \in \cC, y_c}
  \max_{y': y'_c = y_c} \ang{y', \ssp}$. Then $f(u) - f(v) \le
  \sqrt{2\ell}||u-v||_2$.
\end{lem}
\begin{proof}
  Let $y_{ui} = \argmax_{y': y'_c = y_c}\ang{y',u}$ for the $i$'th clique
  assignment $y_c$, and $y_{vi}$ the same for $v$. Then we have,
  \begin{align*}
    f'(u)-f'(v) & = \frac{1}{m} \sum_{i=1}^m \ang{y,u} -
    \ang{y_{ui},u} + \ang{y_{vi},v} - \ang{y,v} \\
    & \le \frac{1}{m}\sum_{i=1}^m \ang{y_{vi}-y, v-u} \\
    & \le \frac{1}{m}\sum_{i=1}^m \sqrt{2\ell}||u-v||_2 = \sqrt{2\ell}||u-v||_2.
  \end{align*}
  Here we have condensed the same argument used to prove the previous lemma.
\end{proof}
\begin{lem}
  \label{lem:phidiff}
  Let $g(\ssp) = \ang{y,\ssp} - \thr.$ Then $g(u) - g(v) \le
  \sqrt{2\ell}||u-v||_2$.
\end{lem}
\begin{proof}
  Plugging in the definition of $\thr$, we see that $g(\ssp) =
  \alpha f(\ssp) + (1-\alpha)f'(\ssp)$. Therefore from the previous
  two lemmas we have that $g(u) - g(v) = \alpha( f(u) - f(v) ) +
  (1-\alpha)( f'(u) -f'(v)) \le \sqrt{2\ell}||u-v||_2.$
\end{proof}
From Lemma \ref{lem:phidiff}, we see that $\phi(y,\cdot) = g(\cdot)$ is
Lipschitz with constant $\sqrt{2\ell}$. We can now show that $\phi_f$ and
$\phi_e$ are Lipschitz continuous with constant
$\sqrt{2\ell}/\gamma$. Let $L(\cdot)$ denote the Lipschitz
constant. Then $L(\phi_t)  = L(r_\gamma)\cdot L(\phi(y,\cdot)) \le \sqrt{2\ell}/\gamma.$

To show $L(\phi_e)$ requires more bookkeeping because we must bound
$\phi(\wit{y_c},\ssp)$. We can prove equivalent lemmas to lemmas
\ref{lem:trick}, \ref{lem:mmargdiff} and \ref{lem:phidiff} where we
substitute $\ang{y,\ssp}$ with $\max_{y':y'_c=y_c} \ang{y',\ssp}$, and
thus show that $L(\phi(\wit{y_c},\cdot)) \le \sqrt{2\ell}$. Therefore,
$L(\phi_e) = \frac{1}{m}\sum_{c \in \cC,y_c} L(r_\gamma)\cdot
L(\phi(\wit{y_c}, \cdot)) \le \sqrt{2\ell}/\gamma$, as desired.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cascades_aistats2010"
%%% End:


==> text/cruft.tex <==
% \begin{align}
%   & \mmarg{y_{23} = {\tt le}} = 132.3 \\
%   & \mmarg{y_{23} = {\tt ra}} = 123.4 \\
%   & \mmarg{y_{23} = {\tt fk}} = 75.3
% \end{align}

b


% consistent with the true answer $y^i$ will be filtered.
% We define $\cY_j$ to be the set of
% possible states for the $j$'th variable. The threshold proposed in
% \cite{weiss10} is a ``max mean-max'' function,
% \begin{equation}
%   \label{eq:meanmax}
%   \thr = \alpha \scoremax + (1-\alpha)\frac{1}{\sum_{j=1}^\ell |\cY_j|}\sum_{j=1}^\ell\sum_{y_j \in \cY_j} \mmarg{y_j}.
% \end{equation}

% Filtering max marginals in this fashion can be learned because of the
% ``safe filtering'' property: ensuring that $\scorei{y^i} > \thri$ is
% sufficient (although not necessary) to guarantee that no marginal
% consistent with the true answer $y^i$ will be filtered. Thus, for
% fixed $\alpha$, \cite{weiss10} proposed learning parameters $\theta$
% to maximize the margin $\scorei{y^i}-\thri$ and therefore minimize
% filtering errors:
% \begin{equation}
%   \label{eq:std_sc}
%   \inf_{\theta, \xi\ge 0} \frac{\lambda}{2}||\theta||^2 + \frac{1}{n}\sum_i \xi^i \suchthat \scorei{y^i} \ge \thri + \ell^i - \xi^i, \quad \forall i = 1, \dots, n
% \end{equation}
% Above, $\xi^i$ are slack variables for the margin constraints, and $\ell^i$ is the size of the $i$'th example.

% [From AISTATS]

% For example, a first order Markov sequence model has cliques $\{Y_i,
% Y_{i+1}, X\}$ to score features depending on emissions $\{X,Y_i\}$ and
% transitions $\{Y_i, Y_{i+1}\}$:
% \begin{equation}
% \bw^\top\bft(x,y) = \sum_{i=1}^{\ell} \bw^\top\bft_i(x,y_i,y_{i+1}).
% \end{equation}
% For the first order model, evaluating \eqref{eq:linear_classifiers}
% requires $O(K^2\ell)$ time using the Viterbi decoding algorithm. For
% an order-$d$ Markov model, with cliques over $\{y_i, \dots, y_{i+d},
% x\}$, inference requires $O(k^{d+1}\ell)$ time.

% Several structured prediction methods have been proposed for learning
% $\bw$, such as conditional random fields~\citep{lafferty01crfs},
% structured perceptron~\citep{collins_discriminative_2002}, hidden
% Markov support vector machines~\citep{altun03hmsvm} and max-margin
% Markov networks~\citep{taskar03max}.  Our focus here is instead on
% learning a cascade of increasingly complex models in order to
% efficiently construct models that would otherwise be intractable.

%  (so that the vectors are each in
% the same space). To conclude this section, we extend Theorem
% \ref{thm:gencascade} to provide a generalization bound on the {\em
%   ensemble} filtering loss.  To do so, we first eliminate the
% dependence on $x$ and $\theta$ by rewriting $\cL_{joint}$ in terms of
% the {\em scores} of every possible state assignment, $\theta \cdot
% \bft(x,y_j)$, according to each sub-model. Let the vector $\ssp \in
% \reals^{mP}$ denote these scores, where $m$ is the number of possible
% state assignments in the sub-models.

We prove the theorem by applying the following result from \cite{bartlettM02}:
\begin{thm}[Bartlett and Mendelson, 2002]
  \label{thm:genbound}
  Consider a loss function $\mathcal{L}$ and a dominating cost
  function $\phi$ such that $\cL(y,x) \le \phi(y,x)$. Let $F:
  \mathcal{X} \mapsto \mathcal{A}$ be a class of functions. Then for
  any integer $n$ and any $0 < \delta < 1$, with probability $1 -
  \delta$ over samples of length $n$, every $f$ in $F$ satisfies
  \begin{equation}
    \label{eq:genbound}
      \bbE\cL(Y,f(X)) \le  \hat{\bbE}_n \phi(Y,f(X)) + R_n(\tilde{\phi} \;\circ\; F) + \sqrt{ \frac{8 \ln(2/\delta)}{n} },
  \end{equation}
  where $\tilde{\phi} \circ F$ is a centered composition of $\phi$
  with $f \in F$, $\tilde{\phi} \circ f = \phi(y,f(X)) - \phi(y,0)$.

  Furthermore, there are absolute constants $c$ and $C$ such that for
  every class $F$ and every integer $n$,
  \begin{equation}
    \label{eq:rad_to_gaus}
    cR_n(F) \le G_n(F) \le C \ln  n R_n(F).
  \end{equation}
  Let $\cA = \reals^m$ and $F: \cX \to \cA$ be a class of functions
  that is the direct sum of real-valued classes $F_1, \dots,
  F_m$. Then, for every integer $n$ and every sample $(X_1,Y_1), \dots,
  (X_n,Y_n)$,
  \begin{equation}
    \label{eq:multi_gaus}
    \hG_n(\tphi \circ F) \le 2L \sum_{i=1}^m \hG_n(F_i).
  \end{equation}
  Let $F = \{x \mapsto \bw^\top\bft(x,\cdot) \mid ||\bw||_2 \le B,
  ||\bft(x,\cdot)||_2 \le 1\}$. Then,
  \begin{equation}
    \label{eq:lingaus}
    \hat{G}_n(F) \le \frac{2B}{\sqrt{n}}.
  \end{equation}
\end{thm}




$$\max_{y_1,y_2} \sum_{j=1}^2 \score{y_j} + \score{y_{{j-1},j}}$$
$$\score{y_{2,3}}$$
$$\max_{y_3, \dots, y_\ell} \sum_{j=3}^\ell \score{y_j} + \score{y_{j,j+1}}$$



% \subsection{Cascaded inference with max-marginals}

% We will discuss how to learn a cascade of models in Section 4, but
% first we describe the inference procedure.  The basic notion behind
% our approach is very simple: at each level of the cascade, we receive
% as input a set of possible clique assignments corresponding to the
% cliques of the current level. Each level further filters this set of
% clique assignments and generates a set of possible clique assignments
% which are passed as input to the next level. Note that each level is
% able to prune further than the preceding level because it can consider
% higher-order interactions. At the end of the cascade, the most complex
% model chooses a single prediction as usual, but it needs only consider
% the clique assignments that have not already been pruned. Finally,
% pruning is done using clique max-marginals, for reasons which we
% describe later in this section.

% An example of a cascade for sequential prediction using Markov models
% is shown is Figure \ref{fig:schematic}. A $d$-order Markov model has
% maximal cliques $\{X, Y_i, Y_{i+1}, \dots, Y_{i+d}\}$. We can consider
% a cascade of sequence models of increasing order as a set of bigram
% models where the state space is increasing exponentially by a factor
% of $K$ from one model to the next.  Given a list of valid assignments
% $\cV^i$ in a $d$-order model, we can generate an expanded list of
% valid assignments $\cV^{i+1}$ for a $(d+1)$-order model by
% concatenating the valid $d$-grams with all possible additional states.

% More generally, for a given input $x$, for each maximal clique $c\in
% \cC$ in the current level of the cascade, we have a list of valid
% assignments $\cV_c \subseteq \cY_c$. Inference is performed only over
% the set of valid clique assignments $\cV = \bigcup_{c \in \cC}
% \cV_c$. Using the filtering model $\bw$ of the current cascade level,
% the clique assignments in $\cV_c$ are scored by their max-marginals,
% and a threshold $t$ is chosen to prune any $y_c \in \cV_c$ with a
% score less than the threshold. The sets $\cV$ are then passed to the
% next level of the cascade, where higher-order cliques consistent with
% unpruned cliques are constructed. If we can eliminate at least a
% fraction of the entries in $\cV$ on each round of the cascade, then
% $|\cV|$ decreases exponentially fast and the overall efficiency of
% inference is controlled.

% Thus, to define the cascade, we need to define: (1) the set of models
% to use in the cascade, and (2) a procedure to choose a threshold
% $t$. In the remainder of this section we discuss our approach to these
% decisions.

% First, to define a set of models for the cascade, we require only that
% the sets of cliques of the models form a nesting sequence. The cliques
% of the models must satisfy the relation,
% \begin{equation}
%   \label{eq:nested}
%   \cC^1 \subseteq \cC^2 \subseteq \dots \subseteq \cC^d,
% \end{equation}
% where $\cC^i$ is the set of cliques of the $i$'th model of the
% cascade. In other words, every clique assignment $y_c$ of the $i$'th
% model is contained in at least one clique assignment $y_c'$ of the
% $(i+1)$'th model. This property allows for the use of increasingly
% complex models as the depth of the cascade increases. As long as
% \eqref{eq:nested} holds, a simple and intuitive mapping from the set
% of valid cliques of the $i$'th model $\cV^i$ to a corresponding set of
% valid cliques of the $(i+1)$'th model, $\cV^i$:
% \begin{equation}
%   \label{eq:cliquemapping}
%   \cV^{i+1}_c = \{ y_c \in \cY_c \mid \forall c' \in \cC^i, c' \subseteq c, y_{c'} \in \cV_{c'}^i\}
% \end{equation}
% This is the set of clique assignments $y_c$ in the $(i+1)$'th model
% for which all consistent clique assignments $y_{c'}$ for subcliques
% $c' \in \cC^i$ have not been pruned by the $i$'th
% model.

% In order to filter clique assignments, we use their
% \textit{max-marginals}.  We introduce the shorthand $\score{y} =
% \bw^\top\bft(x,y)$ for the cumulative score of an output $y$, and
% define the max marginal $\mmarg{y_c}$ as follows:
% $$\mmarg{y_c} \triangleq \max_{y'\in \cY} \;\;\{ \score{y'} : y'_c = y_c\}.$$
% Computing max-marginals can be achieved using the same dynamic
% programming inference procedures in factor graphs as would be used to
% evaluate \eqref{eq:linear_classifiers}. Most importantly, max
% marginals satisfy the following simple property:
% Lemma \ref{prop:pruning} states that if the score of the true label
% $y$ is greater than the max marginal of a clique assignment $y'_c$,
% then that clique assignment $y'_c$ must be inconsistent with the truth
% $y$. The lemma follows from the fact that the max marginal of any
% clique assignment $y_c$ consistent with $y$ is at least the score of
% $y$.


In this work, we tackle the problem of learning a structured cascade
for problems in which inference is {\em intractable}, but in which the
large node state-space has a natural hierarchy that can be
exploited. For example, such hierarchies arise in pose estimation by
discretizing the articulation of joints at multiple resolutions, or in
image segmentation due to the semantic relationship between class
labels (e.g., ``grass'' and ``tree'' can be grouped as ``plants,''
``horse'' and ``cow'' can be grouped as ``animal.'')

\out{
We then define the joint marginal the ensembles consists
of repeating tree models over $P$ variables, where the $p$'th model
incorporates persistence of the $p$'th variable through time. We learn
a filter over the ensemble jointly by summing the max marginals of
each model, and we compute a filtering threshold on the summed max
marginals. Then 
The advantage of summing the marginals in this manner is that a
weakness in one member of the ensemble on a particular example can be
compensated for by the strengths of the other models. Although one or
more of the individual scores $\pscore{y^i}$ may be under threshold
$\pthri$, the ensemble can still avoid a mistake if another member
scores $y^i$ high enough to compensate. On the PATV problem, this may
occur if the model part with the strongest visual cues for continuity
through time varies from example to example; e.g., in scenes where the
actor faces the camera, modeling a smooth face trajectory is useful,
while if the face is obscured or the actor is facing away from camera,
modeling a smooth arm trajectory may be more accurate. In fact, we
find experimentally (section \ref{sec:results}) that persistence of
certain variables is much more helpful than others. Note that an
alternative to \eqref{eq:joint_sc} using the original SC framework
would be to simply learn a cascade of $P$ models, but in that
approach, mistakes are cumulative, and there is no way for any model
to compensate for the weaknesses of the others.}




\subsection{Part-of-Speech Tagging}

We next evaluated our approach on several part of speech (POS) tagging
tasks. Our objective was to rigorously compare the efficacy of our
approach to alternative methods on a problem while reproducing
well-established benchmark prediction accuracy. The goal of POS
tagging is to assign a label to each word in a sentence. We used three
different languages in our experiments: English, Portuguese and
Bulgarian. For English, we used volumes 0-17 of the Wall Street
Journal portion of the Penn TreeBank~\citep{PennTreebank} for
training, volumes 18-20 for development, and volumes 21-24 for
testing. We used the Bulgarian BulTreeBank~\citep{Simov02buildinga}
and the Bosque subset of the Portuguese Floresta
Sinta(c)tica~\citep{floresta}
%\footnote{http://www.linguateca.pt/Floresta/}
for Bulgarian and Portuguese datasets, respectively.

For these experiments, we focused on comparing the efficiency of our
approach to the efficiency of several alternative approaches. We again
used a set of Markov models of increasing order; however, to increase
filtering efficiency, we computed max marginals over subcliques
representing $(d-1)$ order state assignments rather than $d$-order
cliques representing transitions. Thus, the bigram model filters
unigrams and the trigram model filters bigrams, etc. Although we ran
the cascades up to 5-gram models, peak accuracy was reached with
trigrams on the POS task.

We compared our SC method to two baselines: the standard structured
perceptron (SP) and a maximum a posteriori CRF. All methods used the
same standard set of binary features: namely, a feature each
(word,tag) pair $\ind{X_t = x_t, Y_t = y_t}$ and feature for each
$d$-gram in the model. For the baseline methods, we trained to
minimize classification error (for SP) or log-loss (for CRF) and then
chose $\alpha \in [0,1]$ to achieve minimum $\cL_e$ subject to $\cL_f
\le \epsilon$ on the development set. For the CRF, we computed
sum-product marginals $P(y_c|x) = \sum_{y': y'_c = y_c} P(y'|x)$, and
used the threshold $\thr = \alpha$ to eliminate all $y_c$ such that
$P(y_c|x) \le \alpha$. For all algorithms, we used grid search over
several values of $\eta$ and $\lambda$, in addition to early stopping,
to choose the optimal $\bw$ based on the development set.  For
SC training, we considered initial $\alpha$'s from the candidate set
$\{0, 0.2, 0.4, 0.6, 0.8\}$.

We first evaluated our approach on the WSJ dataset.  \out{We took the
  optimal $\bw$ over $\eta \in \{1.0, 0.1, 0.001, 0.0001\}$, selecting
  on the development set.} To ensure accuracy of the final predictor,
we set a strict threshold of $\epsilon = 0.01$\%. All methods were
trained using a structured perceptron for the final classifier. The
results are summarized in Table \ref{tab:fullwsj}. SC was compared to
CRF, an unfiltered SP model (Full), and a heuristic baseline in which
only POS tags associated with a given word in the training set were
searched during inference (Tags). SC was two orders of magnitude
faster than the full model in practice, with the search space reduced
to only $\approx 4$ states per position in inference (roughly the
complexity of a greedy approximate beam search with 4 beams.)  SC
also outperformed CRF by a factor of 2.6 and the heuristic by a factor
of 6.8. Note that because of the trade-off between accuracy and
efficiency, CRF suffered less filter loss relative to SC due to
pruning less aggressively, although neither method suffered enough
filtering loss to affect the accuracy of the final
classifier. Finally, training the full trigram POS tagger with exact
inference is extremely slow and took several days to train; training
the SC cascade took only a few hours, despite the fact that more
models were trained in total.

% \begin{table}

%   \centering
%   {\small
%   \begin{tabular}{|l|cccc|}
%     \hline {\bf Model:} & {\bf Full} & {\bf SC} & {\bf CRF} & {\bf Tags} \\
%     \hline
%     Accuracy (\%) & 96.83 & 96.82& 96.84 & --- \\
%     Filter loss (\%) & 0& 0.121 & {\bf 0.024} & 0.118 \\
%     Test Time (ms) & 173.28 & {\bf 1.56} & 4.16 & 10.6 \\
%     Avg. Num States & 1935.7 & {\bf 3.93} & 11.845 & 95.39 \\
%     \hline
%   \end{tabular}}
% \caption{\small Summary of WSJ Results.
%   Accuracy is the accuracy of the final trigram model.
%   Filter loss is the number of incorrectly pruned bigrams at the end of the cascade.
%   The last row is the average number of states considered at each position in the test set.}
%   \label{tab:fullwsj}
% \end{table}

We next investigated the efficiency vs. filtering accuracy trade-off
of SC compared to the SP and CRF baselines on all three
languages. For each of the three languages, we generated 10 different
training sets from 40\% of the full training datasets. Randomization
was taken with the same 10 seeds for each dataset/algorithm pair. For
all methods, we trained bigram models under two conditions: first, as
the initial step of a cascade (e.g., no prior filtering), and second,
as the second step of a cascade after initial filtering by the SC
algorithm with $\epsilon = 0.05$\%, and analyzed the resulting
trade-off between efficiency and accuracy.

The results are presented in Figure \ref{fig:tradeoff}. The figures
were generated by computing for each $\epsilon$ along the x-axis the
corresponding {\em test} efficiency $\cL_e$ when the constraint on
filter loss ($\cL_f \le \epsilon$) is enforced using {\em development}
set data. Points for which the constraint could not be enforced (even
with $\alpha=0$) are not shown. SC handily beats the competitors in
both the filtered and unfiltered case. Note that in the unfiltered
condition, the CRF is unable to achieve significant pruning efficiency
for any $\epsilon$, while the SP cannot achieve filtering accuracy for
small $\epsilon$. However, because SC and SP become equivalent as
$\alpha$ approaches 1, we observe that the performance
of SC and SP converge as $\epsilon$ increases.




==> text/eccv/abstract.tex <==
abstract here


==> text/eccv/commands.tex <==
%% specific commands

%kronecker features
\newcommand{\Kbar}{\mathbf{\bar{K}}}
\newcommand{\ybar}{\mathbf{\bar{y}}}
\newcommand{\xbar}{\mathbf{\bar{x}}}
\newcommand{\xBar}{\mathbf{\bar{\bar{x}}}}

\newcommand{\Loss}{\mathcal{L}}
\newcommand{\LossZO}{\mathcal{L}_{01}}
\newcommand{\LossM}{\mathcal{L}_{\psi}}
\newcommand{\LossA}{\mathcal{L}_{\psi}}
\newcommand{\LossMAX}{\mathcal{L}^{max}_{\psi}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bft}{\mathbf{f}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\ip}[2]{{#1}\cdot{#2}}
\newcommand{\Rgn}{\mathcal{R}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\Y}{\mathcal{Y}}

\newcommand{\Ind}{\mathbf{1}}
\newcommand{\argmax}{\mathop{\arg\max}}

\newcommand{\Vones}[1]{\ensuremath{\mathbf{1}_{#1}}}
\newcommand{\eqdef}{\stackrel{\rm def}{=}}

\newcommand{\out}[1]{}
\newcommand{\denselist}{\itemsep 0pt\topsep-8pt\partopsep-8pt}
\newcommand{\mypar}[1]{\noindent{\bf #1:}}
\newcommand{\myparnoc}[1]{\noindent{\bf #1}}
\newcommand{\myparnobf}[1]{\noindent{ #1:}}

\newcommand{\deriv}[2]{ \frac{\partial #1}{\partial #2} }
\newcommand{\diag}{ \mathbf{diag} }

%% paper-specific definitions:
\newcommand{\lparts}{l}
\newcommand{\lpart}{l}
\newcommand{\Lpart}{L}
\newcommand{\Lparts}{L}
\newcommand{\Lspace}{\mathcal{L}}
\newcommand{\abin}{\mathbf{bin}_{uv}}
\newcommand{\dregion}{\mathbf{d}_{region}}
\newcommand{\dcontour}{\mathbf{d}_{contour}}
\newcommand{\setrank}{\textbf{rank}}
\newcommand{\cascade}{\mathcal{C}}
\newcommand{\tree}{\Upsilon}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\renewcommand{\algorithmiccomment}[1]{\; // #1}


\newcommand{\mmi}{\theta_x^\star(\lpart_i)}

%\renewcommand{\includegraphics}[2]{}

%% usual commands
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
%\newcommand{\todo}[1]{{\bf{TODO: #1}}}
%\newcommand{\todo}[1]{}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}

%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{definition}[1][Definition]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{example}[1][Example]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{remark}[1][Remark]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

%\newcommand{\qed}{\nobreak \ifvmode \relax \else
%      \ifdim\lastskip<1.5em \hskip-\lastskip
%      \hskip1.5em plus0em minus0.5em \fi \nobreak
%      \vrule height0.75em width0.5em depth0.25em\fi}

%\newcommand{\qed}{\hfill \ensuremath{\Box}}

%\newcommand{\qed}{\ensuremath{\Box}}

\newcommand{\boxedequation}[2]{%
  \[\fbox{
      \addtolength{\textwidth}{-2\fboxsep}%
      %\addtolength{\linewidth}{-2\fboxsep}%
      \addtolength{\linewidth}{-2\fboxrule}%
      \begin{minipage}{#1\linewidth}%
      \begin{equation}#2\end{equation}%
      \end{minipage}%
    }\]%
}
\newcommand{\boxedeqnarray}[1]{%
  \[\fbox{%
      %\addtolength{\linewidth}{-2\fboxsep}%
      %\addtolength{\linewidth}{-2\fboxrule}%
      \begin{minipage}{0.7\linewidth}%
      \begin{eqnarray*}#1\end{eqnarray*}%
      \end{minipage}\nonumber%
    }\]%
}

%abbreviations
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g.}}
%\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
%\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}

%\def\ie{\emph{i.e.}}
%\makeatother



%% specific commands
\newcommand{\trans}[1]{{#1}^{\ensuremath{\mathsf{T}}}}           % transpose
\newcommand{\st}{\quad\textrm{s.t.}\quad}                        % s.t. for such that
\newcommand{\mvec}{\textrm{vec}}
\newcommand{\nchoosek}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}  %use binom instead...


==> text/eccv/experiments.tex <==
\section{Experiments}\label{experiments_sec}
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.98\textwidth]{data/results_all.pdf}
\end{center}
\caption{\label{res_all_img}Examples of correctly localized limbs under different conditions (low contrast, clutter) and poses (different positions of the arms, partial self occlusions). }
\vspace{-0.4cm}
\end{figure}
We evaluate our approach on the publicly available Buffy The Vampire Slayer v2.1 and PASCAL Stickmen datasets~\cite{eichner09}.  We use the upper body detection windows provided with the dataset as input to localize and scale normalize the images before running our experiments as in~\cite{eichner09,ferrari08,andriluka09}.  We use the usual 235 Buffy test images for testing as well as the 360 detected people from PASCAL stickmen.  We use the remaining 513 images from Buffy for training and validation. 
%The 235 test images were selected because upper bodies were correctly localized using a detector from~\cite{ferrari08}, from which we can crop and normalize the input to our models.  For the training set we hand-annotate similar upper-body boxes.

\myparnoc{Evaluation Measures}  The typical measure of performance on this dataset is a matching criteria based on both endpoints of each part (e.g., matching the elbow and the wrist correctly): A limb guess is correct if the limb endpoints are on average within $r$ of the corresponding groundtruth segments, where $r$ is a fraction of the groundtruth part length.  By varying $r$, a performance curve is produced where the performance is measured in the percentage of correct parts (PCP) matched with respect to $r$.  %We define PCP$_r$ as the value of the curve at $r$.  Previous work~\cite{ferrari08,posesearch,andriluka09,eichner09} have compared PCP$_{0.5}$ values, a fairly loose matching criteria.

%For comparison to previous work, we also report PCP values, using the publicly available function to compute it.  
%The PCP metric is somewhat unsatisfying because it is non-continuous and confounds part length estimation error with joint and angle estimation error.  
%None of the methods reporting results on this dataset (~\cite{ferrari08,posesearch,andriluka09,eichner09}) actually model part length as part of their state space (including us), and each resorts to some post-hoc method of guessing the non-joint endpoint given the output of their pictorial structure model.  We use the simplest approach of assuming each part has a fixed length in every image.  Changing this length parameter can change PCP results significantly.  
%We propose a new evaluation criteria which we use for some of our experimental analysis: normalized $L_2$ distance to the groundtruth state: let
\out{
{\footnotesize
\[
\hat{\lpart_i} =
\left[ {\begin{array}{c}
 \lpart_{ix}/ \max \Lspace_{ix} \;\; \lpart_{iy}/\max \Lspace_{iy}  \;\; |\tan^{-1}(\lpart_{iv},\lpart_{iu})|/\pi \\
 \end{array} } \right]^T
\]
}

be a normalized 3 dimensional state-space representation with each component is in the range $[0,1]$.  For a similarly normalized groundtruth part $\hat{\lpart_i}^{gt} $, we report normalized $L_2$ distance $|| \hat{\lpart_i} - \hat{\lpart_i}^{gt}||_2$, and analogously defined normalized root-mean-squared error (RMSE).  This measure is invariant to image dimensions and angle quantization, is continuous, and directly measures what we model in our state representation.
}

\begin{figure}[t]
\centering
\includegraphics[width=0.3\textwidth, height = 3.3cm]{data/CPS_vs_baseline_PCP.pdf}\quad
\includegraphics[width=0.34\textwidth, height = 3.4cm]{data/feature_analysis.png}
% \includegraphics[width=0.23\textwidth]{data/CPS_vs_baseline_PCP.pdf}\\
% \includegraphics[width=0.3\textwidth]{data/feature_analysis.png}
\caption{\label{fig:overall} \textbf{Left:} PCP curves of our cascade method versus a detection pruning approach, evaluated using PCP on arm parts (see text).  \textbf{Right:} Analysis of incorporating individual types of features into the last stage of our system. }
\end{figure}

%\begin{figure}[t]
%\centering
%\subfigure[ ]{
%%\includegraphics[width=0.3\textwidth, height = 3.2cm]{data/CPS_vs_baseline_PCP.pdf}
%%\includegraphics[width=0.3\textwidth, height = 3.2cm]{data/feature_analysis.png}
%% \includegraphics[width=0.23\textwidth]{data/CPS_vs_baseline_PCP.pdf}
%% \includegraphics[width=0.3\textwidth]{data/feature_analysis.png} 
%\includegraphics[width=0.23\textwidth]{data/results_fig_all.pdf}
%\label{fig:overall}
%}
%\subtable[ ]{
%{\scriptsize
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%method &	torso &	head	 &	upper	 &	lower	 &	total \\
% &	&		 &	arms	 &	arms	 &	\\
%\hline\hline
%Ferrari et al.~2008~\cite{ferrari08}	 &	-	 &	-	 &	-	 &	-   &	 61.4\% \\
%\hline
%Ferrari et al.~2009~\cite{posesearch}	 &	-	 &	-	 &	-	 &	-		 &	74.5\% \\
%\hline
%Andriluka et al.~\cite{andriluka09}	 &	90.7\%	 &	95.5\%	 &	79.3\%	 &	41.2\%	 &		73.5\% \\
%\hline
%Eichner et al.~\cite{eichner09}		 &	98.7\% 	 &		97.9\%		 &	82.8\%	& 59.8\%	 &	80.1\% \\
%\hline
%APS~\cite{sapp2010}	&	100\%		 &	100\%		 &	91.1\% &		65.7\%	 &	85.9\% \\
%\hline
%CPS (ours)	&	100\%	&	96.2\%	&	95.3\%	&	63.0\%	& 	85.5\% \\
%\hline
%0th order baseline&		99.6\%	&	87.3\%&		90.0\%	&	55.3\% 	&		79.6\% \\
%\hline\hline						
%Eichner et al.~\cite{eichner09}		&	98.72\%	&	97.87\%	&	82.8\%	&	59.79\%		&	80.1\% \\
%\hline
%APS~\cite{sapp2010}	&	100\%	&	-	&	83.9\%	&	54.0\%		&	79.0\% \\
%\hline
%CPS (ours)	&	100\%	&	-	&	87.1\%	&	49.4\%		&	77.2 \%\\
%\hline
%\end{tabular}
%}

%}
%\caption{\textbf{Left:} PCP curves of our cascade method versus a detection pruning approach, evaluated using PCP on arm parts (see text).  \textbf{Right:} Analysis of incorporating individual types of features into the last stage of our system. }
%\end{figure}



\myparnoc{Overall system performance}
As shown in Table~\ref{tab:overall}, we perform comparably with the state-of-the-art on all parts, improving over~\cite{sapp2010} on upper arms on both datasets and significantly outperforming earlier work.  We also compare to a much simpler approach, inspired by~\cite{pff-cascade} (detector pruning + rich features):  We prune by thresholding each unary detection map individually to obtain the same number of states as in our final cascade level, and then apply our final model with rich features on these states. As can be seen in Figure~\ref{fig:overall}/left, this baseline performs significantly worse than our method (performing about as well as a standard PS model as reported in~\cite{sapp2010}).  This makes a strong case for using max-marginals (e.g., a global image-dependent quantity) for pruning, as well as learning how to prune safely and efficiently, rather than using static thresholds on individual part scores as in~\cite{pff-cascade}.

Our previous method~\cite{sapp2010} is the only other PS method which incorporates image information into the pairwise term of the model.  However it is still an exhaustive inference method.  Assuming all features have been pre-computed, inference in~\cite{sapp2010} takes an average of 3.2 seconds, whereas inference using the sparse set of states in the final stage of the cascade takes on average 0.285 seconds---a speedup of 11.2x\footnote{Run on an Intel Xeon E5450 3.00GHz CPU with an $80\times80\times24$ state space averaged over 20 trials.~\cite{sapp2010} uses MATLAB's optimized fft function for message passing.}.

%In Figure~\ref{fig:overall}, left, we plot the whole PCP curve and compare against the curves provided by the authors~\cite{ferrari08,posesearch,eichner09}. We show detection examples in Fig.~\ref{res_all_img}. Due to lack of space, more results are included in the supplemental material.
% We first begin comparing our overall system results to other results on this dataset.  In the next 2 sections we will analyze the quality of the different components of the system, but the overall system performance indicates that we have not lost too many correct hypotheses during pruning, and our ability to include richer features to solve the problem is very effective.  Table~\ref{tab:overall} compares our end-to-end system with other reported results, at the PCP$_{0.5}$ evaluation point.  We significantly outperform the state-of-the-art on the more challenging parts: upper and lower arms, and perform comparably on the saturated-performance parts head and torso.  In Figure~\ref{fig:overall} we plot the whole PCP curve and compare against the curves provided by the authors~\cite{ferrari08,posesearch,eichner09}.
%\begin{table}[t]
%\begin{center}
%{\scriptsize
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%method  & torso & head  & upper arms & lower arms & total\\
%\hline\hline
%Ferrari et al.~2008~\cite{ferrari08}	& -	& -	& -	& -	& $61.4\%$\\
%\hline
%Ferrari et al.~2009~\cite{posesearch}	&-	&-	&-	&-	&$74.5\%$\\
%\hline
%Andriluka et al.~\cite{andriluka09}	&$90.7\%$	&$95.5\%$	&$79.3\%$	 &$41.2\%$	&$73.5\%$\\
%\hline
%Eichner et al.~\cite{eichner09}	&$98.72\%$	&$\mathbf{97.87\%}$	 &$82.8\%$	&$59.79\%$	&$80.1\%$ \\
%\hline
%CPS (ours)	&$\mathbf{100\%}$	&$97.4\%$	&$\mathbf{96.6\%}$	 &$\mathbf{62.3\%}$	&$\mathbf{86.2\%}$ \\
%\hline
%\end{tabular}
%}
%\caption{\label{tab:overall} Comparison to other methods at PCP$_{0.5}$}
%\end{center}
%\end{table}
%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=0.4\textwidth, height = 3.8cm]{data/sparse_ps_vs_ferrari.png}
%\includegraphics[width=0.4\textwidth, height = 3.8cm]{data/feature_analysis.png}
%\end{center}
%\caption{\label{fig:overall} \textbf{Left:} PCP curves of our cascade method versus~\cite{ferrari08,posesearch,eichner09}.  \textbf{Right:} Analysis of incorporating individual types of features into the last stage of our system. }
%\end{figure}

% \subsubsection*{Feature analysis}
\input{text/results_table}

%\input{text/results_all}

In Figure~\ref{fig:overall}/right  we analyze which features are most effective, measured in $L_2$ distance to the groundtruth state, normalized by the groundtruth length of the part.  We start only with the basic geometry and unary HoG detector features available to basic PS systems, and add different classes of features individually.  Skin/torso color estimation gives a strong boost in performance, which is consistent with the large performance boost that the results in~\cite{eichner09} obtained over their previous results~\cite{posesearch}. Using contours instead of color is nearly as effective.  The features combine to outperform any individual feature. Examples where different cues help are shown in Figure~\ref{res_feat}.
%\begin{table}[t]
%\begin{center}
%{\footnotesize
%\begin{tabular}{|c|c|c|c|r|c|}
%\hline
%cascade  & max state size & average states  & search space & \multicolumn{2}{| l |}{RMSE of oracle}\\
%\cline{5 - 6}
%level & $l_x\times l_y \times l_{\theta} $ & per part & reduction & {\scriptsize all$\times 10^2$ }& {\scriptsize arms$\times 10^2$}\\
%\hline\hline
%1	& $10\times 10\times12$ & 31626	& $92.8\%$ & 5.14 & 5.06\\
%\hline
%2	 & $10\times 10\times24$ & 14776	& $95.5\%$ & 5.66 & 5.82\\
%\hline
%3	 & $40\times 40\times24$ & 4191	& $98.7\%$ & 6.41 & 6.81\\
%\hline
%4	 & $80\times 80\times24$ & 882 	& $99.7\%$ & 6.92 & 7.45\\
%\hline
%5	 & $110\times 122\times24$ & 703 	& $99.8\%$ &  7.24 & 7.89\\
%\hline\hline
%detector pruning  & $110\times 122\times24$ & 703 & $99.8\%$ & 8.23 & 9.03\\
%\hline
%\end{tabular}
%}
%\caption{\label{tab:c2f} For each level of the cascade as well as the $0^\textrm{th}$-order pruning, we present the reduction of the size of the state space we search in and the quality of the retained hypotheses measured by the normalized RMSE score. As a baseline, we compare to pruning the same number of states in the HoG detection map, which yields a relative increase in error of 14.4\% in the arm parts.}
%\end{center}
%\end{table}

\input{text/pruning_results}

\mypar{Coarse-to-fine Cascade Evaluation}
In Table~\ref{tab:pruning}, we evaluate the drop in performance of our system after each successive stage of pruning.  
%In the early stages, the state space is too coarse for the MAP state sequence of one of the pruning models to be meaningfully compared to the fine-resolution groundtruth, so
We report PCP scores of the best possible as-yet unpruned state left in the original space.  We choose a tight PCP$_{0.2}$ threshold to get an accurate understanding whether we have lost well-localized limbs.  As seen in Table~\ref{tab:pruning}, the drop in PCP$_{0.2}$ is small and linear, whereas the pruning of the state space is exponential---half of the states are pruned in the first stage.  %Note that the first level of the cascade can make many easy pruning decisions, for example, the left elbow cannot be in the upper or lower right portions of the state space, the left shoulder cannot be on the right side, and the possible head and torso angles can be drastically cut down.  
As a baseline, we evaluate the simple detector-based pruning described above.  This leads to a significant loss of correct hypotheses, to which we attribute the poor end-system performance of this baseline (in Figure~\ref{fig:overall} and Table~\ref{tab:overall}), even after adding richer features.
%shold on HoG detection maps individually for each part, and sample the same number of states that we end up with at the end of the cascade.  The RMSE is higher, with a relative increase in error in the arm parts of 14.4\%.

\mypar{Future work} The addition of more powerful shape-based features could further improve performance.  Additional levels of pruning could allow for (1) faster inference, (2) inferring with higher-order cliques to, e.g., express compatability between left and right arms or (3) incorporating additional variables into the state space---relative scale of parts to model foreshortening, or occlusion variables.  Finally, our approach can be naturally extended to pose estimation in video where the cascaded models can be coarsened over space and time.  
 
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.90\textwidth]{data/results_features2.pdf}
\vspace{-0.5cm}
\end{center}
\caption{\label{res_feat} Detections with geometry (top) and with additional cues (bottom). Left: contour features support arms along strong contours and avoid false positives along weak edges. Right: after overlaying the part hypothesis on the segmentation, the incorrect one does not select an elongated set of segments.}
\vskip -0.2in
\end{figure}



==> text/eccv/features.tex <==
\section{Features}\label{sec:features}

% The nodes of the PS denote body parts. The state $s_i=[s_{ix}, s_{iy}, s_{iu}, s_{iv}]$ of each part $L_i$ is defined as the joint location $(s_{ix}, s_{iy})$ of the part in image coordinates together with its orientation, which is encoded as a unit vector $(s_{iu}, s_{iv})$. Furthermore, each body part has a predefined length $l_i$ and width $w_i$, which can be used to define the support of the part, as the rectangle of size $(l_i, w_i)$ starting at the joint and orientated along the part orientation.

\out{
\begin{table}[b]
\begin{center}
{\footnotesize
\begin{floatingtable}[lb]{
\begin{tabular}{|l  |l  |l  |l  |l  |}
\hline
Feature & Class & Part & Cliques & \# \\
\hline\hline
texture (HoG) & appearance &  all & unary & 1 \\
\hline
color models & appearance & arms only & unary & 2 \\
\hline
color similarity & appearance & arms only & pairwise & 1\\
\hline
%$f_5$ & embedding distances & appearance & pairwise & 1\\
%\hline
absolute location &geometry & all & unary & 4 \\
\hline
relative location & geometry& all & pairwise & 10 \\
\hline
contours & shape & arms only & pairwise & 18 \\
\hline
regions & shape & arms only & unary & 7 \\
\hline
\end{tabular}}
\caption{\label{feat_table} A summary of the features. See text for details.}
\end{floatingtable} }
}

The introduced \modelname{} model allows us to capture appearance, geometry and shape information of parts and pairs of parts in the final level of the cascade---much richer than the standard geometric deformation costs and texture filters of previous PS models~\cite{felz05,devacrf,ferrari08,andriluka09}.  
%Table~\ref{feat_table} lists all features that we use and will describe in this section.  
Each part is modeled as a rectangle anchored at the part joint with the major axis defined as the line segment between the joints (see Figure~\ref{fig:ps}).  For training and evaluation, our datasets have been annotated only with this part axis.

%The side of a part is defined as the longer side of part rectangle.  
%Further, the major axis of a part is the line segment starting at the part joint parallel to the part side.

%In the following, we will use the support of each part $l_i$ in the image defined as a rectangle anchored at the part joint position position $(l_{ix}, l_{iy})$ and aligned with the part orientation $(l_{iu}, l_{iv})$  (see Fig.~\ref{fig:ps}). The dimensions $(h_i, w_i)$ of the support rectangle for each part are predefined, where the width is set $0.25$ of the length. The side of the part is defined as the longer side of the supporting rectangle. Further, the main axis of a part is the line segment starting at the part joint parallel to the part side.

\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.9\textwidth]{data/cc_fig.pdf}
\caption{\label{cc_fig} Left: input image; Middle left: segmentation with segment boundaries and their touching points in red. 
%A long sequence of boundaries form a contour if the angle at each touching point is small.
Middle right: contour edges which support part $\lpart_i$ and have normals which do not deviate from the part axis normal by more than $\omega$. 
%Small $\omega$ results in edges which are parallel and close to the part axis.
Right: first and second order moments of the region lying under the major part axis.}
\end{center}
\vskip -0.4in
\end{figure}
\mypar{Shape} We express the shape of limbs via region and contour
information. We use contour cues to capture the notion that limbs have
a long smooth outline connecting and supporting both the upper and
lower parts.  Region information is used to express coarse global
shape properties of each limb, attempting to express the fact the
limbs are often supported by a roughly rectangular collection of
regions---the same notion that drives the bottom-up hypothesis
generation in~\cite{mori04,Srinivasan07}.
% of segments A second shape feature captures the notion that arms tend to have the shape of rectangles.

\mypar{Shape/Contour} We detect long smooth contours from sequences of
image segmentation boundaries obtained via NCut~\cite{cour05}.
%sequences of boundaries of image segments.
We define a graph whose nodes are all boundaries between segments with
edges linking touching boundaries. Each contour is a path in this
graph (see Fig.~\ref{cc_fig}, middle left). To reduce the number of
possible paths, we restrict ourselves to all shortest paths. To
quantify the smoothness of a contour, we compute an angle between each
two touching segment boundaries\footnote{This angle is computed as the
  angle between the lines fitted to the segment boundary ends, defined
  as one third of the boundary. }. The smoothness of a contour is
quantified as the maximum angle between boundaries along this
contour. Finally, we find among all shortest paths those whose length
exceeds $\ell_{\textrm{th}}$ pixels and whose smoothness is less then
$s_{\textrm{th}}$ and denote them by $\{c_1,\dots c_m\}$.\footnote{We
  set $\ell_{\textrm{th}} = 60$ pixels, $s_{\textrm{th}} = 45^\circ$
  resulting in $15$ to $30$ contours per image.}

% To define the above features, we extract segments using NCut \cite{cour05}. For the contour features, we extract long smooth contours, each defined as a sequence of linked segment boundaries, such that the transitions between boundaries are smooth (see Fig.~\ref{cc_fig}, middle left). To obtain such sequences, we define a graph, whose nodes are all boundaries between segments with edges linking touching boundaries. For each pair of segment boundaries, we compute the shortest path between them, which represents a contour in the image. We retain contours which are longer than $l_{\textrm{th}}$ pixels and are smooth. To quantify the smoothness of a contour, we compute an angle between each two touching segment boundaries. This can be done by fitting a line to the segment boundary end, defined as one third of the boundary, and compute the angle between the the boundary ends at the touching point.  The smoothness of a contour is quantified as the maximum angle between boundaries along this contour. We retain contours whose smoothness is less than $s_{\textrm{th}}$. In our implementation we use $30$ segments and set $l_{\textrm{th}} = 60$ pixels, $s_{\textrm{th}} = 45^\circ$, which results in $m$ contours per image $\{c_1,\dots c_m\}$ for $m$ usually between $15$ and $30$.

We can use the above contours to define features for each pair of
lower and upper arms, which encode the notion that those two parts
should share a long smooth contour, which is parallel and close to the
part boundaries. For each arm part $l_i$ and a contour $c_k$ we can
estimate the edges of $c_k$ which lie inside one of the halves of the
supporting rectangle of $l_i$ and whose edge normals build an angle
smaller than $\omega$ with the normal of the part axis (see
Fig.~\ref{cc_fig}, right). We denote the number of those edges by
$q_{ik}(\omega)$. Intuitively, a contour supports a limb if it is
mostly parallel and enclosed in one of the limb sides, i.e.~the value
$q_{ik}(\omega)$ is large for small angles $\omega$. A pair of arm
limbs $l_i$, $l_j$ should have a high score if both parts are
supported by a contour $c_k$, which can be expressed as the following
two scores
\[
  \textrm{cc}_{ijk}^{(1)}(\omega, \omega') = \frac{1}{2}\left(\frac{q_{ik}(\omega)}{h_i} + \frac{q_{jk}(\omega')}{h_j}\right)\quad\textrm{and}\quad\textrm{cc}_{ijk}^{(2)}(\omega, \omega') = \min\left\{\frac{q_{ik}(\omega)}{h_i}, \frac{q_{jk}(\omega')}{h_j}\right\}
\]
where we normalize $q_{ik}$ by the length of the limb $h_i$ to ensure
that the score is in $[0,1]$. The first score measures the overall
support of the parts, while the second measures the minimum
support. Hence, for $l_i$, $l_j$ we can find the highest score among
all contours, which expresses the highest degree of support which this
pair of arms can receive from any of the image contours:
\[
\textrm{cc}_{ij}^{(t)}(\omega, \omega') = \max_{k\in\{1, \dots , m\}}\textrm{cc}_{ijk}^{(t)}(\omega, \omega'), \quad\textrm{for} \quad t\in\{1,2\}
\]
By varying the angles $\omega$ and $\omega'$ in a set of admissible
angles $\Omega$ defining parallelism between the part and the contour,
we obtain $|\Omega|^2$ contour features\footnote{We set
  $\Omega=\{10^\circ, 20^\circ, 30^\circ\}$, which results in $18$
  features for both scores.}.
% For the left limbs we use the right half of the supporting rectangle, viewed from the part joint, while for the right limbs we use the left half. This corresponds to the outer contour of each arm

\mypar{Shape/Region Moments} We compute the first and second order
moments of the segments lying under the major part axis (see
Fig.~\ref{cc_fig}, right)\footnote{We select segments which cover at
  least $25\%$ of the part axis.} to coarsely express shape of limb
hypotheses as a collection of segments, $R_{\lpart_i}$. To achieve
rotation and translation invariance, we compute the moments in the
part coordinate system.  We include convexity information
$|conv(R_{\lpart_i})|/|R_{\lpart_i}|$, where $conv(\cdot)$ is the
convex hull of a set of points, and $|R_{\lpart_i}|$ is the number of
points in the collection of segments.  We also include the number of
points on the convex hull, and the number of part axis points that
pass through $R_{\lpart_i}$ to express continuity along the part axis.
% The resulting $7$ features are used in the unary potentials of \modelname{}.
 
% Note that contour feature is a pure bottom-up cue which does not capture the precise arm shape but encodes figural properties of the arm -- smoothness and continuity of its boundary. It is a mid-level cue related to a configuration of two parts. The part shape, however, encodes a more precise shape but only of a single part.
 
 %\mypar{Appearance}
%We capture the  appearance of the individual body parts using Histogram of Gradient (HoG) and color based features.

\mypar{Appearance/Texture} Following the edge-based representation
used in \cite{latentsvm}, we model the appearance the body parts using
Histogram of Gradient (HoG) descriptor.  For each of the 6 body parts
-- head, torso, upper and lower arms -- we learn an individual
Gentleboost classifier \cite{friedman00} on the HoG features using the
Limbs Annotated in Movies Dataset\footnote{LAMDa is available at
  \url{http://vision.grasp.upenn.edu/video}}.
%The output of the classifier is our first appearance feature.

\mypar{Appearance/Color} As opposed to HoG, color drastically varies
between people. We use the same assumptions as \cite{eichner09} and
build color models assuming a fixed location for the head and torso at
run-time for each image.  We train Adaboost classifiers using these
pre-defined regions of positive and negative example pixels,
represented as RGB, Lab, and HSV components.  For a particular image,
a 5-round Adaboost ensemble~\cite{freund1997decision} is learned for
each color model (head, torso) and reapplied to all the pixels in the
image.  A similar technique is also used by~\cite{strikeapose} to
incorporate color.
%Face and torso can reveal information about skin and clothing color of all other parts.  
Features are computed as the mean score of each discrimintative color model on the pixels lying in the rectangle of the part.

% on positive examples drawn from fixed rectangles, which roughly localize the person torso and head, and negative examples drawn from the background of training images. We use the color channels in RGB, Lab and HSV spaces for each pixels as features. Then we can use those models on unknown part hypotheses from the same image -- head and torso reveal information about the skin and clothing color which are same for the arm clothing and hand color. For an arm hypothesis, the two color features $f_2, f_3$ are computed as the mean score of the pixels lying in the support of the part using both models. 

We use similarity of appearance between lower and upper arms as
features for the pairwise potentials of \modelname{}. Precisely, we
use the $\chi^2$ distance between the color histograms of the pixels
lying in the part support. The histograms are computed using
minimum-variance quantization of the RGB color values of each image
into $8$ colors.
% Precisely, we use two features, the first $f_4$ being the $\chi^2$ distance between the color histograms of the pixels lying in the part support. The histograms are computed using minimum-variance quantization of the RGB color values of each image into $8$ colors. The second feature $f_5$ is defined in terms of the spectral embedding obtained from NCuts segmentation \cite{cour05}. NCuts is defined in terms of a pixel affinity matrix which encodes color and intervening contour similarities (see~\cite{cour05} for details). The final segmentation is obtained through discretization of the top eigenvectors (we use the top $30$) of the affinity matrix. These vectors define for each pixel an embedding vector (in our case of dimension $30$) with the property that the vectors in this embedding space are clearly clustered according to the NCut segmentation criterion and the cues used in the affinity matrix. Thus, the mean embedding vector of all pixels in the support of a body part can be interpreted as an segmentation embedding vector of the part. FInally, the dot product of two such vectors representing two arm parts can be interpreted as similarity score, which is our last appearance feature $f_5$.

\mypar{Geometry} The body part configuration is encoded in two set of
features. The location $(l_{ix}, l_{iy})$ and orientation $(l_{iu},
l_{iv})$, included in the state of a part, are used added as absolute
location prior features.  We express the relative difference between
part $\lpart_i$ its parent $\lpart_j$ in the coordinate frame of the
parent part as $T_{ij}(\lpart_i) - \lpart_j$.
% parent's coordinate frame, and $\lpart_{i\omega}$ is simply the angular representation of $\lpart_i$'s direction.
%same quantities as in the original ps structure, but expanded out intThe relative positions between two parts $l_i$ and its parent $l_j$ are captured by the difference and the products of differences between the state components of the two parts: 
%\[
%f_7=(dl_x, dl_y, dl_x^2, dl_y^2, dl_xdl_y, dl_u, dl_v, dl_u^2, dl_v^2, dl_udl_v)
%\]
%where $dl_k = l_{ik} - l_{jk}$ is the difference of the state component $k$. Note that we include second order terms to model non-linear geometric interactions. 
Note we could introduce second-order terms to model a quadratic deformation cost akin to the classical PS, but we instead adopt more flexible binning or boosting of these features (see Section~\ref{implementation}).




==> text/eccv/implementation.tex <==
\section{Implementation Details} \label{implementation}

%In this section we discuss the application of the cascaded models from sec.~\ref{sec:model} and the features from sec.~\ref{sec:features}.
\vspace{-0.2cm}
\subsubsection*{Coarse-to-Fine Cascade} 
%We assume the upper-body is already roughly localized via an upper-body detector, in keeping with our dataset (see Section~\ref{experiments_sec}).  We normalize all images to the same size, and discretize the full-resolution part state space as a $120 \times 110\times 24$ grid for the part location and orientation. 
While our fine-level state space has size $80 \times 80 \times 24$, our first level cascade coarsens the state-space down to $10 \times 10 \times 12 = 1200$ states per part, which allows us to do exhaustive inference efficiently.  We always train and prune with $\alpha = 0$, effectively throwing away half of the states at each stage.  After pruning we double one of the dimensions (first angle, then the minimum of width or height) and continue (see Table~\ref{tab:pruning}). 
%As described in Section~\ref{sec:model}, after learning, we rank each part state in each training example according to its max-marginal score, and choose a max-marginal rank cutoff for pruning so that the groundtruth sequence remains in 95\% of the training data ($\beta = 0.95$). 
%After each pruning stage we increase the dimensions of the state-space if this increase will keep the number of states under a hard memory limit.  We found that there was always at least one part that was sufficiently pruned to increase resolution at each stage.  Five stages were required in total to reach the original state-space resolution.  
%Table~\ref{tab:c2f} enumerates the progression of state space sizes and percentage of the total space pruned after each stage.
In the coarse-to-fine stages we only use standard PS features.  HoG part detectors are run once over the original state space, and their outputs are resized to for features in coarser state spaces.  We also use the standard relative geometric cues as described in Sec.~\ref{sec:features}.  We bin the values of each feature uniformly, which adds flexibility to the standard PS model---rather than learning a mean and covariance, multi-modal pairwise costs can be learned.  
%We learn weights for the different bins via averaged perceptron---each model passes over the training set 10 times in random order, and the final weights are the average of the last quarter of the epochs.  % This type of geometric binning is also included in the PS implementation of~\cite{devacrf}, but they do not bin unary potential features.
\subsubsection*{Sparse States, Rich Features} To obtain segments, we use NCut\cite{cour05}. For the contour features we use 30 segments and for region moments -- 125 segments. As can be seen in Table~\ref{tab:pruning}, the coarse-to-fine cascade leaves us with roughly 500 hypotheses per part.  For these hypotheses, we generate all features mentioned in Sec.~\ref{sec:features}.  For pairs of part hypotheses which are farther than 20\% of the image dimensions from the mean connection location, features are not evaluated and an additional feature expressing this condition is added to the feature set.  % We use an efficient kd-tree nearest neighbor algorithm to retrieve all pairs of valid parts which are close enough.
We concatenate all unary and pairwise features for part-pairs into a feature vector and learn boosting ensembles which give us our pairwise clique potentials\footnote{
% for each part pair: part-pair configurations close to the groundtruth are labeled positive, and part-pair configurations far from the groundtruth are used as negatives.  
%We get roughly 20 positive examples and 120,000 negative examples per image, which we subsample uniformly to fit into memory.  
We use OpenCV's implementation of Gentleboost and boost on trees of depth 3, setting the optimal number of rounds via a hold-out set.}.
This method of learning clique potentials has several advantages over stochastic subgradient learning: it is faster to train, can determine better thresholds on features than uniform binning, and can combine different features in a tree to learn complex, non-linear interactions.

%We concatenate all unary and pairwise features for part pairs into a feature vector for each potential state-pair.  Rather than learning weights via perceptron for these pairwise potentials, we learn Adaboost ensembles offline for each part pair: part-pair configurations close to the groundtruth are labeled positive, and part-pair configurations far from the groundtruth are used as negatives.  We get roughly 20 positive examples and 120,000 negative examples per image, which we subsample uniformly to fit into memory.  We use Gentleboost with trees of depth 2 and set the optimal number of rounds via a hold-out set.  This method of learning clique potentials has several advantages over perceptron: it is faster to train, can determine better thresholds on features than uniform binning, and can combine different features in a tree to learn complex, non-linear interactions.







==> text/eccv/intro.tex <==
\section{Introduction}

Pictorial structure models~\cite{fischler1973ps} are a popular method for human body pose estimation~\cite{felz05,fergus2005sparse,devacrf,ferrari08,andriluka09}.
The model is a Conditional Random Field over pose variables that characterizes 
local appearance properties of parts and geometric part-part interactions.   
The search over the joint pose space is linear time in the number of parts when 
the part-part dependencies form a tree.  However,  the individual part 
state-spaces are too large (typically hundreds of thousands of states) to allow 
complex appearance models be evaluated densely.   Most appearance models are 
therefore simple linear filters on edges, color and 
location~\cite{felz05,devacrf,ferrari08,andriluka09}. Similarly, because of 
quadratic state-space complexity, part-part relationships are typically 
restricted to be image-independent deformation costs that allow for convolution 
or distance transform tricks to speed up inference~\cite{felz05}. A common 
problem in such models is poor localization of parts that have weak appearance 
cues or are easily confused with background clutter (accuracy for lower arms in 
human figures is almost half of that for torso or head~\cite{andriluka09}).   
Localizing these elusive parts requires richer models of individual part shape 
and joint part-part appearance, including contour continuation and segmentation 
cues, which are prohibitive to compute densely.

In order to enable richer appearance models, we propose to learn a cascade of 
pictorial structures (\modelname{}) of increasing pose resolution which 
progressively filter the pose state space.  Conceptually, the idea is similar 
to the work on cascades for face detection~\cite{geman2001,viola02}, but the 
key difference is the use of structured models. Each level of the cascade at a 
given spatial/angular resolution refines the set of candidates from the 
previous level and then runs inference to determine which poses to filter out.  
For each part, the model selects poses with the largest max-marginal scores, 
subject to a computational budget.  Unlike conventional pruning heuristics, 
where the possible part locations are identified using the output of a 
detector, models in our cascade use inference in simpler structured models to 
identify what to prune, taking into account global pose in filtering decisions.
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\textwidth]{data/overview.png}
\end{center}
\caption{\label{fig:overview} Overview: A discriminative coarse-to-fine cascade 
of pictorial structures filters the pose space so that expressive and 
computationally expensive cues can be used in the final pictorial structure.  
Shown are 5 levels of our coarse-to-fine cascade for the right upper and lower 
arm parts.  Green vectors represent position and angle of unpruned states, the 
downsampled images correspond to the dimensions of the resepective state space, 
and the white rectangles represent classification using our final model.}
\end{figure}
As a result, at the final level the \modelname{} model has to deal with a much 
smaller hypotheses set which allows us to use a rich combination of features.  
In addition to the traditional part detectors and geometric features, we are 
able to incorporate object boundary continuity and smoothness, as well as shape 
features. The former features represent mid-level and bottom-up cues, while the 
latter capture shape information, which is complementary to the traditional 
HoG-based part models.  The approach is illustrated in the overview 
Figure~\ref{fig:overview}. We apply the presented \modelname{} model combined 
with the richer set of features on the Buffy and PASCAL stickmen benchmark, 
improving the state-of-the-art on arm localization. 

%TV show benchmark~\cite{ferrari08} and achieve state of the art accuracy of 
%$86.2\%$, an improvement of about 6\%.



==> text/eccv/model.tex <==
\section{Framework}\label{sec:model}
We first summarize the basic pictorial structure model and then
describe the inference and learning in the cascaded pictorial structures.
%\subsection{Basic PS Model}
\begin{floatingfigure}[lt]{0.52\columnwidth}
\begin{center}
\centerline{\includegraphics[width=0.5\columnwidth]{data/model_parameters2.pdf}}
\caption{Basic PS model with state $l_i$ for a part $L_i$.}
\label{fig:ps}
\end{center}
\vspace{-0.5cm}
\end{floatingfigure}
Classical pictorial structures are a class of graphical models where
the nodes of the graph represents object parts, and edges between
parts encode pairwise geometric relationships.  For modeling human
pose, the standard PS model decomposes as a tree structure into unary
potentials (also referred to as appearance terms) and pairwise terms
between pairs of physically connected parts.  Figure~\ref{fig:ps}
shows a PS model for 6 upper body parts, with lower arms connected to
upper arms, and upper arms and head connected to torso.  In previous
work~\cite{devacrf,felz05,ferrari08,posesearch,andriluka09}, the
pairwise terms do not depend on data and are hence referred to as a spatial or structural prior.
%\begin{figure}[]
%\begin{center}
%\centerline{\includegraphics[width=0.75\columnwidth]{data/model_parameters2.pdf}}
%\caption{Basic upper-body model with part state $l$ and part support rectangle of size $(w,h)$.}
%\label{fig:ps}
%\end{center}
%% \vskip -0.5in
%\end{figure}
The state of part $\Lpart_i$, denoted as $\lpart_i \in \Lspace_i$, encodes the joint location of the part in image coordinates and the direction of the limb as a unit vector: $\lpart_i = [\lpart_{ix} \; \lpart_{iy} \; \lpart_{iu} \; \lpart_{iv}]^T$. The state of the model is the collection of states of $M$ parts: $p(\Lparts = \lparts) = p(\Lpart_1 = \lpart_1, \ldots, \Lpart_M = \lpart_M)$.  The size of the state space for each part, $|\Lspace_i|$, the number of possible locations in the image times the number of pre-defined discretized angles. For example, standard PS implementations typically model the state space of each part in a roughly $100 \times 100$ grid for $\lpart_{ix} \times \lpart_{iy}$, with 24 different possible values of angles, yielding $|\Lspace_i| = 100 \times 100 \times 24 = 240,000$. The standard PS formulation (see~\cite{felz05}) is usually written in a log-quadratic form:
\begin{align}
p( \lparts | x) &\propto \prod_{ij} \exp(-\frac{1}{2}||\Sigma_{ij}^{-1/2}(T_{ij}(\lpart_i) - \lpart_j - \mu_{ij})||_2^2)  \times \prod_{i=1}^M \exp(\mu_i^T\phi_i(\lpart_i,x))
\label{eqn:standard_ps}
\end{align}
The parameters of the model are $\mu_i,\mu_{ij}$ and $\Sigma_{ij}$, and $\phi_i(\lpart_i,x)$ are features of the (image) data $x$ at location/angle $\lpart_i$.  The affine mapping $T_{ij}$ transforms the part coordinates into a relative reference frame.  The PS model can be interpreted as a set of springs at rest in default positions $\mu_{ij}$, and stretched according to tightness $\Sigma^{-1}_{ij}$ and displacement $\phi_{ij}(\lparts) = T_{ij}(\lpart_i) - \lpart_j$.  The unary terms pull the springs toward locations $\lpart_i$ with higher scores $\mu_i^T\phi_i(\lpart_i,x)$ which are more likely to be a location for part $i$.

This form of the pairwise potentials allows inference to be performed faster than $O(|\Lspace_i|^2)$:  MAP estimates $\argmax_{\lparts} p(\lparts | x)$ can be computed efficiently using a generalized distance transform for max-product message passing in $O(|\Lspace_i|)$ time.  Marginals of the distribution, $p(\lpart_i | x)$, can be computed efficiently using FFT convolution for sum-product message passing in $O(|\Lspace_i| \log |\Lspace_i|)$~\cite{felz05}.

While fast to compute and intuitive from a spring-model perspective, this model has two significant limitations.  One, the pairwise costs are unimodal Gaussians, which cannot capture the true multimodal interactions between pairs of body parts.  Two, the pairwise terms are only a function of the geometry of the state configuration, and are oblivious to the image cues, for example, appearance similarity or contour continuity of the a pair of parts.

\label{subsec:our_ps}
We choose instead to model part configurations as a general log-linear Conditional Random Field over pairwise and unary terms:
\begin{align}
p( \lparts | x) &\propto \exp \Biggl[\sum_{ij}  \theta_{ij}^T \phi_{ij}(\lpart_i,\lpart_j,x) +
\sum_i \theta_i^T\phi_i(\l_i,x) \Biggl] = e^{\theta^T \phi(\lparts,x)}.
\label{eqn:our_ps}
\end{align}
The parameters of our model are the pairwise and unary weight vectors $\theta_{ij}$ and $\theta_i$ corresponding to the pairwise and unary feature vectors $\phi_{ij}(\lpart_i,\lpart_j,x)$ and $\phi_i(\l_i,x)$.  For brevity, we stack all the parameters and features into vectors using notation $\theta^T \phi(\lparts,x)$. The key differences with the classical PS model are that (1) our pairwise costs allow data-dependent terms, and (2) we do not constrain our parameters to fit any parametric distribution such as a Gaussian.  For example, we can express the pairwise features used in the classical model as $\lpart_{i} \cdot \lpart_{i} \text{, } \lpart_{j}\cdot\lpart_{j} \text{ and }  \lpart_{i}\cdot\lpart_{j}$ without requiring that their corresponding weights can be combined into a positive semi-definite covariance matrix.

In this general form, inference can not be performed efficiently with distance transforms or convolution, and we rely on standard $O(|\Lspace_i|^2)$ dynamic programming techniques to compute the MAP assignment or part posteriors.  Many highly-effective pairwise features one might design would be intractable to compute in this manner for a reasonably-sized state space---for example an $100\times100$ image with a part angle discretization of $24$ bins yields $|\Lspace_i|^2 = 57.6$ billion part-part hypotheses.

In the next section, we describe how we circumvent this issue via a cascade of models which aggressively prune the state space at each stage typically without discarding the correct sequence.  After the state space is pruned, we are left with a small enough number of states to be able to incorporate powerful data-dependent pairwise and unary features into our model.


\subsection*{Structured Prediction Cascades} \label{cascades} The
recently introduced Structured Prediction Cascade
framework~\cite{cascades} provides a principled way to prune the state
space of a structured prediction problem via a sequence of
increasingly complex models.  There are many possible ways of defining
a sequence of increasingly complex models.  In~\cite{cascades} the
authors introduce higher-order cliques into their models in successive
stages (first unary, then pairwise, ternary, etc.).  Another option is
to start with simple but computationally efficient features, and add
more complex features downstream as the number of states decreases.
Yet another option is to geometrically coarsen the original state
space and successively prune and refine.  We use a coarse-to-fine
state space approach with simple features until we are at a reasonably
fine enough state space resolution and left with few enough states
that we can introduce more complex features.  We start with a severely
coarsened state space and use standard pictorial structures unary
detector scores and geometric features to perform quick exhaustive
inference on the coarse state space.

%The simplest analogy of the framework is to the popular cascade classifier introduced by Viola and Jones for binary prediction problems~\cite{Viola2002}.
More specifically, each level of the cascade uses inference to
identify which states to prune away and the next level refines the
spatial/angular resolution on the unpruned states.  The key ingredient
to the cascade framework is that states are pruned using {\em
  max-marginal} scores, computed using dynamic programming techniques.
For brevity of notation, define the score of a joint part state
$\lparts$ as $\theta_x(\lparts)$ and the max-marginal score of a part
state as follows:
\begin{align}
\theta_x(\lparts) &= \theta^T \phi(\lparts,x)= \sum_{ij}  \theta_{ij}^T \phi_{ij}(\lpart_i,\lpart_j,x) +
\sum_i \theta_i^T\phi_i(\l_i,x) \\
\mmi  &= \max_{\lparts' \in \Lparts} \;\;\; \{ \theta_x(\lparts') \; : \; \lpart_i'=\lpart_i \}
\end{align}

In words, the max-marginal for location/angle $\lpart_i$ is the score of the best sequence which constrains $\Lpart_i = \lpart_i$.  In a pictorial structure model, this corresponds to fixing limb $i$ at location $\lpart_i$, and determining the highest scoring configuration of other part locations and angles under this constraint.  A part could have weak individual image evidence of being at location $\lpart_i$ but still have a high max-marginal score if the rest of the model believes this is a likely location.  Similarly, we denote the MAP assignment score as
$\theta_x^\star = \max_{\lparts \in \Lparts} \theta_x(\lparts)$, the unconstrained best configuration of all parts.

When learning a cascade, we have two competing objectives that we must trade off,
accuracy and efficiency: we want to minimize the number of errors incurred by each
level of the cascade  and maximize the number of filtered max marginals.  A natural strategy is to prune away the lowest ranked states based on max-marginal scores. Instead, \cite{cascades} prune the states whose max-marginal score is lower than an data-specific threshold $t_x$: $l_i$ is pruned if $\mmi < t_x$.  This threshold is defined as a convex combination of the MAP assignment score and the mean max-marginal score, meant to approximate a percentile threshold: $$t_x(\theta,\alpha) = \alpha \theta^\star_x + (1-\alpha)\frac{1}{M}\sum_{i=1}^M\frac{1}{|\Lspace_i|}\sum_{\lpart_i \in \Lspace_i} \mmi,$$ where $\alpha\in[0,1]$ is a parameter to be chosen that determines how aggressively to prune. When $\alpha = 1$, only the best state is kept, which is equivalent to finding the MAP assignment.  When $\alpha = 0$ approximately half of the states are pruned (if the median of max-marginals is equal to the mean) .  The advantage of using  $t_x(\theta,\alpha)$ is that it is convex in $\theta$, and leads to a convex formulation for parameter estimation that trades off the proportion of incorrectly pruned states with the proportion of unpruned states.
Note that  $\alpha$ controls efficiency, so we focus on learning the parameters $\theta$ that 
minimize the number of errors for a given filtering level $\alpha$.   The learning formulation uses a simple fact about max-marginals and the definition of $t_x(\theta,\alpha)$
to get a handle on errors of the cascade:
if $\theta_x(\lparts) > t_x(\theta,\alpha)$, then for all i, $\mmi >  t_x(\theta,\alpha)$, so no part state of $\lparts$ is pruned.   Given an example $(x,\lparts)$,
this condition $\theta_x(\lparts) > t_x(\theta,\alpha)$ is sufficient to ensure that no correct part is pruned.
%\begin{floatingfigure}[lt]{0.52\columnwidth}
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.75\textwidth]{data/casscades.pdf}
\caption{Upper right: Detector-based pruning by thresholding (for the lower right arm) yields many hypotheses far way from the true one. Lower row: The CPS, however, exploits global information to perform better pruning.}
\label{fig:cascade_pruning}
\end{center}
\vspace{-0.7cm}
\end{figure}
%\end{floatingfigure}

To learn one level of the structured cascade model $\theta$ for a fixed $\alpha$, we try to minimize 
the number of correct states that are pruned on training data by solving the
following convex margin optimization problem given $N$ training examples $(x^n,\lparts^n)$:
\begin{equation}
  \label{eq:convex_opt}
 \min_{\theta} \;\;\;\ \frac{\lambda}{2}||\theta||^2 + \frac{1}{N}\sum_{n=1}^N H(\theta;x^n,\lparts^n),
\end{equation}
where $H$ is a hinge upper bound 
$H(\theta;x,\lparts) = \max\{0, 1 + t_x(\theta,\alpha) - \theta_x(\lparts)\}$.
The upper-bound $H$ is a hinge loss measuring the margin between the
filter threshold $t_{x^n}(\theta,\alpha)$ and the score of the truth
$\theta^T\phi(\lparts^n,x^n)$; the loss is zero if the truth scores above
the threshold by margin $1$.  We solve \eqref{eq:convex_opt} using stochastic
sub-gradient descent. Given an example $(x,\lparts)$, we apply the following
update if $H(\theta;x,\lparts)$ (and the sub-gradient) is non-zero:
\begin{equation*}
    \label{eq:spf_update}
    \theta'  \leftarrow \theta + \eta \left(-\lambda \theta + \phi(\lparts,x) - \alpha \phi(\lparts^\star,x)  - (1-\alpha) \frac{1}{M} \sum_{i} \frac{1}{|\Lspace_i|}\sum_{\lpart_i \in \Lspace_i}  \phi(\lparts^\star(\lparts_i),x)\right).
\end{equation*}
Above, $\eta$ is a learning rate parameter, $\lparts^\star = \argmax_{\lparts'}
\theta_x(\lparts')$ is the highest scoring assignment and $\lparts^\star(\lparts_i) = \argmax_{\lparts': \lparts'_i = l_i} \theta_x(\lparts')$
are highest scoring assignments constrained to $\lpart_i$ for part $i$.
The key distinguishing feature of this update as compared to
structured perceptron is that it subtracts features included in all
max-marginal assignments $\lparts^\star(\lparts_i)$\footnote{Note that because \eqref{eq:convex_opt} is $\lambda$-strongly convex,
if we chose $\eta_t = 1/(\lambda t)$ and add a projection step to keep 
$\theta$ in a closed set, the update would correspond to the Pegasos
update with convergence guarantees of $\tilde{O}(1/\epsilon)$ iterations for
$\epsilon$-accurate solutions~\cite{shalev-shwartz07pegasos}.  In our experiments, we found the projection step made no difference and used only 2 passes over the data, with $\eta$ fixed.}.
%, as we discuss in Section~\ref{implementation}.


\out{
\subsection*{Cascaded Pictorial Structures}

We take a similar but simpler approach that approximates the Structured Prediction Cascades method.  At each stage of the cascade, we learn parameters using the standard averaged perceptron algorithm~\cite{collins_discriminative_2002} (see supplemental material for the details).  Instead of a score threshold, we estimate a rank cutoff for max-marginals for each part, selected so that a large fraction $\beta$ of the training groundtruth poses are unpruned.  In practice, we found that we could prune away large portions (over 90\%) of the state space while only losing 5\% of the groundtruth states ($\beta = 0.95$) on the training data. Section~\ref{experiments_sec} details the proportion of states pruned at each level of the actual cascade we used.


There are many possible ways of defining a sequence of increasingly complex models.  In~\cite{cascades} the authors introduce higher-order cliques into their models in successive stages (first unary, then pairwise, ternary, etc.).  Another option is to start with simple but computationally efficient features, and add more complex features downstream as the number of states decreases.  Yet another option is to geometrically coarsen the original state space and successively prune and refine.

We use a coarse-to-fine state space approach with simple features until we are at a reasonably enough state space resolution and left with few enough states that we can introduce more complex features.  We start with a severely coarsened state space and use standard pictorial structures unary detector scores and geometric features to perform quick exhaustive inference on the coarse state space.  

Model parameters for each level are learned using the perceptron algorithm, and a rank-pruning threshold is set for each part using $\beta=0.95$.  For parts whose state spaces can be sufficiently pruned, we increase the resolution of the state space, mapping coarse states to a set of finer resolution states, and repeat.  Different parts have different rank-pruning thresholds, and different parts have different resolution state space at a particular stage of the cascade.  This allows us to maintain a different resolution of uncertainty for parts with weaker evidence, and postpone pruning decisions as long as possible.  We ensure progress is made after each cascade level by enforcing a minimum amount of pruning at each level.  Section~\ref{implementation} details the levels of the cascade learned using this approach.
}

The stages of the cascade are learned sequentially, from coarse to fine, and each has a different $\theta$ and $\Lspace_i$ for each part, as well as  $\alpha$.  The states of the next level are simply refined versions of the states that have not been pruned. We describe 
the refinement structure of the cascade in Section~\ref{implementation}.
In the end of a coarse-to-fine cascade we are left with a small, sparse set of states that typically contains the groundtruth states or states relatively close to them---in practice we are left with around 500 states per part, and 95\% of the time we retain a state the is close enough to be considered a match (see Table~\ref{tab:pruning}). At this point we have the freedom to add a variety of complex unary and pairwise part interaction features involving geometry, appearance, and compatibility with perceptual grouping principles which we describe in Section~\ref{sec:features}.

\myparnoc{Why not just detector-based pruning?} A naive approach used in a variety of applications is to simply subsample states by thresholding outputs of part or sparse feature detectors, possibly combined with non-max suppression.  Our approach, based on pruning on max-marginal values in a first-order model, is more sophisticated: for articulated parts-based models, strong evidence from other parts can keep a part which has weak individual evidence, and would be pruned using only detection scores.  The failure of prefiltering  part locations in human pose estimation is also noted by~\cite{andriluka09}, and serves as the primary justification for their use of the dense classical PS. This is illustrated in Figure~\ref{fig:cascade_pruning} on an example image from~\cite{ferrari08}.


==> text/eccv/pruning_results.tex <==
\begin{table}[t]
\begin{center}
{\scriptsize

\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{level}	 & state	& \multicolumn{2}{|c|}{\# states in the}	&  \multirow{3}{*}{ } state space	& $\text{PCP}_{0.2}$ \\\cline{3-4}
 & 	 dimensions &original	& pruned	& reduction	&  arms \\
 & 	 & space	& space	& \%	& oracle  \\

\hline
0	 & 10x10x12	 & 153600	 & 1200 & 	 00.00 & ---\\
\hline
1	 & 10x10x24	 & 72968 & 	1140  &  52.50	 & 54 \\
\hline
3	 & 20x20x24	 & 6704	 & 642	&  95.64	 & 51 \\
\hline
5	 & 40x40x24	 & 2682	 & 671	 & 98.25	 & 50 \\
\hline 
7	 & 80x80x24	 & 492	 & 492& 	 99.67	 & 50 \\
\hline
detection pruning	 & 80x80x24	 & 492	 & 492& 	 99.67	 & 44 \\
%pruning	 &	 &	 && 	 	 &  \\
\hline
\end{tabular} }
\caption{\label{tab:pruning} For each level of the cascade we present the reduction of the size of the state space after pruning each stage and the quality of the retained hypotheses measured using PCP$_{0.2}$. As a baseline, we compare to pruning the same number of states in the HoG detection map (see text).}
\end{center}
\vspace{-0.8cm}
\end{table}


==> text/eccv/related.tex <==
\section{Related Work} \label{sec:related}

The literature on human pose estimation is vast and varied in settings: applications range from highly-constrained MOCAP environments (\eg~\cite{lan5beyond}) to extremely articulated baseball players (\eg~\cite{mori04}) to the recently popular ``in the wild'' datasets Buffy (from TV) and the PASCAL Stickmen (from amateur photographs)~\cite{ferrari08}.
%person layout challenge~\cite{}. 
We focus our attention here on the work most similar in spirit to ours, namely, pictorial structures models.  First proposed in~\cite{fischler1973ps}, efficient inference methods
focusing on tree-based models with quadratic deformation costs were introduced in~\cite{felz05}.  Ramanan~\cite{devacrf} proposed learning PS parameters discriminitively by maximizing conditional likelihood and introduced further improvements using iterative EM-like parsing~\cite{devaparse}.
%---the model is run once using generic detectors, and then image-specific appearance terms are included based on the first parse, and the model is run again.
Ferrari et al.~\cite{ferrari08,posesearch} also prune the search space for computational efficiency and to avoid false positives.  
%They employ a multi-stage system to prune the search space:  An upper body is first localized, and a foreground-background segmentation is run to remove clutter, and portions of the state space for are hard-coded to be pruned because of their unlikeliness of containing the part.  
Our end goal is the same, but we adopt a more principled approach, expressing features on regions and locations and letting our system learn what to eliminate at run-time given the image.


%The publicly available code has been built upon in~\cite{ferrari08} by pre-processing to localize and remove background clutter, and parsing through time and space in video via loopy-belief propagation.  Further gains have been made by restricting the state space~\cite{ferrari08,posesearch}, adding additional pairwise terms that break the tree-structured assumption~\cite{posesearch}, and estimating color distributions using {\em a priori} estimates of where the parts should be~\cite{eichner09}.

For unstructured, binary classification, cascades of classifiers have been quite successful for reducing computation.  Fleuret and Geman~\cite{geman2001} propose a coarse-to-fine sequence of binary tests to detect the presence and pose of objects in an image.  The learned sequence of tests is trained to minimize expected computational cost.  The extremely popular Viola-Jones classifier~\cite{viola02} implements a cascade of boosting ensembles, with earlier stages using fewer features to quickly reject large portions of the state space.

Our cascade model is inspired by these binary classification cascades, and is based on the structured prediction cascades framework~\cite{cascades}.  In natural language parsing, several works \cite{carreras2008tag,petrov:PhD} use a coarse-to-fine idea closely related to ours and~\cite{geman2001}: the marginals of a simple context free grammar or dependency model are used to prune the parse chart for a more complex grammar.

Recently, Felzenszwalb et al.~\cite{pff-cascade} proposed a cascade for a structured parts-based model.  Their cascade works by early stopping while evaluating individual parts, if the combined part scores are less than fixed thresholds.  While the form of this cascade can be posed in our more general framework (a cascade of models with an increasing number of parts), we differ from~\cite{pff-cascade} in that our pruning is based on thresholds that adapt based on inference in each test example, and we explicitly learn parameters in order to prune safely and efficiently. In~\cite{geman2001,viola02,pff-cascade}, the focus is on preserving established levels of accuracy while increasing speed.  The focus in this paper is instead developing more complex models---previously infeasible due to the original intractable complexity---to improve state-of-the-art performance.

A different approach to reduce the intractable number of state hypotheses is to instead propose a small set of likely hypotheses based on bottom-up perceptual grouping principles~\cite{mori04,Srinivasan07}.  Mori et al.~\cite{mori04} use bottom-up saliency cues, for example strength of supporting contours, to generate limb hypotheses.  They then prune via hand-set rules based on part-pair geometry and color consistency. The shape, color and contour based features we use in our last cascade stage are inspired by such bottom-up processes.  However, our cascade is solely a sequence of discriminatively-trained top-down models.


\out{
We differ from this progression of PS-based models~\cite{devacrf,devaparse,ferrari08,posesearch,eichner09} in several ways: \textbf{(1)} We do not employ multiple iterations of parsing, or loopy belief propagation.  Instead we perform inference once with a tree-structured model.  \textbf{(2)} We do not use color information~\footnote{Modulo what is used to compute superpixels and Pb, described in Section~\ref{sec:shapekernel}}---the driving force behind our kernel is shape information from regions and contours. \textbf{(3)} We perform no post-processing of the beliefs of our inference; rather we trust them to be our final answer.  The final output in~\cite{ferrari08,eichner09} involve ad-hoc post-processing. Our basic PS implementation most closely resembles~\cite{andriluka09}, but our parameters are discriminitively trained.

Finally the goal of our kernel design process is similar to the focus of ~\cite{posesearch}, which in {\em query mode} seeks to retrieve poses similar to a query image.  Our requirements in designing a kernel are slightly different in that we require a mapping from every training instance to an effective similarity score, rather than focusing on precision and recall.  Also, they use PS inference as input to their retrieval.
}


==> text/eccv/results_all.tex <==
\begin{table}[t]
\subfigure[][]{ 
\label{tab:overall}
{\scriptsize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
method &	torso &	head	 &	upper	 &	lower	 &	total \\
 &	&		 &	arms	 &	arms	 &	\\
\hline\hline
\textbf{Buffy} & & & & &\\
\hline
\cite{ferrari08}	 &	-	 &	-	 &	-	 &	-   &	 61.4 \\
\hline
\cite{posesearch}	 &	-	 &	-	 &	-	 &	-		 &	74.5 \\
\hline
\cite{andriluka09}	 &	90.7	 &	95.5	 &	79.3	 &	41.2	 &		73.5 \\
\hline
\cite{eichner09}		 &	98.7 	 &		97.9		 &	82.8	& 59.8	 &	80.1 \\
\hline
APS~\cite{sapp2010}	&	100		 &	100		 &	91.1 &		65.7	 &	85.9 \\
\hline
CPS 	&	100	&	96.2	&	95.3	&	63.0	& 	85.5 \\
\hline
Detector &		99.6	&	87.3&		90.0	&	55.3 	&		79.6 \\
pruning &			&	&			&	&		 \\
\hline\hline						
\textbf{PASCAL} & & & & & \\
\hline
\cite{eichner09}		&	98.72	&	97.87	&	82.8	&	59.79		&	80.1 \\
\hline
APS~\cite{sapp2010}	&	100	&	98.0	&	83.9	&	54.0		&	79.0 \\
\hline
CPS 	&	100	&	90.0	&	87.1	&	49.4		&	77.2 \\
\hline
\end{tabular}
}
}
\subfigure[][]{
\label{tab:pruning}
{\scriptsize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{level}	 & state	& \multicolumn{2}{|c|}{\# states in the}	&  \% & $\text{PCP}_{0.2}$ \\\cline{3-4}
 & 	 dimensions &original	& pruned	&   reduction	&  arms \\
 & 	 & space	& space	& 	&  \\

\hline
0	 & 10x10x12	 & 153600	 & 1200 & 	 00.00 &\\
\hline
1	 & 10x10x24	 & 72968 & 	1140  &  52.50	 & 54 \\
\hline
3	 & 20x20x24	 & 6704	 & 642	&  95.64	 & 51 \\
\hline
5	 & 40x40x24	 & 2682	 & 671	 & 98.25	 & 50 \\
\hline 
7	 & 80x80x24	 & 492	 & 492& 	 99.67	 & 50 \\
\hline
Detector	 & 80x80x24	 & 492	 & 492& 	 99.67	 & 44 \\
pruning	 &	 &	 && 	 	 &  \\
\hline
\end{tabular} }
}
\label{tab:results_all}
\caption{\textbf{Left:} Comparison to other methods at PCP$_{0.5}$.  See text for details.  We perform comparably to state-of-the-art on all parts, improving on upper arms. \textbf{Right:} For each level of the cascade we present the reduction of the size of the state space after pruning each stage and the quality of the retained hypotheses measured using $PCP_{0.2}$. As a baseline, we compare to pruning the same number of states in the HoG detection map (see text). }
\vspace{-0.5cm}
\end{table}

==> text/eccv/results_table.tex <==

\begin{table}[t]
\begin{center}
{\scriptsize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
method &	torso &	head	 &	upper	 &	lower	 &	total \\
 &	&		 &	arms	 &	arms	 &	\\
\hline\hline
\textbf{Buffy} & & & & &\\
\hline
%Ferrari et al.~2008~\cite{ferrari08}	 &	-	 &	-	 &	-	 &	-   &	 61.4 \\
%\hline
%Ferrari et al.~2009~\cite{posesearch}	 &	-	 &	-	 &	-	 &	-		 &	74.5 \\
\hline
Andriluka et al.~\cite{andriluka09}	 &	90.7	 &	95.5	 &	79.3	 &	41.2	 &		73.5 \\
\hline
Eichner et al.~\cite{eichner09}		 &	98.7 	 &		97.9		 &	82.8	& 59.8	 &	80.1 \\
\hline
APS~\cite{sapp2010}	&	100		 &	100		 &	91.1 &		65.7	 &	85.9 \\
\hline
CPS (ours)	&	99.6 &	98.7	&	91.9	&	64.5	& 	85.2 \\
\hline
Detector pruning &		99.6	&	87.3&		90.0	&	55.3 	&		79.6 \\
\hline\hline						
\textbf{PASCAL stickmen} & & & & & \\
\hline
Eichner et al.~\cite{eichner09}		&	97.22	&	88.60	&	73.75	&	41.53		&	69.31 \\
\hline
APS~\cite{sapp2010}	&	100	&	98.0	&	83.9	&	54.0		&	79.0 \\
\hline
CPS (ours)	&	100	&	99.2	&	81.5	&	53.9		&	78.3 \\
\hline
\end{tabular}
}
\caption{\label{tab:overall} Comparison to other methods at PCP$_{0.5}$.  See text for details.  We perform comparably to state-of-the-art on all parts, improving on upper arms.
\textbf{NOTE}: the numbers included here are slightly different from the published version---what is seen here exactly matches the publicly available reference implementation at \\
\url{http://vision.grasp.upenn.edu/video/}.}
\end{center}
\vspace{-0.8cm}
\end{table}



==> text/ensembles.tex <==


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 


==> text/grant/intro.tex <==
\noindent{\Large\bf Project Description}
\vspace{-0.5cm}
\section{Introduction}
% paragraph goal: ml is needed to build systems across many disciplines
% current methods rely on supervised machine learning
% supervised learning takes a lot of work
%pg:
%\textbf{A new complexity trade-off.}
The classical trade-off between approximation and estimation error
(bias/variance) is fundamental in machine learning.  In regression and
classification problems, the \textit{approximation error} can be
reduced by increasing the complexity of the model at the cost of
higher \textit{estimation error}. Standard statistical procedures
explore a \textit{hierarchy of models} of increasing complexity
without much concern for the computational cost of using the model at
test time~\cite{hastie2001esl}.  However, in structured prediction
tasks~\cite{psd-book}, such as machine translation, speech
recognition, articulated human pose estimation, computational
constraints play a critical role as models with increasing complexity
of inference are considered.  In all these tasks, there is an
exponential number of possible predictions for every input.  Breaking
these joint predictions up into independent decisions (e.g., translate
each word independently, recognize a phoneme at a time, detect arms
separately) ignores critical correlations and leads to poor
performance.  Structured models used for these tasks, such as grammars
and graphical models, can capture strong dependencies but at
considerable cost of inference.  For example, a first order
conditional random field (CRF)~\cite{lafferty01crf} is fast to
evaluate but may not be an accurate model for phoneme recognition,
while a fifth order model is more accurate, but prohibitively
expensive for both learning and prediction. Model complexity can lead
to over-fitting problems due to the sparseness of the training data,
but this aspect of the error is fairly well understood and controlled
using standard regularization methods.

Computational constraints introduce a much more complicated balancing
act.  First, they prevent one from even exploring more expressive
models because of computational limits at prediction time.  Second, if
one does decide to explore, one typically uses heuristic pruning
techniques or approximate search methods in order to make higher order
models feasible.
%In practice, model complexity is limited by inference cost at prediction time, either explicitly by the user or implicitly
%because of the limits of available time or memory. 
%We therefore need to balance expected error with inference cost. 
These methods are currently used essentially by trial-and-error,
without quantitative understanding of the additional error introduced
by approximating more expressive but intractable models.  For example,
in statistical machine translation, syntactic models are combined with
n-gram language models to produce impractically large inference
problems, which are heavily and heuristically pruned in order to fit
into memory and any reasonable time
budget~\cite{hiero,venugopal2007efficient,
  zhang2008efficient,petrov-haghighi-klein:2008:EMNLP}.  Most machine
translation and natural language parsing systems do not use full
end-to-end discriminative learning because of the need to repeatedly
perform inference at training
time~\cite{moses,li2008scalable,lopez2008statistical}.  As another
example, consider estimating articulated human pose in realistic
videos (see Fig.~\ref{fig:res_all_img}): predicting the positions of
the head, arms, torso, legs, etc. in every image frame. Even moderate
degrees-of-freedom and spatial resolution lead to very large
state-spaces and intractable computational barriers to capturing
complex dynamics and appearance models, and most systems use heuristic
approximations to scale up inference~\cite{ferrari08}.  While
domain-specific and hand-tuned short-cuts can often speed up
inference, they obscure the merits of the model and make systems quite
opaque and brittle.  Simply put, when the system accuracy does not
improve after enriching the model, we don't know if the model is
biased, over-fit or poorly approximated by heuristic inference.
Unlike in standard supervised learning, the model complexity hierarchy
is critically stunted by this \textit{inference bottleneck}.

\begin{figure}[t]
\begin{center}
%\includegraphics[width=0.98\textwidth]{figs/results_all.pdf}
\end{center}
\caption{\label{fig:res_all_img}  Articulated pose
estimation in challenging videos where the state-space is prohibitively large for standard methods (preliminary results shown).}
\vspace{-0.4cm}
\end{figure}

One of the most common ways of dealing with complexity is through
abstraction and refinement.  Many problems have a natural granularity
or abstraction hierarchy: for example, temporal, spatial, or symbolic.
Various abstraction hierarchies are often used in classical planning
and reinforcement learning~ \cite{ParrRu98, SuttonPr99, Dietterich00}.
In coarse-to-fine dynamic programming~\cite{raphael01c2fdp} and
hierarchical $A^*$~\cite{felzenszwalb2007generalized}, search states
and operators form a refinement hierarchy and multiple levels of
heuristic cost functions must satisfy proper lower-bound constraints
between abstraction layers in order to guarantee admissability and
optimality (essentially, abstract costs must lower-bound fine-level
costs).  Tremendous savings arise when abstract states/operators
accurately summarize their refinements and inference can leave many
states at the abstract, unrefined levels, focusing instead on refining
only the most promising states. However, the admissability
restrictions on costs are often difficult to satisfy in practical
problems without forfeiting efficiency. Furthermore, the models and
their abstractions are assumed given, not learned from data to
maximize accuracy and efficiency.  In computer vision, coarse-to-fine
cascades of classifiers have been quite successful for reducing
computation.  Fleuret and Geman~\cite{geman2001} propose a
coarse-to-fine sequence of binary tests to detect the presence and
position of objects in an image.  The popular Viola-Jones face
detector~\cite{viola02} implements a cascade of boosted ensembles,
with earlier stages using fewer features to quickly reject large
portions of the state space.  In natural language parsing, several
works \cite{charniak2000maximum,carreras2008tag,petrov:PhD} use a
coarse-to-fine idea: the marginals of a simple context free grammar or
dependency model are used to prune the parse chart for a more complex
grammar.  The key idea in these approaches is that the
\textit{complexity hierarchy is explored at test time}, and more
complex models are used on more \textit{difficult examples}, and in
the structured case of grammars, on \textit{difficult parts} of
sentences.  By dropping strict admissability and only using expensive
inference in the rare difficult cases, high overall efficiency and
accuracy can be achieved.  However, previous works remain
unsatisfactory in several respects: (1) model parameters are not
learned specifically to balance accuracy/efficiency trade-off, but
using unrelated criteria; (2) no optimality or generalization
guarantees exist; (3) no theoretical analysis of what properties of
the problem would ensure success of coarse-to-fine methods.

% \begin{wrapfigure}{r}{0.2\textwidth}
% \vspace{-0.5cm}
%   \centering
%   \includegraphics[width=0.2\textwidth]{figs/cascade.pdf}
%   \vskip -2mm
%   \caption{\small Diagram of a structured cascade where each filter
%   is a model that progressively prunes the space of predictions $\Y(x)$ for input $x$.}
%   \label{fig:filters}
% \vspace{-0.5cm}
% %\end{figure}
% \end{wrapfigure}
The fundamental \textit{goal of this proposal} is to enable principled use of richer models in structured prediction.  The main
enabling technique is the input-adaptive exploration of the complexity hierarchy at both training and test time.  
The proposal addresses \textit{hierarchical structured prediction} by learning
a cascade of models of increasing complexity that progressively filter a given structured output space, minimizing overall error and
computational effort at prediction time according to a desired trade-off (see illustration in Fig.~\ref{fig:filters}). 
Each level corresponds to a structured model and levels manipulate exponentially large sets of filtered outputs using max marginals.
A novel convex loss function is proposed for learning cascaded models that balances filtering error with filtering efficiency. Initial analysis shows that the use of max-marginals allows derivation of generalization bounds for both accuracy and efficiency of the cascade.   Unlike admissable model abstraction
used in hierarchical $A^*$ or coarse-to-fine dynamic programming, different layers of abstraction are not constrained
to strictly lower-bound each other but are learned to be \textit{provably accurate and efficient with high probability} in eliminating unpromising decisions.  Preliminary experimental results show
that the proposed cascade formulation is very effective on several problems (reducing the complexity of inference by up to five orders of magnitude) and enables scaling up to much richer and more accurate models.  These promising results motivate further
experimentation and larger-scale applications as well as several natural theoretical questions and extensions of the cascade framework.  
% On the theoretical front, a natural question is what intuitive and easily quantifiable 
%properties of a given problem guarantee the success coarse-to-fine reasoning.  On the algorithmic front, I propose
%to extend the cascade idea to allow multiple models per layer that coordinate their filtering decisions.  When
%such models contain different tractable subsets of true dependencies in the data.
% propose several extensions
%of the theoretical analysis, 





\mypar{Objectives and Significance}
The need to analyze and make effective use of the vast amounts
of data has made machine learning indispensable in building
intelligent, adaptive systems. Major improvements in accuracy and
robustness, in computer vision and computational linguistics in
particular, have been propelled by advances in supervised machine
learning. Research enabling intelligent systems through machine learning has shown 
great scientific, technological, and economic importance.  
The proposed research aims to address fundamental barriers in creation of richer models able to 
handle dramatically more complex and difficult predictions.  Specifically, 
the proposal presents a novel  \textit{hierarchical structured prediction}
framework using data-driven coarse-to-fine reasoning.

\mypar{Research Plan Overview}
The objectives of the research aspect of the proposal are:
\begin{packed_itemize}
\item \textbf{Flexible framework} for designing coarse-to-fine
models and information flow between them at training and test time.  The goal is to
support many possible abstraction hierarchies, for example, spatial and temporal resolution, increasing 
Markov order, etc. 
\item \textbf{Efficient algorithms for learning efficient models} 
that explicitly control computation vs. approximation trade-off.   Developing
a convex loss function that balances accuracy and efficiency at each level 
of the cascade. Designing a learning formulation that can also learn
\textit{decomposable cascades}, where each level
combines multiple overlapping models.
\item \textbf{Extensive validation} of the framework on difficult
real-world problems. The plan includes large-scale evaluation in two domains:
graphical models for detailed action understanding in video and  grammar-based models for 
natural language parsing and translation.
\item \textbf{Theoretical understanding} of generalization capacity of
coarse-to-fine models and conditions 
on the learning problems under which coarse-to-fine reasoning 
can be guaranteed to succeed. \end{packed_itemize}

\mypar{Educational Plan Overview}
My educational plan focuses on integrative, collaborative learning
along three modes of participation:
\begin{packed_itemize}
\item \textbf{Expanding participation in computing.} In my courses,
students from non-traditional and non-computational backgrounds are
recruited and motivated by use of accessible, relevant examples, and
promoting a collaborative, informal-by-design learning environment.

\item \textbf{Expanding collaborative environments in research.}
In an undergraduate research program I designed, the focus is on
engaging faculty and their graduate students in joint mentoring
of undergraduate researchers. Increasing the number of stakeholders and interactive-time brings undergraduate researchers up-to-speed faster, and is a forcing function for more research results. In an integrative center I've co-founded, we created the foundational integrated learning environment to foment and spark cross-disciplinary
collaborations.

\item \textbf{Dissemination of results and computational
tools.} Disseminating accessible learning materials
and general tools, to attract interest of both students and faculty
in other fields is a key priority. Using workshops, tutorials, on-line published
materials, I attempt to draw attention and interest of students and faculty to
available tools and interesting problems in machine learning and structured prediction.
\end{packed_itemize}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\out{
% establish the success of discriminative methods
\mypar{Supervised Learning and Structured Prediction.} The need to
analyze and make effective use of the vast amounts of data has made
machine learning indispensable in many fields of science, medicine
and engineering.
%The breadth of tasks addressed by machine learning
%is rapidly expanding within and beyond computer science.
Today, machine learning offers widely used statistical methods and
\textit{primary tools for building intelligent systems from
examples} in many fields:
computational linguistics%~\cite{mansch99},
computer vision%~\cite{forpon03},
robotics%~\cite{thrun2005},
to name
a few. At the fundamental level, building an intelligent system
means the machine is given a set of examples (these examples are
pairs of input and response, and can be "supervised"
"semi-supervised" or "partially supervised"). From these
"experiences" the machine learns a model (the model can be
"structured" or not). The learned model is later used to predict the
response to new inputs not previously seen in the original set of
examples.

\out{ \textit{Supervised learning}, a sub-field of machine learning
which automates learning from examples with precise pairings of
input and response, \out{addressing classification and regression
problems, } has perhaps seen most success, as software has become
essentially off-the-shelf, widely available and frequently used by
non-experts\cite{svmlite,weka,torch,spider}. In the last decade,
supervised learning has been extended beyond classification and
regression to \textit{structured prediction}. }

 In
\textit{structured prediction}, \textit{structure}  refers to the
assumption about entities in the problem domain: that they are
mutually dependent or constrained. These dependencies and
constraints reflect sequential, spatial or combinatorial structure
in the problem domain, and capturing such interactions is often as
important as capturing input-output dependencies~\cite{psd-book}.
Structured prediction offers improvement over classification and
regression because most real-world problems incorporate related,
non-independent entities: for example, natural language parsing,
machine translation, object segmentation, gene prediction, protein
alignment and numerous other tasks in computational linguistics,
speech, vision, biology. Recent advances in structured prediction
have brought about a unified view, efficient methodology and more
importantly, significant accuracy improvements for both classical
and novel real-world
problems~\cite{lafferty01crf,collins02discriminative,hofmannmm,taskar03max,taskar04thesis}.
For an overview of structured prediction, and how it tackles the
fundamental computational and statistical challenges arising in
structured models, the PI has co-edited a collection of
articles~\cite{psd-book}.

With the advent of these theoretical advances,
the burden of building intelligent systems has shifted from
brittle and murky `parameter tweaking' and rule-based programming to
more transparent and reusable data annotation.
In many real-world domains progress is limited due to the \textit{labeled data bottleneck}:
the massive burden of curating a set of examples in which the output variables
are precisely assigned to the input, exactly as we would like the intelligent
system to label them.
Paradoxically, we have accumulated more learning tools than can be applied since
we cannot produce the \textit{large, standardized, and precise expert} data required
to use these tools.
This proposal aims to address this bottleneck by
advancing a new framework within a burgeoning sub-field of
machine learning: \textit{structured partially supervised learning}.
At its core, this new framework aims to lift
restrictions on the kinds of "supervised" and "unsupervised"
given examples necessary in order to efficiently and accurately learn
models within the structured setting.
By contrast, previous work addressing this problem uses heuristic
procedures to complete imprecisely labeled or unlabeled examples
and reduce the problems to their supervised form.
The expected framework will offer:
1. direct, declarative methods: giving the user direct and declarative control over the semantics of the response variables.
2. theoretical soundness: establish theoretical conditions under which performance is comparable or close to supervised learning.
3. efficiency:
4. modeling flexibility: User can control the level of expressivity of the model, and incorporate less or more prior knowledge, without trading off tractability

\textbf{significance of project} The objective is to make structured
learning possible in domains where no large fully labeled examples
exist, but more flexible annotations arise naturally. Three domains
in which significant progress can be made are video search, ?, and
language translation. The tools delivered will be general (and hence
applicable to new fields), advance the current understanding of
structured prediction settings as well as the structure underlying
natural systems, \textbf{significance- why?} The tools arising from
this proposal will be flexible and efficient, and can be soundly
applied to new domains as they are generic machine learning tools

Lifting restrictions has the potential
of hastening the application of prediction models in such widely used
arenas as language translation, video annotation, and to transfer
 could potentially hasten the
appearance of prediction
By contrast, this proposal outlines a framework for a declarative direct method gives user direct and declarative control over the semantics of the latent variables.
"prove you're as-good-as": Establish theoretical conditions under which performance close to supervised can occur
"
"efficiency"
"expressive" "controlability" and "flexibility" - user can incorporate a lot more prior knowledge- without being intractable.

There's
My overarching goal
is to make partially supervised prediction as reliable and robust as structured prediction is currently.




The new framework proposed
would extend the problem settings and domains in which structured prediction
can be used.



At its core, this new framework aims to remove as many restrictions on the kinds of
"supervised" and "unsupervised" given examples necessary in order to efficiently and accurately learn
within structured partially supervised settings.
As such, this framework will address a problem known as the \textit{labeled data bottleneck}.

fine distinction making between supervised semi supervised and
structured partially supervised (!) complex outputs: more than a
single label for }


\out{
\section{OLD}

The need to analyze and make effective use of the vast amounts
of data has made machine learning indispensable in building
intelligent, adaptive systems. Major improvements in accuracy and
robustness, in computer vision and computational linguistics in
particular, have been propelled by advances in supervised machine
learning. However, there is a major obstacle to the deployment of
trainable systems: the limited availability of \textit{task-specific
human-annotated} data. Supervised learning assumes labeled training
data, which require extensive human expertise and consume tremendous
amounts of time.

Standard supervised learning assumes a labeled example as the basic
unit of supervision. One of the central questions of statistical
learning theory is the number of labeled examples needed to learn a
predictive model within a specified accuracy~\cite{vapnik_1995}.
State-of-the-art models for tasks in computational linguistics
(e.g., parsing, speech recognition, machine translation) and
computer vision (e.g., object detection and recognition, pose
estimation, scene parsing) often contain millions of
parameters~\cite{mansch99,forpon03}. As the complexity of the input,
the output, and the model increases, the number of required labeled
examples becomes prohibitively large for many tasks of interest. The
burden of annotation is often the most costly and painstaking
investment in applying supervised machine learning to any novel task
or a standard task in a novel setting. For example, 400 hours were
needed to label a single hour of speech at the phonetic
level~\cite{greenberg96switchboard}, 2 years to annotate 4,000
sentences with syntactic parse trees for the Chinese
Treebank~\cite{hwa05bootstrapping}, 4 to 7 years to annotate 50,000
sentences across a range of languages~\cite{abeille03treebanks}.
Moreover, models learned in one domain, such as a syntactic parser
for news articles, often fail miserably on the same task in
bio-medical or conversational text~\cite{Dredze07Frustratingly}.  As
number of tasks and domains of interest grows and evolves, direct
hand-labeling of data cannot scale.

% paragraph goal: availability of cheap, indirect, related annotation
%
The fundamental goal of this proposal is to systematically study how the reliance on a large fully labeled corpus can be eliminated by weakly labeled data.
%While purely unsupervised learning methods are unstable and
%difficult to guide towards desired predictions,
}

\out{

We would like to build \textit{structured prediction models} that
are able to parse scenes in video and documents in foreign languages
from such incomplete annotations.  \textit{Structured prediction
models} assume that variables of interest (detection of objects,
entities, actions, events) in the problem domain are mutually
dependent or constrained and attempt to predict them in a joint,
integrated manner~\cite{psd-book}. These dependencies and
constraints reflect sequential, spatial or combinatorial structure
in the problem domain, and capturing such interactions is often as
important as capturing input-output dependencies.  Recent advances
in supervised structured prediction have brought about a unified
view, efficient methodology and more importantly, significant
accuracy improvements for both classical and novel real-world
problems~\cite{lafferty01crf,collins02discriminative,hofmannmm,taskar03max,taskar04thesis}.




At present, supervised structured prediction methods cannot directly
leverage these large, weakly supervised datasets. Instead, ad hoc,
unstable and procedural methods are often being used without full
understanding of the properties of the data that ensure their
success. There is a pressing need for principled, declarative
methods that allow flexible supervision for structured prediction
models to leverage vast amounts of data without requiring
hand-labeling.


 In \textit{structured prediction}, \textit{structure} refers
to the assumption about entities in the problem domain: that they
are mutually dependent or constrained. These dependencies and
constraints reflect sequential, spatial or combinatorial structure
in the problem domain, and capturing such interactions is often as
important as capturing input-output dependencies~\cite{psd-book}.
Structured prediction offers improvement over classification and
regression because most real-world problems incorporate related,
non-independent entities: for example, natural language parsing,
machine translation, object segmentation, gene prediction, protein
alignment and numerous other tasks in computational linguistics,
speech, vision, biology. Recent advances in structured prediction
have brought about a unified view, efficient methodology and more
importantly, significant accuracy improvements for both classical
and novel real-world
problems~\cite{Lafferty+al-01:crf,collins02discriminative,hofmannmm,taskar03max,taskar04thesis}.
}
-independent entities: for example, natural language parsing,
machine translation, object segmentation, gene prediction, protein
alignment and numerous other tasks in computational linguistics,
speech, vision, biology. Recent advances in structured prediction
have brought about a unified view, efficient methodology and more
importantly, significant accuracy improvements for both classical
and novel real-world
problems~\cite{Lafferty+al-01:crf,collins02discriminative,hofmannmm,taskar03max,taskar04thesis}.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 


==> text/grant/math.tex <==
%% specific commands


%\newcommand{\E}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\Ehat}[1]{\widehat{\mathbb{E}}\left[#1\right]}
\newcommand{\mcal}[1]{\mathcal{#1}}
\newcommand{\mbf}[1]{\mathbf{#1}}
%\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\ceil}[1]{\left \lceil #1 \right \rceil}
\newcommand{\ang}[1]{\left \langle #1 \right \rangle}
\newcommand{\cY}{\mcal{Y}}
\newcommand{\cX}{\mcal{X}}
\newcommand{\cZ}{\mcal{Z}}
\newcommand{\cC}{\mcal{C}}
\newcommand{\cV}{\mcal{V}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\hG}{\hat{G}}
\newcommand{\tphi}{\tilde{\phi}}
\newcommand{\bw}{\mathbf{\theta}}
%\newcommand{\bft}{\mathbf{f}}
%\newcommand{\out}[1]{}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\ind}[1]{\mathbf{1}\left[#1\right]}
\newcommand{\Sc}{S_{\bx,bw}}
\newcommand{\hbw}{h_{\bw}}

\newcommand{\bbP}{\mathbb{P}}

%\newcommand{\mmarg}[1]{\theta^\star_x(#1)}   % max marginal score
\newcommand{\mmarg}[1]{\theta^\star(x,#1)}   % max marginal score
%\newcommand{\score}[1]{\theta_x(#1)}         % score function
\newcommand{\score}[1]{\theta(x,#1)}         % score function
\newcommand{\scoremax}{\theta^\star(x)}   % argmax score
%\newcommand{\scoremax}[0]{\theta^\star_x}   % argmax score
\newcommand{\ssp}[0]{\theta_x}              % score space
\newcommand{\sspRV}[0]{\theta_X}              % score space
\newcommand{\wit}[1]{y^\star(#1)}          % "witness"
%\newcommand{\thr}[0]{t_x(\theta,\alpha)}
\newcommand{\thr}[0]{t_\theta(x,\alpha)}
\newcommand{\thri}{t_{x^n}(\alpha)}
%\newcommand{\mmi}{\theta_x^\star(\lpart_i)}
\newcommand{\mmi}{\theta^\star(x,\lpart_i)}

\newcommand{\lparts}{y}
\newcommand{\lpart}{y}
\newcommand{\Lpart}{Y}
\newcommand{\Lparts}{Y}
\newcommand{\Lspace}{\mathcal{Y}}



\newcommand{\pmmarg}[1]{\theta_p^\star(x,#1)}   % max marginal score
\newcommand{\pscore}[1]{\theta_p(x,#1)}         % score function
\newcommand{\pscoremax}[0]{\theta_p^\star(x)}   % argmax score

\newcommand{\pmmargi}[1]{\theta_p^\star(x^n,#1)}   % max marginal score
\newcommand{\pscorei}[1]{\theta_p(x^n,#1)}         % score function
\newcommand{\pscoremaxi}[0]{\theta_p^\star(x^n)}   % argmax score


\newcommand{\pthr}[1]{t_p(#1,\alpha)}
\newcommand{\pthri}{t_p(x^n,\alpha)}

\newcommand{\suchthat}{\quad \textrm{ s.t. } \quad}
\newcommand{\mif}{\textrm{ if }}


%Kronecker features
\newcommand{\Kbar}{\mathbf{\bar{K}}}
\newcommand{\ybar}{\mathbf{\bar{y}}}
\newcommand{\xbar}{\mathbf{\bar{x}}}
\newcommand{\xBar}{\mathbf{\bar{\bar{x}}}}
\newcommand{\nll}{{\rm null}}


\newcommand{\Loss}{\mathcal{L}}
\newcommand{\LossZO}{\mathcal{L}_{01}}
\newcommand{\LossM}{\mathcal{L}_{\psi}}
\newcommand{\LossA}{\mathcal{L}_{\psi}}
\newcommand{\LossMAX}{\mathcal{L}^{max}_{\psi}}
\newcommand{\X}{\mathcal{X}}
%\newcommand{\E}{\mathbf{E}}
%\newcommand{\bw}{\mathbf{w}}
\newcommand{\bft}{\mathbf{f}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\ip}[2]{{#1}\cdot{#2}}
\newcommand{\Rgn}{\mathcal{R}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\vectornorm}[2]{\left|\left|#1\right|\right|_{2}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\Ind}{\mathbf{1}}
%\newcommand{\Ind}{\mathbf{1}}
%\newcommand{\argmax}{\mathop{\arg\max}}
\newcommand{\Q}{\mathcal{Q}}


\newcommand{\KL}{\mathop{\rm KL}}
\newcommand{\likelihood}{\mathcal{L}}
\newcommand{\Xp}{\mathbf{E}}
\newcommand{\XpD}{\mathbf{\widehat{E}}}


\newcommand{\Vones}[1]{\ensuremath{\mathbf{1}_{#1}}}
\newcommand{\eqdef}{\stackrel{\rm def}{=}}

\newcommand{\out}[1]{}
\newcommand{\denselist}{\itemsep 0pt\topsep-8pt\partopsep-8pt}
\newcommand{\mypar}[1]{\noindent{\bf #1.}}

%\renewcommand{\includegraphics}[2]{}

%% usual commands
%\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\todo}[1]{{\bf{TODO: #1}}}
%\newcommand{\todo}[1]{}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}

%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

% \newenvironment{definition}[1][Definition.]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% \newenvironment{example}[1][Example]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
% \newenvironment{remark}[1][Remark]{\begin{trivlist}
% \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

%\newcommand{\qed}{\nobreak \ifvmode \relax \else
%      \ifdim\lastskip<1.5em \hskip-\lastskip
%      \hskip1.5em plus0em minus0.5em \fi \nobreak
%      \vrule height0.75em width0.5em depth0.25em\fi}

\newcommand{\qed}{\hfill \ensuremath{\Box}}

%\newcommand{\qed}{\ensuremath{\Box}}

\newcommand{\boxedequation}[2]{%
  \[\fbox{
      \addtolength{\textwidth}{-2\fboxsep}%
      %\addtolength{\linewidth}{-2\fboxsep}%
      \addtolength{\linewidth}{-2\fboxrule}%
      \begin{minipage}{#1\linewidth}%
      \begin{equation}#2\end{equation}%
      \end{minipage}%
    }\]%
}
\newcommand{\boxedeqnarray}[1]{%
  \[\fbox{%
      %\addtolength{\linewidth}{-2\fboxsep}%
      %\addtolength{\linewidth}{-2\fboxrule}%
      \begin{minipage}{0.7\linewidth}%
      \begin{eqnarray*}#1\end{eqnarray*}%
      \end{minipage}\nonumber%
    }\]%
}
\newcommand{\boxedeqnalign}[1]{%
  \[\fbox{%
      %\addtolength{\linewidth}{-2\fboxsep}%
      %\addtolength{\linewidth}{-2\fboxrule}%
      \begin{minipage}{0.99\linewidth}%
      \begin{align}#1\end{align}%
      \end{minipage}\nonumber%
    }\]%
}

%abbreviations
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
%\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
%\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}

\def\ie{\emph{i.e}.}
%\makeatother



%% specific commands
\newcommand{\trans}[1]{{#1}^{\ensuremath{\mathsf{T}}}}           % transpose
\newcommand{\st}{\quad\textrm{s.t.}\quad}                        % s.t. for such that
\newcommand{\mvec}{\textrm{vec}}
\newcommand{\nchoosek}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}  %use binom instead...



\newenvironment{packed_itemize}{
\vspace{-6pt}
\begin{itemize}
  \setlength{\leftmargin}{1em}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}
{\end{itemize}
\vspace{-6pt}
}

% mands
% \newcommand{\trans}[1]{{#1}^{\ensuremath{\mathsf{T}}}}           % transpose
% \newcommand{\st}{\quad\textrm{s.t.}\quad}                        % s.t. for such that
% \newcommand{\mvec}{\textrm{vec}}
% \newcommand{\

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 


==> text/grant/plan.tex <==
\section{Research Plan}


%$$
%{\rm P} \mathbb{R} \imath \mathfrak{M}\mathcal{L}
%$$

We first review the structured prediction framework and then 
propose several types of structured prediction cascades,
one based on increasing Markov order~\cite{cascades},
and another on increasing spatial resolution~\cite{sapp10cascades}. 
We motivate the use of max-marginals as the key ingredient
in deciding how to filter the complex space of predictions
and pass information between layers of the cascade. 
We present a novel learning formulation that balances
efficiency and accuracy.  Preliminary results with this formulation
are quite promising and suggest further generalizations, analysis and  
applications of the cascade framework.

\mypar{Structured Prediction}
Given an input space $\cX$, output space $\cY$, and a training set $
\{\ang{x^1,y^1},\dots,\ang{x^N,y^N}\}$ of $N$ independent and
identically-distributed ({i.i.d.}) random samples from a joint
distribution $D(X,Y)$, the standard supervised learning task is to learn a
hypothesis $h: \cX \mapsto \cY$ that minimizes the expected loss
$\E{D}{ \cL\left(h(x) , y\right)}$ for some non-negative loss function
$\cL : \cY \times \cY \rightarrow \reals^+$.

We consider the case of structured classification where $Y$ is a $\ell$-vector of variables and $\cY = \cY_1
\times \dots \times \cY_\ell$.  In many settings, the number of
random variables $Y$ differs depending on input $X$ (for example, length of the sentence in part of speech tagging), but for simplicity of notation, we assume a fixed number $\ell$ here.
We denote the components of $y$ as $y = \{y_1, \dots, y_\ell\}$, where $y_i \in \{1, \dots, K\}$.
The linear hypothesis class we consider is of the form:
\begin{equation}
  \label{eq:linear_classifiers}
  \hbw(x) = \argmax_{y\in\cY} \bw^\top\bft(x,y)
\end{equation}
where $\bw \in \reals^p$ is a vector of parameters and $\bft:
\cX\times\cY\mapsto\reals^p$ is a function mapping $(x,y)$ pairs to a
set of $p$ real-valued features. We further assume that $\bft$
decomposes over a set of cliques $\cC \subseteq \bbP\{X, Y\}$
(where $\bbP$ is a powerset):
\begin{equation}
  \label{eq:feature_sep}
  \bw^\top\bft(x,y) = \sum_{c \in \cC} \bw^\top\bft_c(x,y_c).
\end{equation}
Above, $y_c$ is an assignment to the subset of $Y$ variables in the clique $c$ and we will use $\cY_c$ to refer to the set all assignments to the clique. By considering different cliques over $X$ and $Y$, $\bft$ can represent arbitrary interactions between the components of $x$ and $y$. Thus, evaluating $\hbw(x)$ is not always tractable, and
computational resources limit the expressiveness of the features that
can be used.

For example, a first order Markov sequence model has cliques $\{Y_i,
Y_{i+1}, X\}$ to score features depending on emissions $\{X,Y_i\}$ and
transitions $\{Y_i, Y_{i+1}\}$:
 $%\begin{equation}
\bw^\top\bft(x,y) = \sum_{i=1}^{\ell-1} \bw^\top\bft_i(x,y_i,y_{i+1}).
$ %\end{equation}
For the first order model, evaluating \eqref{eq:linear_classifiers}
requires $O(K^2\ell)$ time using the Viterbi decoding algorithm. For
an order-$d$ Markov model, with cliques over $\{y_i, \dots, y_{i+d},
x\}$, inference requires $O(K^{d+1}\ell)$ time.

Several structured prediction methods have been proposed for learning
$\bw$, such as conditional random fields~\cite{lafferty01crf},
structured perceptron~\cite{collins_discriminative_2002}, hidden
Markov support vector machines~\cite{altun03hmsvm} and max-margin
Markov networks~\cite{taskar03max}.  Our focus here is instead on
learning a cascade of increasingly complex models in order to
efficiently construct models that would otherwise be too expensive or 
intractable to learn and use.

\mypar{Markov Order Cascades}
We will discuss how to learn a cascade of models below, but
first we describe the cascaded inference procedure.  The basic notion behind
our approach is very simple: at each level of the cascade, we receive
as input a set of possible clique assignments corresponding to the
cliques of the current level. Each level further filters this set of
clique assignments and generates a set of possible clique assignments
which are passed as input to the next level. Note that each level is
able to prune further than the preceding level because it can consider
higher-order interactions. At the end of the cascade, the most complex
model chooses a single prediction as usual, but it needs only consider
the clique assignments that have not already been pruned. Finally,
pruning is done using clique max-marginals, for reasons which we
describe below.


An example of a cascade for sequential prediction using Markov models
is shown is Figure \ref{fig:schematic}. A $d$-order Markov model has
maximal cliques $\{X, Y_i, Y_{i+1}, \dots, Y_{i+d}\}$. We can consider
a cascade of sequence models of increasing order as a set of bigram
models where the state space is increasing exponentially by a factor
of $K$ from one model to the next.  Given a list of valid assignments
$\cV^i$ in a $d$-order model, we can generate an expanded list of
valid assignments $\cV^{i+1}$ for a $(d+1)$-order model by
concatenating the valid $d$-grams with all possible additional states.

% For example, a $1$st-order (bigram) model scores cliques $\{X,Y_i,
% Y_{i+1}\}$, while a $2$nd-order (trigram) mode scores cliques $\{X,
% Y_i, Y_{i+1}, Y_{i+2}\}$. hus, we can consider a cascade of sequence
% models of increasing order as a set of bigram models where the state
% space is increasing exponentially by a factor of $K$ from one model to
% the next.  Given a list of valid assignments $\cV^i$ in a $d$-order
% model, we can generate an expanded list of valid assignments
% $\cV^{i+1}$ for a $(d+1)$-order model by concatenating the valid
% $d$-grams with all possible additional states.
% % We will discuss how to learn such a cascade in section
% \ref{sec:learning}, but first, we define its operation at inference
% time. The basic notion behind our approach is very simple: at each
% level of the cascade, we start with the output space filtered by a
% simpler model in the previous level and further filter the space by
% considering higher-order interactions. At the end of the cascade, a
% standard structured prediction model with the most complex
% interactions chooses an assignment over the final filtered space. A
% filtered space of outputs is represented by a set of valid clique
% assignments and the decision to prune a clique assignment is based on
% its max-marginal: the score of the best assignment consistent with
% this clique assignment.  The reason for using max-marginals is explained below.

%\begin{figure}
\begin{wrapfigure}{r}{0.50\textwidth}
\vspace{-0.5ex}
  \centering
%  \includegraphics[width=0.45\textwidth]{figs/exp_factors_sparse.png}
  \vskip -2mm
  \caption{\small Schematic of a structured prediction cascade using
    unigram, bigram, and trigram Markov sequence models. Models are
    represented as factor graphs; as order increases, the state space
    grows, but the size of the filtered space remains small (filled
    area).}
  \label{fig:schematic}
%\end{figure}
\end{wrapfigure}
More generally, for a given input $x$, for each maximal clique $c\in
\cC$ in the current level of the cascade, we have a list of valid
assignments $\cV_c \subseteq \cY_c$. Inference is performed only over
the set of valid clique assignments $\cV = \bigcup_{c \in \cC}
\cV_c$. Using the filtering model $\bw$ of the current cascade level,
the clique assignments in $\cV_c$ are scored by their max-marginals,
and a threshold $t$ is chosen to prune any $y_c \in \cV_c$ with a
score less than the threshold. The sets $\cV$ are then passed to the
next level of the cascade, where higher-order cliques consistent with
unpruned cliques are constructed. If we can eliminate at least a
fraction of the entries in $\cV$ on each round of the cascade, then
$|\cV|$ decreases exponentially fast and the overall efficiency of
inference is controlled.

Thus, to define the cascade, we need to define: (1) the set of models
to use in the cascade, and (2) a procedure to choose a threshold
$t$.  We fist discuss a cascade of increasing Markov order, which is
very useful for sequence labeling tasks.  Below we also
present a cascade over spatial resolution.

To define a set of models for the Markov order cascade, we require only that
the sets of cliques of the models form a nesting sequence. The cliques
of the models must satisfy the relation, 
$%\begin{equation}
  \label{eq:nested}
  \cC^1 \subseteq \cC^2 \subseteq \dots \subseteq \cC^d,
%\end{equation}
$ where $\cC^i$ is the set of cliques of the $i$'th model of the
cascade. In other words, every clique assignment $y_c$ of the $i$'th
model is contained in at least one clique assignment $y_c'$ of the
$(i+1)$'th model. This property allows for the use of increasingly
complex models as the depth of the cascade increases. As long as
\eqref{eq:nested} holds, a simple and intuitive mapping from the set
of valid cliques of the $i$'th model $\cV^i$ to a corresponding set of
valid cliques of the $(i+1)$'th model, $\cV^i$:
\begin{equation}
  \label{eq:cliquemapping}
  \cV^{i+1}_c = \{ y_c \in \cY_c \mid \forall c' \in \cC^i, c' \subseteq c, y_{c'} \in \cV_{c'}^i\}
\end{equation}
This is the set of clique assignments $y_c$ in the $(i+1)$'th model
for which all consistent clique assignments $y_{c'}$ for subcliques
$c' \in \cC^i$ have not been pruned by the $i$'th
model.

In order to filter clique assignments, we use their
\textit{max-marginals}, which we justify shortly.  We introduce the shorthand $\score{y} =
\bw^\top\bft(x,y)$ for the cumulative score of an output $y$, and
define the max marginal $\mmarg{y_c}$ as follows:
$$\mmarg{y_c} \triangleq \max_{y'\in \cY} \;\;\{ \score{y'} : y'_c = y_c\}.$$
Computing max-marginals can be achieved using the same dynamic
programming inference procedures in factor graphs as would be used to
evaluate \eqref{eq:linear_classifiers}.  

Note that pruning using max-marginals
\textit{guarantees} that at the next level, there will be at least one 
\textit{consistent global prediction}.  It is easy to create examples where using standard marginals (where max is replaced by sum
and the score is exponentiated) and may create a situation that
there are no consistent sequences left (going from second order cliques to third order cliques). 
Pruning using max-marginals guaranties
that at least the highest-scoring path is not pruned.
Most importantly, max
marginals satisfy the following simple property:
\begin{lemma} [Safe Filtering]
  \label{prop:pruning}
  If $\score{y} \ge t$ then for all $c$,  $\mmarg{y_c}\ge t $ and no part of $y$ is pruned.
\end{lemma}
The lemma follows from the fact that the max marginal of any
clique assignment $y_c$ consistent with $y$ is at least the score of
$y$. A consequence of Lemma~\ref{prop:pruning} is that on training data, a sufficient
condition for the target output $y$ not to be pruned is that the
threshold $t$ is lower than the score $\score{y}$. Note that a similar
condition does not generally hold for standard sum-product marginals
of a CRF (where $p(y|x)\propto e^{\score{y}}$), which motivates our
use of max-marginals.

The next component of the inference procedure is choosing a threshold
$t$ for a given input $x$.  Note that the threshold cannot be defined
as a single global value but should instead depend strongly on the
input $x$ and $\score{\cdot}$ since scores are on different scales. We
also have the constraint that computing a threshold function must be
fast enough such that sequentially computing scores and thresholds for
multiple models in the cascade does not adversely effect the
efficiency of the whole procedure. One might choose a quantile
function to consistently eliminate a desired proportion of the max
marginals for each example. However, quantile functions are
discontinuous in the score function, and we instead approximate a
quantile threshold with a smooth {\em mean-max} threshold
function, defined as a convex combination of the mean of the max
marginals and the maximum score $\scoremax = \max_y \score{y}$,
\begin{equation}
  \label{eq:meanmax}
  \thr = \alpha \scoremax + (1-\alpha)\frac{1}{|\cV|} \sum_{c\in\cC, y_c\in V_c} \mmarg{y_c}.
\end{equation}
Choosing a mean-max threshold is therefore choosing $\alpha \in
[0,1)$. Note that $\thr$ is a convex function of $\score{\cdot}$ (in
fact, piece-wise linear), which combined with Lemma
\ref{prop:pruning} will be important for learning the filtering models
and analyzing their generalization. In our experiments, we found that
the distribution of max marginals was well centered around the mean,
so that choosing $\alpha \approx 0$ resulted in $\approx50\%$ of max
marginals being eliminated on average. As $\alpha$ approaches $1$, the
number of max marginals eliminated rapidly approaches $100\%$. 
Cross-validation can be used to determine the optimal $\alpha$ given a computational
budget.

\mypar{Pictorial Structure Cascades}
We first summarize the basic pictorial structure model and then
describe the inference and learning in the cascaded pictorial structures
using spatial resolution abstraction.
Classical pictorial structures are a class of graphical models where the nodes of the graph represents object parts, and edges between parts encode pairwise geometric relationships.  For modeling human pose, the standard PS model decomposes as a tree structure into unary potentials (also referred to as appearance terms) and pairwise terms between pairs of physically connected parts.  Figure~\ref{fig:ps} shows a PS model for 6 upper body parts, with lower arms connected to upper arms, and upper arms and head connected to torso.  In previous work~\cite{devacrf,felz05,ferrari08,posesearch,andriluka09}, the pairwise terms do not depend on data and are hence referred to as a spatial or structural prior.
%\begin{figure}[]
%\begin{center}
%\centerline{\includegraphics[width=0.75\columnwidth]{data/model_parameters2.pdf}}
%\caption{Basic upper-body model with part state $l$ and part support rectangle of size $(w,h)$.}
%\label{fig:ps}
%\end{center}
%% \vskip -0.5in
%\end{figure}
The state of part $\Lpart_i$, denoted as $\lpart_i \in \Lspace_i$, encodes the joint location of the part in image coordinates and the direction of the limb as a unit vector: $\lpart_i = [\lpart_{ir} \; \lpart_{ic} \; \lpart_{iu} \; \lpart_{iv}]^T$. The state of the model is the collection of states of $\ell$ parts: $p(\Lparts = \lparts) = p(\Lpart_1 = \lpart_1, \ldots, \Lpart_\ell= \lpart_\ell)$.  The size of the state space for each part, $|\Lspace_i|$, is the number of possible locations in the image times the number of pre-defined discretized angles. For example, standard PS implementations typically model the state space of each part in a roughly $100 \times 100$ grid for $\lpart_{ir} \times \lpart_{ic}$, with 24 different possible values of angles, yielding $|\Lspace_i| = 100 \times 100 \times 24 = 240,000$. The standard PS formulation (see~\cite{felz05}) is usually written in a log-quadratic form:
\begin{align}
p( \lparts | x) &\propto \prod_{ij} \exp(-\frac{1}{2}||\Sigma_{ij}^{-1/2}(T_{ij}(\lpart_i) - \lpart_j - \mu_{ij})||_2^2)  \times \prod_{i=1}^M \exp(\mu_i^T\phi_i(\lpart_i,x))
\label{eqn:standard_ps}
\end{align}
The parameters of the model are $\mu_i,\mu_{ij}$ and $\Sigma_{ij}$, and $\phi_i(\lpart_i,x)$ are features of the (image) data $x$ at location/angle $\lpart_i$.  The affine mapping $T_{ij}$ transforms the part coordinates into a relative reference frame.  The PS model can be interpreted as a set of springs at rest in default positions $\mu_{ij}$, and stretched according to tightness $\Sigma^{-1}_{ij}$ and displacement $\phi_{ij}(\lparts) = T_{ij}(\lpart_i) - \lpart_j$.  The unary terms pull the springs toward locations $\lpart_i$ with higher scores $\mu_i^T\phi_i(\lpart_i,x)$ which are more likely to be a location for part $i$.
%\subsection{Basic PS Model}
\begin{wrapfigure}{r}{0.40\textwidth}
%\begin{floatingfigure}[lt]{0.52\columnwidth}
\vspace{-0.5cm}
\begin{center}
%\centerline{\includegraphics[width=0.4\columnwidth]{figs/model_parameters.pdf}}
\vspace{-0.5cm}
\caption{\small Basic PS model with state $y_i$ for a part $Y_i$.}
\label{fig:ps}
\end{center}
\vspace{-1cm}
%\end{floatingfigure}
\end{wrapfigure}

This form of the pairwise potentials allows inference to be performed faster than $O(|\Lspace_i|^2)$:  MAP estimates $\argmax_{\lparts} p(\lparts | x)$ can be computed efficiently using a generalized distance transform for max-product message passing in $O(|\Lspace_i|)$ time.  Marginals of the distribution, $p(\lpart_i | x)$, can be computed efficiently using FFT convolution for sum-product message passing in $O(|\Lspace_i| \log |\Lspace_i|)$~\cite{felz05}.

While fast to compute and intuitive from a spring-model perspective, this model has two significant limitations.  One, the pairwise costs are unimodal Gaussians, which cannot capture the true multimodal interactions between pairs of body parts.  Two, the pairwise terms are only a function of the geometry of the state configuration, and are oblivious to the image cues, for example, appearance similarity or contour continuity of the a pair of parts.

\label{subsec:our_ps}
We chose instead to model part configurations as a linear structured model:
\begin{align}
\bw^\top\bft(x,y)  =  \sum_{ij}  \bw^{\top} \bft(x,\lpart_i,\lpart_j) +
\sum_i  \bw^{\top} \bft(x,\lpart_i) .
\label{eqn:our_ps}
\end{align}
The parameters of our model are the pairwise and unary weight vectors corresponding to the pairwise and unary feature vectors, but for brevity, we stack all the parameters and features into vectors using notation $\bw^\top\bft(x,y)$. The key differences with the classical PS model are that (1) our pairwise costs allow data-dependent terms, and (2) we do not constrain our parameters to fit any parametric distribution such as a Gaussian.  For example, we can express the pairwise features used in the classical model as $\lpart_{i} \cdot \lpart_{i} \text{, } \lpart_{j}\cdot\lpart_{j} \text{ and }  \lpart_{i}\cdot\lpart_{j}$ without requiring that their corresponding weights can be combined into a positive semi-definite covariance matrix.

In this general form, inference cannot be performed efficiently with distance transforms or convolution, and we rely on standard $O(|\Lspace_i|^2)$ dynamic programming techniques to compute the MAP assignment or part marginals.  Many highly-effective pairwise features one might design would be intractable to compute in this manner for a reasonably-sized state space---for example an $100\times100$ image with a part angle discretization of $24$ bins yields $|\Lspace_i|^2 = 57.6$ billion part-part hypotheses.

However, we can circumvent this issue via a cascade of models which aggressively prune the state space at each stage typically without discarding the correct sequence.  
We can start with a severely coarsened state space and use fast unary detectors and geometric features to perform quick exhaustive inference on the coarse state space.  
Each level of the cascade uses inference to identify which states to prune away and the next level refines the spatial/angular resolution on the unpruned states.
After the state space is pruned, we are left with a small enough number of states to be able to incorporate powerful data-dependent pairwise and unary features into our model
(see Fig.~\ref{fig:overview}).
\begin{figure}[t]
\begin{center}
%\includegraphics[width=0.9\textwidth]{figs/overview.png}
\end{center}
\vspace{-.5cm}
\caption{\label{fig:overview} \small Overview: A discriminative coarse-to-fine cascade 
of pictorial structures filters the pose space so that expressive and 
computationally expensive cues can be used in the final pictorial structure.  
Shown are 5 levels of our coarse-to-fine cascade for the right upper and lower 
arm parts.  Green vectors represent position and angle of unpruned states, the 
downsampled images correspond to the dimensions of the respective state space, 
and the white rectangles represent classification using our final model.}
\end{figure}


\mypar{Learning Cascade Parameters}
When learning a cascade, we have two competing objectives that we must trade off,
accuracy and efficiency: we want to minimize the number of errors incurred by each
level of the cascade  and maximize the number of filtered max marginals.  As we stated above, we prune the states whose max-marginal score is lower than a data-specific threshold $\thr$: $y_i$ is pruned if $\mmi < \thr$.  (For simplicity of notation, we use the pictorial structure cascade for exposition.) This threshold is defined as a convex combination of the MAP assignment score and the mean max-marginal score, meant to approximate a percentile threshold: $t_{\theta}(x,\alpha)= \alpha \theta^\star(x) + (1-\alpha)\frac{1}{\sum_{i=1}^\ell|\Lspace_i|}\sum_{i=1}^\ell\sum_{\lpart_i \in \Lspace_i} \mmi,$ where $\alpha\in[0,1]$ is a parameter to be chosen that determines how aggressively to prune. When $\alpha = 1$, only the best state is kept, which is equivalent to finding the MAP assignment.  When $\alpha = 0$ approximately half of the states are pruned (if the median of max-marginals is equal to the mean) .  The advantage of using  $\thr$ is that it is convex in $\theta$, and leads to a convex formulation for parameter estimation of a single cascade layer that trades off the proportion of incorrectly pruned states with the proportion of unpruned states.
Note that  $\alpha$ controls efficiency, so we focus on learning the parameters $\theta$ that 
minimize the number of errors for a given filtering level $\alpha$.   The learning formulation uses a simple fact about max-marginals and the definition of $t_{\theta}(x,\alpha)$
to get a handle on errors of the cascade:
if $\theta(x,\lparts) > t_{\theta}(x,\alpha)$, then for all i, $\mmi >  t_\theta(x,\alpha)$, so no part state of $\lparts$ is pruned.   Given an example $(x,\lparts)$,
this condition $\theta(x,\lparts) > t_\theta(x,\alpha)$ is sufficient to ensure that no correct part is pruned.

To learn one level of the structured cascade model $\theta$ for a fixed $\alpha$, we try to minimize 
the number of correct states that are pruned on training data by solving the
following convex margin optimization problem given $N$ training examples $(x^n,\lparts^n)$:
\begin{equation}
  \label{eq:convex_opt}
 \min_{\theta} \;\;\;\ \frac{\lambda}{2}||\theta||^2 + \frac{1}{N}\sum_{n=1}^N H(\theta;x^n,\lparts^n),
\end{equation}
where $H$ is a hinge upper bound 
$H(\theta;x,\lparts) = \max\{0, 1 + t_\theta(x,\alpha) - \theta(x,\lparts)\}$.
The upper-bound $H$ is a hinge loss measuring the margin between the
filter threshold $t_{\theta}(x^n,\alpha)$ and the score of the truth
$\theta(\lparts^n,x^n)$; the loss is zero if the truth scores above
the threshold by margin $1$.  Note that since $t_{\theta}(x^n,\alpha)$ is convex in $\theta$, the entire objective is
convex and can be optimized in many ways.  In particular,  we can solve \eqref{eq:convex_opt} using stochastic
sub-gradient~\cite{ratliff2007online}, which requires standard max-sum inference to compute the sub-gradient.  Successive layers
of the cascade are learned on the filtered output of the previous layer.
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-0.7cm}
%\begin{figure}[t]
\begin{center}
%\includegraphics[width=0.5\textwidth]{figs/casscades.pdf}
\caption{\small Upper right: Simple detector-based pruning by thresholding (for the lower right arm) yields many hypotheses far way from the true one. Lower row: The cascade, however, exploits global information to perform better pruning.}
\label{fig:cascade_pruning}
\end{center}
\vspace{-0.7cm}
%\end{figure}
\end{wrapfigure}
\mypar{Comparison to simple detector-based pruning} A naive approach used in a variety of applications is to simply subsample states by thresholding outputs of part or sparse feature detectors, possibly combined with non-max suppression.  Our approach, based on pruning on max-marginal values in a first-order model, is more sophisticated: for articulated parts-based models, strong evidence from other parts can keep a part which has weak individual evidence, and would be pruned using only detection scores.  The failure of prefiltering  part locations in human pose estimation is also noted by~\cite{andriluka09}, and serves as the primary justification for their use of the dense classical PS. This is illustrated in Figure~\ref{fig:cascade_pruning} on an example image from~\cite{ferrari08}.


%\subsection*{Preliminary results}
\mypar{Preliminary results: pose estimation} 
In~\cite{sapp10cascades}, we evaluated our approach on the publicly available pose dataset~\cite{eichner09}.  
%and PASCAL Stickmen datasets
The introduced CPS model allows us to capture appearance, geometry and shape information of parts and pairs of parts in the final level of the cascade --- much richer than the standard geometric deformation costs and texture filters of previous models. 
We use the same accuracy metric and the upper body detection windows provided with the dataset as input to localize and scale normalize the images before running our experiments as in~\cite{eichner09,ferrari08,andriluka09}. In preliminary results shown in Table~\ref{tab:overall}, we improve over our own  earlier work (which is much more compute intensive)~\cite{sapp10adaptive} on upper arms and significantly outperforming other works.  We also compare to a much simpler approach, inspired by~\cite{pff-cascade} (detector pruning + rich features):  We prune by thresholding each unary detection map individually to obtain the same number of states as in our final cascade level, and then apply our final model with rich features on these states. This baseline performs significantly worse than our method (performing about as well as a standard PS model as reported in~\cite{sapp10adaptive}).  This makes a strong case for using max-marginals (e.g., a global image-dependent quantity) for pruning, 
%as well as learning how to prune safely and efficiently, 
rather than using static thresholds on individual part scores as in~\cite{pff-cascade}.
\begin{wraptable}{r}{0.5\textwidth}
\vspace{-.3cm}
\begin{center}
{\scriptsize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
method &	torso &	head	 &	u. arms	 &	l. arms	 &	total \\
% &	&		 &	arms	 &	arms	 &	\\ \hline
\hline
%\textbf{Buffy} & & & & &\\
%\hline
%Ferrari et al.~\cite{ferrari08}	 &	-	 &	-	 &	-	 &	-   &	 61.4 \\
%\hline
Ferrari et al.~\cite{posesearch}	 &	-	 &	-	 &	-	 &	-		 &	74.5 \\
\hline
Andriluka et al.~\cite{andriluka09}	 &	90.7	 &	95.5	 &	79.3	 &	41.2	 &		73.5 \\
\hline
Eichner et al.~\cite{eichner09}		 &	98.7 	 &		97.9		 &	82.8	& 59.8	 &	80.1 \\
\hline
Detector pruning &		99.6	&	87.3&		90.0	&	55.3 	&		79.6 \\
\hline
APS~\cite{sapp10adaptive}	&	100		 &	100		 &	91.1 &		65.7	 &	85.9 \\
\hline
CPS (ours)	&	100	&	96.2	&	95.3	&	63.0	& 	85.5 \\
\hline
\out{
\hline						
\textbf{PASCAL stickmen} & & & & & \\
\hline
Eichner et al.~\cite{eichner09}		&	97.22	&	88.60	&	73.75	&	41.53		&	69.31 \\
\hline
APS~\cite{sapp10adaptive}	&	100	&	98.0	&	83.9	&	54.0		&	79.0 \\
\hline
CPS (ours)	&	100	&	90.0	&	87.1	&	49.4		&	77.2 \\
\hline
}
\end{tabular}
}
\caption{\label{tab:overall} \small We strongly outperform previous methods except our own computationally expensive APS model.}
\end{center}
\vspace{-0.3cm}
\end{wraptable}

Our previous method~\cite{sapp10adaptive} is the only other PS method which incorporates image information into the pairwise term of the model.  However it is still an exhaustive inference method.  Assuming all features have been pre-computed, inference in~\cite{sapp10adaptive} takes an average of 3.2 seconds, whereas inference using the sparse set of states in the final stage of the cascade takes on average 0.285 seconds---a speedup of 11.2x\footnote{Run on an Intel Xeon E5450 3.00GHz CPU with an $80\times80\times24$ state space averaged over 20 trials.~\cite{sapp10adaptive} uses MATLAB's optimized fft function for message passing.}.

\mypar{Preliminary results: handwritng recognition} In~\cite{cascades}, we evaluated the accuracy 
of the cascade using a  handwriting recognition dataset~\cite{taskar03max}.  Our objective was to measure the improvement in predictive accuracy as
higher order models were incorporated into the cascade. The
cascade consisted of four Markov models of increasing order. Pixels
are used as features for the lowest order model, and 2,3, and 4-grams
of letters are the features for the three higher order models,
respectively. We found that the use
of higher order models dramatically increased accuracy of the
predictions, raising accuracy at the character level above 90\% and more
than tripling the word-level accuracy. Furthermore, the cascade
reduced the search space of the 4-gram model by 5 orders of magnitude,
while incurring only 3.41\% filtering error.


\mypar{Decomposable Cascades}
We have so far assumed  exact inference is
possible on the filtered set of assignments throughout the cascade. 
This assumption relied on the sequential or tree structure of the models.
In many problems, however, the desired structure might not have low-treewidth.
Consider articulated pose estimation in video: a desirable model for the tracking problem would consist of a
set of state variables for each part (limbs, torso, head) that are 
connected  in each frame (like pictorial structures) and also
across frames to model persistence/velocity of each part (see Fig~\ref{fig:dbn}, left).
Just as in Dynamic Bayesian Networks, inference in such a model
is of exponential complexity in the number of parts (state variables)~\cite{koller2009probabilistic}.

We propose decomposing the temporal dependencies in the fully
connected model and approximating the
intractable model with an ensemble of tractable models (Fig.~\ref{fig:dbn}). 
Each model in the ensemble captures all the spatial dependencies in each frame but
the temporal persistence of only a single state
variable and so inference remains tractable. Below we discuss how the outputs
of the inference of each model are combined for filtering out assignments. 
Other ways to break up the model into tractable pieces are of course possible.
We refer to this collection of tractable models as the {\em decomposition ensemble} 
and propose to extend the cascade framework to operate with such
ensembles. Each layer of the cascade will use multiple models
to prune the output space for the next layer with higher spatial resolution
or higher Markov order.
Our proposed method will jointly learn parameters for all the models in the
level's ensemble, yet require only a linear increases in resources during learning. 

\begin{figure}[h]
  \vspace{-0.7cm}
  \centering
%    \input{figs/dbn.tex}
    \caption{\small Learning to filter with complex dynamics by a
      decomposition ensemble. Left: the fully connected, intractable
      tracking model. Right: the decomposition ensemble of models in
      which each state variables temporal persistence is modeled separately.}
  \label{fig:dbn}
  \vspace{-0.3cm}
\end{figure}

The proposed ensemble consists of $P$
models (and state variables), where the $p$'th model incorporates persistence of the
$p$'th variable through time.  All the models share the same variables,
but have a different set of edges. We learn to filter using the ensemble
jointly by summing the max marginals of each model computed separately,
 and we compute a
filtering threshold on the summed max marginals. We let
$\pscore{\cdot}$, $\pmmarg{\cdot}$, $\pscoremax$ and $\pthr{x}$ be the
score, max marginal, max score, and threshold of the $p$'th model,
respectively.  On a given input $x$, an assignment to part $i$ in frame $t$ will be filtered
by the ensemble if the sum of thresholds is larger than the sum of max-marginals at time $t$ for part $i$: 
$\sum_p \pthr{x} > \sum_{p} \pmmarg{y_{it}}$.
The advantage of summing the marginals in this manner is that a
weakness in one member of the ensemble on a particular example can be
compensated for by the strengths of the other models. Although one or
more of the individual scores $\pmmarg{y_{it}}$ may be under threshold
$\pthr{x}$, the ensemble can still avoid a mistake if another member
scores $y_{it}$ high enough to compensate. In pose estimation problem, this may
occur if the model part with the strongest visual cues for continuity
through time varies from example to example; e.g., in scenes where the
actor faces the camera, modeling a smooth face trajectory is useful,
while if the face is obscured or the actor is facing away from camera,
modeling a smooth arm trajectory may be more accurate. 
The most useful property of the cascade framework
carries over to the decomposition ensemble setting. We can derive a
similar ``safe filtering'' lemma for joint marginals, as follows:
if $\sum_p \pscore{y} > t$ then no part of $y$ is pruned.
Hence, we can recast the cascade optimization problem
 using the sums of $P$ max marginals as follows:
\begin{equation}
  \label{eq:joint_sc}
  \min_{\theta_1, \dots, \theta_P} \frac{\lambda}{2} \sum_p ||\theta_p||^2 
  +  \frac{1}{N}\sum_{n=1}^N \max\left(0, 1+ \sum_p \pthri - \pscorei{y^n}\right).
  %\suchthat \sum_p \pscorei{y^i} \ge \sum_p \pthri + \ell^i, \quad \forall i = 1, \dots, n.
\end{equation}
(The above formulation assumes all example sequences are of equal length,
otherwise the hinge loss offset needs to scale with the length.)
Once again, stochastic subgradient can be used to optimize this convex loss,
where we need to perform inference in each model separately to compute
the subgradient. Note that an alternative to \eqref{eq:joint_sc} using the cascade framework
would be to simply learn a cascade of $P$ models, but in that
approach, mistakes are cumulative, and there is no way for any model
to compensate for the weaknesses of the others.  The idea of
decomposing models into tractable sub-models is closely related to 
dual decomposition~\cite{bertsekas99nonlinear,komodakis2007mrf} and variational 
methods~\cite{jordan99introduction,trw,wainwright03variational}
for approximate inference.  It is likely to be useful beyond DBN-like
temporal models, but also for grid-type and more general graph topologies.

\mypar{Theoretical analysis}
Our initial analysis in~\cite{cascades} derived a generalization theorem that  provides theoretical justification for
the definitions of the hinge-type loss function of the structured cascade objective; 
if a model $(\bw,\alpha)$ has a large margin with respect to the threshold $\thr$ on a finite sample of training data, 
then with high probability, the performance of the model on unseen test data will not be too
much worse as $N$ gets large. This theorem  is the first theoretical guarantee on the 
generalization of {\em accuracy} 
and {\em efficiency} of a structured filtering model.  We plan to show a similar bound for the decomposable
cascades.
These bounds provide an a-posteriori type of guarantees: if cascade is effective on training data, it will also be
effective on new data.  But a more difficult question is what intuitive properties of the specific problem structure or data
distribution guarantee that a coarse-to-fine approach will succeed.  We plan to attack this problem
by assuming existence of large-margin separators with a kind of \textit{power decay}: most of 
the margin comes from the coarse features/cliques and the contributions of successive layers 
are on expectation exponentially smaller.  Such an assumption should allow us to lower-bound
the amount of output space that can be filtered by coarse-level models.

%\subsection*{Evaluation}
\mypar{Evaluation: Pose estimation and action parsing in videos} Our preliminary results on pose estimation are promising
and will pave the way of parsing actions: understanding the context and consequences of 
interactions between actors in video; e.g., to be able to follow a pointing arm or to observe the transfer of 
an important object from one person to another. While many current approaches use shallow representations of objects and actions via bags of generic descriptors based on local gradient and optical flow histograms (e.g.~\cite{LMSR08}), we are pursuing a model-based approach, where the aim is not to just detect, but to parse at least 10 action types. We aim use the cascade architecture to precisely locate the actionÕs key elements: (1) its temporal beginning and end; (2) the spatial trajectory of actor(s) and (3) the spatial trajectory of object(s) involved.  This effort will leverage support from the Google and RCTA grants.

\mypar{Evaluation: Syntactic parsing and machine translation} 
Our preliminary results on sequence labeling tasks like handwriting recognition  and part-of-speech tagging~\cite{cascades}
are very encouraging.  Parsing and syntax-based translation are natural candidates for coarse-to-fine reasoning.  
Similar cascade learning formulation can be derived using max-marginals of the CKY algorithm. The work 
of~\cite{petrov:PhD} showed the benefits of coarse-to-fine reasoning using grammar abstractions in generative models with
latent variables.  Our belief is that our cascade framework will allow us to scale up discriminative learning
for parsing and translation by carefully exploiting decomposition ensembles of simpler grammars in addition to natural 
hierarchies of non-terminal abstraction.

\out{

\section{from eccv}
Pictorial structure models~\cite{fischler1973ps} are a popular method for human body pose estimation~\cite{felz05,fergus2005sparse,devacrf,ferrari08,andriluka09}.
The model is a Conditional Random Field over pose variables that characterizes local appearance properties of parts and geometric part-part interactions.   The search over the joint pose space is linear time in the number of parts when the part-part dependencies form a tree.  However,  the individual part state-spaces are too large (typically hundreds of thousands of states) to allow complex appearance models be evaluated densely.   Most appearance models are therefore simple linear filters on edges, color and location~\cite{felz05,devacrf,ferrari08,andriluka09}. Similarly, because of quadratic state-space complexity, part-part relationships are typically restricted to be image-independent deformation costs that allow the convolution or distance transform tricks to speed up inference~\cite{felz05}. A common problem in such models is poor localization of parts that have weak appearance cues or are easily confused with background clutter (accuracy for lower arms in human figures is almost half of that for torso or head~\cite{andriluka09}).   Localizing these elusive parts requires richer models of individual part shape and joint part-part appearance, including contour continuation and segmentation cues, which are prohibitive to compute densely.

In order to enable richer appearance models, we propose to learn a cascade of pictorial structures () of increasing pose resolution which progressively filter the pose state space.  Conceptually, the idea is similar to the work on cascades for face detection~\cite{geman2001,viola02}, but the key difference is the use of structured models. Each level of the cascade at a given spatial/angular resolution refines the set of candidates from the previous level and then runs inference to determine which poses to filter out.  For each part, the model selects poses with the largest max-marginal scores, subject to a computational budget.  Unlike conventional pruning heuristics, where the possible part locations are identified using the output of a detector, models in our cascade use inference in simpler structured models to identify what to prune, taking into account global pose in filtering decisions
}


olution refines the set of candidates from the previous level and then runs inference to determine which poses to filter out.  For each part, the model selects poses with the largest max-marginal scores, subject to a computational budget.  Unlike conventional pruning heuristics, where the possible

==> text/grant/related.tex <==
% !TEX root =  career.tex
\section{Related Work}

\mypar{Graphical Models and Structured Prediction} Effective modeling
of uncertainty and complexity of interactions is a fundamental problem
in understanding and designing complex systems. By combining ideas
from statistics and graph theory, probabilistic graphical models
provide a general representation and an algorithmic framework for
reasoning about statistical
dependencies~\cite{koller2009probabilistic}. Structured prediction
often uses graphical models to solve problems of classification or
regression in which the output variables are mutually dependent or
constrained~\cite{psd-book}. These dependencies and constraints
reflect sequential, spatial or combinatorial structure in the problem
domain, and capturing such interactions is often as important as
capturing input-output dependencies. Many such problems, including
natural language parsing, machine translation, object segmentation,
and numerous other tasks in computational linguistics, speech, vision,
biology, are not new. However, recent advances have brought about a
unified view, efficient methodology and more importantly, significant
accuracy improvements for both classical and novel problems. The PI's
work~\cite{taskar03max,taskar04amns,taskar05extra,taskar05l2x} as well
as work by others (e.g.
\cite{lafferty01crf,joachimsmm,crfvision1,crfvision3,condid}) address
the fundamental computational and statistical challenges arising from
the high dimensionality of the inputs and the exponential explosion of
the number of possible joint outcomes.

\mypar{Computation/approximation trade-off}
Several recent works have considered the trade-off between error and
computation at \textit{estimation} time in large-scale classification
using stochastic/online methods,
notably~\cite{shalevshwartz2008soi,bottou-bousquet-2008}.  The issue
of controlling computation at \textit{prediction} time as well as
estimation time comes up in kernelized classifiers, where prediction
speed depends on the number of ``support vectors''.  Several
algorithms~\cite{Crammer03onlineclassification,dekel2008forgetron,cavallanti2007tbh},
including the Forgetron and Randomized Budget Perceptron are designed
to maintain a limited active set of support vectors in an online
fashion while minimizing error.

\mypar{Coarse-to-fine reasoning}
For unstructured, binary classification, cascades of classifiers have been quite successful for reducing computation.  Fleuret and Geman~\cite{geman2001} propose a coarse-to-fine sequence of binary tests to detect the presence and pose of objects in an image.  The learned sequence of tests is trained to minimize expected computational cost.  The extremely popular Viola-Jones classifier~\cite{viola02} implements a cascade of boosting ensembles, with earlier stages using fewer features to quickly reject large portions of the state space.
Our cascade framework is inspired by these binary classification cascades.  In natural language parsing, several works \cite{charniak2000maximum,carreras2008tag,petrov:PhD} use a coarse-to-fine idea closely related to ours and~\cite{geman2001}: the marginals of a simple context free grammar or dependency model are used to prune the parse chart for a more complex grammar.

Recently, Felzenszwalb et al.~\cite{pff-cascade} proposed a cascade for a structured parts-based object detection model.  Their cascade works by early stopping while evaluating individual parts, if the combined part scores are less than fixed thresholds.  While the form of this cascade can be posed in our more general framework (a cascade of models with an increasing number of parts), we differ from~\cite{pff-cascade} in that our pruning is based on thresholds that adapt based on inference in each test example, and we explicitly learn parameters in order to prune safely and efficiently. In~\cite{geman2001,viola02,pff-cascade}, the focus is on preserving established levels of accuracy while increasing speed.  
%The focus in this paper is instead developing more complex models---previously infeasible due to the original intractable complexity---to improve state-of-the-art performance.
\out{
A different approach to reduce the intractable number of state hypotheses is to instead propose a small set of likely hypotheses based on bottom-up perceptual grouping principles~\cite{mori04,Srinivasan07}.  Mori et al.~\cite{mori04} use bottom-up saliency cues, for example strength of supporting contours, to generate limb hypotheses.  They then prune via hand-set rules based on part-pair geometry and color consistency. The shape, color and contour based features we use in our last cascade stage are inspired by such bottom-up processes.  
%However, our cascade is solely a sequence of discriminatively-trained top-down models.
}

\out{
\section{IRL}

As we've discussed, the true IRL/AL analog of your cascading algorithm would be an algorithm that learned the policy of an observed expert in a coarse discretization of the environment, and then progressively moved on to finer and finer discretizations, "throwing out" unlikely states along the way in order to control computational complexity. In a good case, it seems that the running time of this algorithm will scale with the number of states that the expert visits, not the number of states in the whole environment. This is potentially a tremendous savings.

I agree that Nathan Ratliff and Drew Bagnell are the most likely people to have done something like this already. However, I don't think they've done this, nor has anyone else, as best as I can tell. Moreover, I think ideas from hierarchical RL can be readily adapted here, and perhaps it would make sense in the grant proposal to describe this idea using terminology from that field. For example, in hierarchical RL, a policy that is executed in only part of the state space is sometimes called an ``option'', and a master policy is learned by stitching together options. I could help you more with this, if you like. By the way, the major citations in hierarchical RL are \cite{ParrRu98, SuttonPr99, Dietterich00}.

I have only found two papers that can fairly be described as hierarchical IRL/AL, but they are not really related to the idea described above. One is by \cite{KolterAb07} (which you know about), and the other is by \cite{RosmanRa10}, which is quite recent. Both papers learn to mimic the expert's policy from partial demonstrations in portions of the whole state space (Rosman calls these ``basis'' environments).

I'm not sure that the section of Ratliff's thesis that you pointed me is relevant to us. Let me describe that work, and perhaps you can decide. The algorithm is also described in \cite{RatliffBr07}, and is an improvement on the work in \cite{RatliffBa06}. The algorithm takes as input several paths in a map, and the goal is to compute a reward function for which these paths are near-optimal. Instead of having a fixed number of features, they add them dynamically. Moreover, the reward function can be a non-linear function of the features. They start with a small number of features, and learn a linear reward function that is an optimum of the usual structured prediction loss. Then they do "inference" and compute the best path for this learned reward function. Then they construct a training set which contains a positive example for each feature vector of the states visited by this best path, and a negative example for each feature vector of the states visited by the expert's paths. They use a regression algorithm to learn a (possibly nonlinear) function of the features that fits this training set, and add this function as a new feature. Then the process repeats.

I checked both Pieter Abbeel's and Nathan Ratliff's theses, and neither contained any further references that seem related to hierarchical IRL/AL in the sense that we have discussed.

Let me also say a little bit about non-IRL/AL work. In vision, instead of learning a coarse-to-fine sequence of models, as you do with structured prediction cascades, there is much work about learning a hierarchy of coarse-to-fine features. Of course, you are already familiar with most of this work. For example, Viola-Jones work can be described this way, as can Serre and Poggio's max pooling algorithm. However, I found a recent paper by Bagnell \emph{et al} on Stacked Hierarchical Classification \cite{MunozBa10}, that I thought might be new to you. They divide images into regions, and construct an agglomerative hierarchy of these regions (so each level of the hierarchy is a partition of the image, and the root of the hierarchy is the whole image). For each node in the hierarchy, they train a classifier to predict the label proportions of the corresponding region. The interesting thing is that these predictions are then passed on to the nodes in the child level, which use them when learning their classifiers.

Finally: Tamir's talk on Monday was about structured prediction when the graph has cycles. It occurred to me that the cascades idea might be useful here, where the low-order models of the cascade are acyclic subgraphs of the full graph. In fact, isn't this one existing approach to dealing with cycles in graphical models (the phrase "tree decomposition" rings a bell)? Anyway, just a thought.

}
e predictions are then passed on to the nodes in the child level, which use them when learning their classifiers.

Finally: Tamir's talk on Monday was about structured prediction when the graph has cycles. It occurred to me that the cascades idea might be useful here, where the low-order models of the cascade are acyclic subgraphs of the full graph. In fact, isn't this one existing approach to dealing with cycles in gra

==> text/nips2010/conclusion.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.98\textwidth]{figs/results_qualitative.png}
\end{center}
\caption{\small \label{fig:results-qualitative} Qualitative test results.  Points shown are the position of left/right shoulders and torsos at the last level of the ensemble SC (blue square, green dot, white circle resp.).  Also shown (green line segments) are the best-fitting hypotheses to groundtruth joints, selected from within the top 4 max-marginal values. Shown as dotted gray lines is the best guess pose returned by the \cite{ferrari08}.}
\end{figure}

\section{Discussion}

{\bf Related Work.} Tracking with articulated body parts is
challenging for two main reasons.  First, body parts are hard to
detect in unconstrained environments due to the enormous variability
in appearance (from lighting, clothing and articulation) and
occlusion.  Second, the huge number of degrees of freedom makes exact
modeling of the problem computationally prohibitive.  In light of
these two issues, many works focus on fixed-camera environments
(e.g.,~\cite{andriluka2008people,pellegrini2009you,kratz-tracking}),
some even assuming sillhouettes can be obtained (e.g.,~\cite{bwu}), or
3d information from multiple sensors (\cite{munoz2007people}).  In
choices of modeling, past works reduce the large state space degrees
of freedom by only modeling location and scale, or resorting to
sampling methods (\cite{sigal2004tracking,kwon2009}, or embedding into
low-dimensional latent spaces \cite{andriluka2008people}. In contrast,
in this work we learn to efficiently navigate an unconstrained state
space in the challenging setting of a single, non-fixed camera.

We adopt the same basic modeling structure as
\cite{sapp2010,ferrari08,andriluka09} in our work, but also model
dependencies through time. We also take a discriminative approach to
training rather than generative. Ferrari et al.~\cite{ferrari08} use
loopy belief propagation to incorporate temporal consistency of parts,
but to our knowledge we are the first to quantitatively evaluate on
movie/TV show sequences.

In the method of dual decomposition \cite{komodakis2007dualdecomp},
efficient optimization of a LP relaxation of MAP inference in an
intractable model is achieved by coupling the inference of a
collection of tractable sub-models. This coupling is achieved by
repeatedly performing inference and updating a set of dual parameters
until convegence. In contrast, we perform inference independently in
each sub-model only {\em once}, and reason about individual variables
using the sums of max-marginals.

\paragraph{Future Research.}
Several key questions remain as future directions of
research. Although we presented generalization bounds for the error of
the cascade, such bounds are purely ``post-hoc.'' We are currently
investigating {\em a priori} properties of or assumptions about the data and
cascade that will provably lead to efficient cascaded learning and
inference. In the future, our approach on the VideoPose dataset could
be easily extended to model more limbs, additionally complex features
in time and geometry (e.g. \cite{sapp10cascades}), and additional
states such as occlusions. Successfully solving this problem is
necessary in order to understand the context and consequences of
interactions between actors in video; e.g., to be able to follow a
pointing arm or to observe the transfer of an important object from
one person to another.

\out{past research has made simplifying assumptions in
both datasets and modeling.  In terms of datasets,}
%There is a vast amount of literature on tracking people, with a
%variety of representations: jointly modeling multiple people's
%locations (e.g., nishinio cvpr2010, ), modeling shape (e.g., xiaofeng
%ren), tracking parts in 2d (e.g., andriluka) and in 3d ().  In all
%such methods, the environment is constrained to make the problem
%easier.  static background, multiple cameras


%{\bf Dynamic Bayes Nets.}

\out{{\bf Pictorial Structures.} There has been recent interest in human
pose estimation in single frames ``in the
wild''~\cite{sapp2010,ferrari08,andriluka09}.  Pictorial structures
models refer to graphical models in which each node represents the
limb of person.  They are popular choice because they offer fast
inference methods due to data-independent pairwise cliques.  We adopt
the same basic structure in our work, but also model dependencies
through time. We also take a discriminative approach to training
rather than generative. Ferrari et al.~\cite{ferrari08} use loopy
belief propagation to incorporate temporal consistency of parts, but
to our knowledge we are the first to quantitatively evaluate on
movie/TV show sequences.}


\out{We presented Structured Ensemble Cascades, a novel, principled
framework for handling state complexity while learning intractable
models. We provided a simple algorithm to minimize a novel convex loss
function, as well as generalization bounds on the error of any learned
parameters. Experimentally, we found that our approach outperformed
approximate inference with loopy belief propagation on a synthetic
task and outperformed a state-of-the-art pose estimation algorithm on
a difficult realistic tracking task.}

\out{In this work, we focus on the problem of human pose articulation and
tracking in videos ``in the wild.''  Unlike much of previous research,
our end-goal is not to track humans in surveillance or street video,
determine 3D pose from multiple input streams, or to recognize classes
of actions, but instead to robustly track the movements of multiple
actors' limbs with high precision. Our input is single-camera, high
resolution video, where both the camera and actors may be moving
independently. Successfully solving this problem is necessary in order
to understand the context and consequences of interactions between
actors in video; e.g., to be able to follow a pointing arm or to
observe the transfer of an important object from one person to
another.}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 


==> text/nips2010/dbn.tex <==
\section{Structured Ensemble Cascades} %Learning to Filter Intractable Markov Models}
\label{sec:dbn}
\out{
\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{figs/cascade_example_overview2.pdf}
  \caption{\small An example of ensemble cascade on VideoPose
    dataset. The state space of torso (white arrows), left arm (green
    arrows), and right arm (purple arrows) are superimposed on several
    frames from a single clip. The states are refined and become
    increasingly localized and sparse as the depth of the cascade
    increases.}
  \label{fig:pose_overview}
\end{figure}}

In this work, we tackle the problem of learning a structured cascade
for problems in which inference is {\em intractable}, but in which the
large node state-space has a natural hierarchy that can be
exploited. For example, such hierarchies arise in pose estimation by
discretizing the articulation of joints at multiple resolutions, or in
image segmentation due to the semantic relationship between class
labels (e.g., ``grass'' and ``tree'' can be grouped as ``plants,''
``horse'' and ``cow'' can be grouped as ``animal.'')

Although the methods discussed in this section can be applied to more
general intractable settings, and our prior work considered more
general cascades that operate on graph cliques, we will assume for
simplicitly that the structured cascades operate in a ``node-centric''
coarse-to-fine manner as follows. For each variable $y_j$ in the
model, each level of the cascade filters a current set of possible
states $\cY_j$, and any surviving states are passed forward to the
next level of the cascade by substituting each state with its set of
descendents in the hierarchy. Thus, in the pose estimation problem,
surviving states are subdivided into multiple finer-resolution states;
in the image segmentation problem, broader object classes are split
into their constituent classes for the next level.

We propose a novel method for learning structured cascades when
inference is intractable due to loops in the graphical structure. The
key idea of our approach is to decompose the loopy model into a
collection of equivalent tractable sub-models for which inference is
tractable. What distinguishes our approach from other decomposition
based methods (e.g., \cite{komodakis2007dualdecomp,bertsekas99}) is
that, because the cascade's objective is filtering and not decoding,
our approach does not require enforcing the constraint that the
sub-models agree on which output has maximum score. We call our
approach {\em structured ensemble cascades}.

\out{
 When working in large, complex state-spaces, Markov
models become intractable due to interactions between multiple state
variables and the fine-level resolution at which states need to be
estimated. For example, in the PATV problem, we track many variables
representing the location and orientation of mutiple limbs
simultaneously in an articulated model. For example, in this paper we
track simultaneously the location of the upper body and the location
and rotation of the upper halves of left and right limbs (Figure
\ref{fig:dbn}, left). Graphically, we have a tree model to represent
the dependency between limbs and torso, but to model temporal
persistence, we require edges between each state variable to the
previous and next video frames. Even when states are discretized at
the relatively coarse resolution of $40 \times 40$ positions and only
$24$ limb rotations, the interactions between state variables in
transitions produces a clique with $\approx 10^{12}$ possible
assignments, which makes inference intractable.

We propose decomposing the temporal dependencies in the fully
connected model (Figure \ref{fig:dbn}, left) and approximating the
intractable model with an ensemble of tractable models. Each model in
the ensemble models the temporal persistence of only a single state
variable, so inference remains tractable. We refer to this collection
of decomposed models as the {\em decomposition ensemble.} In this
section, we extend the SC framework to operate with such
ensembles. Our method jointly learns parameters for every model in the
ensemble, yet requires only a linear increases in
resources. Furthermore, we provide a generalization bound on the
filtering loss of the ensemble as theoretical justification of our
approach.}

\subsection{Decomposition without agreement constraints}

Given a loopy (intractable) graphical model, it is always possible to
express the score of a given output $\score{y}$ as the sum of $P$
scores $\pscore{y}$ under sub-models that collectively cover every
edge in the loopy model: $\score{y} = \sum_p \pscore{y}.$ (See Figures
2 \& 3 for illustrations specific to the experiments presented in this
paper.) For example, in the method of dual decomposition
\cite{komodakis2007dualdecomp}, it is possible to solve a relaxed MAP
problem in the (intractable) full model by running inference in the
(tractable) sub-models under the constraint that {\em all sub-models
  agree on the argmax solution.}  Enforcing this constraint requires
iteratively re-weighting unary potentials of the sub-models and
repeatedly re-running inference until each sub-model convergences to
the same argmax solution.

However, for the purposes of a structured cascade, we are only
interested in computing the max marginals $\mmarg{y_j}$. In other
words, we are only interested in knowing whether or not a
configuration $y$ consistent with $y_j$ that scores highly in each
sub-model $\pscore{y}$ {\em exists.} We show in the remainder of this
section that the requirement that a {\em single} $y$ consistent with
$y_j$ optimizes the score of each submodel (i.e, that all sub-models
{\em agree}) is not necessary for the purposes of filtering. Thus,
because we do not have to enforce agreement between sub-models, we can
learn a structured cascade for intractable models, but pay only a
linear (factor of $P$) increase in inference time over the tractable
sub-models.

Formally, we define a single level of the ensemble cascade as a set of
$P$ models such that $\score{y} = \sum_p \pscore{y}$.  We let
$\pscore{\cdot}$, $\pmmarg{\cdot}$, $\pscoremax$ and $\pthr{x}$ be the
score, max marginal, max score, and threshold of the $p$'th model,
respectively. We define the {\em argmax marginal} or {\em witness}
$\pwit{y_j}$ to be the maximizing complete assignment of the
corresponding max marginal $\pmmarg{y_j}$. Then, if $y = \pwit{y_j}$
is the same for each of the $p$'th submodels, we have that
\begin{equation}
  \label{eq:mmarg-equality}
  \mmarg{y_j} = \sum_p \pmmarg{y_j}  
\end{equation}
Note that if we do not require the sub-models to agree, then
$\mmarg{y_j}$ is stricly less than $\sum_p \pmmarg{y_j}$. Nonetheless,
as we show next, the approximation $\mmarg{y_j} \approx \sum_p
\pmmarg{y_j}$ is still useful and sufficient for filtering in a
structured cascade.

\out{
We then define the joint marginal the ensembles consists
of repeating tree models over $P$ variables, where the $p$'th model
incorporates persistence of the $p$'th variable through time. We learn
a filter over the ensemble jointly by summing the max marginals of
each model, and we compute a filtering threshold on the summed max
marginals. Then 
The advantage of summing the marginals in this manner is that a
weakness in one member of the ensemble on a particular example can be
compensated for by the strengths of the other models. Although one or
more of the individual scores $\pscore{y^i}$ may be under threshold
$\pthri$, the ensemble can still avoid a mistake if another member
scores $y^i$ high enough to compensate. On the PATV problem, this may
occur if the model part with the strongest visual cues for continuity
through time varies from example to example; e.g., in scenes where the
actor faces the camera, modeling a smooth face trajectory is useful,
while if the face is obscured or the actor is facing away from camera,
modeling a smooth arm trajectory may be more accurate. In fact, we
find experimentally (section \ref{sec:results}) that persistence of
certain variables is much more helpful than others. Note that an
alternative to \eqref{eq:joint_sc} using the original SC framework
would be to simply learn a cascade of $P$ models, but in that
approach, mistakes are cumulative, and there is no way for any model
to compensate for the weaknesses of the others.}

\subsection{Safe filtering and generalization error}

We first show that if a given label $y$ has a high score in the full
model, it must also have a large ensemble max marginal score, even if
the sub-models do not agree on the argmax. This results in a ``safe
filtering'' lemma similar to that given in \cite{weiss10}, as follows:
\begin{lem}[Joint Safe Filtering]
  \label{lem:joint_safe}
  If $\sum_p \pscore{y} > t$, then $\sum_p \pmmarg{y_j} > t$ for all $y_j \subseteq y$.
\end{lem}
\begin{proof}
  In English, this lemma states that if the global score is above a
  given threshold, then the sum of sub-model max-marginals is also
  above threshold (with no agreement constraint). The proof is
  straightforward.  For any $y_j$ consistent with $y$, we have
  $\pmmarg{y_j} \ge \pscore{y}$. Therefore $\sum_p \pmmarg{y_j} \ge
  \sum_p \pscore{y} > t$.
\end{proof}
Therefore, we see that an agreement constraint is not necessary in
order to filter safely: if we ensure that the combined score $\sum_p
\pscore{y}$ of the true label $y$ is above threshold, then we can
filter without making a mistake if we compute max marginals by running
inference separately for each sub-model. However, there is still
potentially a price to pay for disagreement. If the sub-models do not
agree, {\em and} the truth is not above threshold, then the threshold
may filter {\em all} of the states for a given variable $y_j$ and
therefore ``break'' the cascade. This results from the fact that
without agreement, there is no single argmax output $y^\star$ that is
always above threshold for any $\alpha$; therefore, it is not
guaranteed that there exists an output $y$ to satisfy the Joint Safe
Filtering Lemma. However, we note that in our experiments, we never
experienced such breakdown of the cascades due to overly aggressive
filtering.

In order to learn parameters that are useful for filtering, Lemma
\ref{lem:joint_safe} suggests a natural {\em ensemble filtering loss},
which we define for any fixed $\alpha$ as follows,
\begin{equation}
  \label{eq:joint_loss}
  \cL_{joint}(\theta, \ang{x,y}) =  \ind{\sum_p\pscore{y} \le \sum_p \pthr{x}},
\end{equation}
where $\theta = \{\theta_1, \dots, \theta_P\}$ is the set of all
parameters of the ensemble. (Note that this loss
function is somewhat conservative because it measures whether or not a
{\em sufficient} but not necessary condition for a filtering error has
occured.) 

To conclude this section, we provide a generalization bound on the
ensemble filtering loss, equivalent to the bounds in \cite{weiss10}
for the single-model cascades. To do so, we first eliminate the
dependence on $x$ and $\theta$ by rewriting $\cL_{joint}$ in terms of
the {\em scores} of every possible state assignment, $\theta \cdot
\bft(x,y_j)$, according to each sub-model. Let the vector $\ssp \in
\reals^{mP}$ denote these scores, where $m$ is the number of possible
state assignments in the sub-models.
\begin{thm}
  \label{thm:gencascade}
  For any fixed $\alpha \in [0,1)$, define the dominating cost
  function $\phi(y, \ssp) = r_\gamma(1/P \sum_p \pscore{y} -
  \pthr{x})$, where $r_\gamma(\cdot)$ is the ramp function with slope
  $\gamma$. Let $||\theta_p||_2 \le F$ for all $p$, and
  $||\bft(x,y_j)||_2 \le 1$ for all $x$ and $y_j$. Then there exists a
  constant $C$ such that for any integer $n$ and any $0 < \delta < 1$
  with probability $1-\delta$ over samples of size $n$, every $\theta
  = \{\theta_1, \dots, \theta_P\}$ satisfies:
  \begin{equation}
    \label{eq:gencascade}
      \bbE \left[\cL_{joint}(Y, \ssp)\right] \le
      \hat{\bbE}\left[\phi(Y,\ssp)\right] +
      \frac{Cm\sqrt{\ell}FP}{\gamma\sqrt{n}}
      + \sqrt{\frac{8 \ln (2/\delta)}{n}},
    \end{equation}
  where $\hat{\bbE}$ is the empirical expectation with respect to
  training data.
\end{thm}
The proof is given in the supplemental materials.

\subsection{Parameter estimation with gradient descent}

% TODO: add 1/n in front of ALL slacks etc.

In this section we now discuss how to minimize the loss
\eqref{eq:joint_loss} given a dataset. We rephrase the SC optimization
problem \eqref{eq:std_sc} using the ensemble max-marginals to
form the ensemble cascade learning problem,
\begin{equation}
  \label{eq:joint_slack}
  \inf_{\theta_1, \dots, \theta_P, \xi \ge 0} \frac{\lambda}{2} \sum_p ||\theta_p||^2 + \frac{1}{n}\sum_i \xi^i
  \suchthat \sum_p \pscorei{y^i} \ge \sum_p \pthri + \ell^i - \xi^i,
\end{equation}
Seeing that the constraints can be ordered to show $\xi^i \le \sum_p
\pthri -\sum_p \pscorei{y^i} +\ell^i$, we can form an equivalent
unconstrained minimization problem and \out{\begin{equation}
  \label{eq:joint_hinge}
  \inf_{\theta_1, \dots, \theta_P} \frac{\lambda}{2}\sum_p ||\theta_p||^2 + \frac{1}{n}\sum_{i} \hinge{\sum_p \pthri - \pscorei{y^i} + \ell^i},
\end{equation}
where $\hinge{x} = \max\{x, 0\}$ is the hinge function. } take the
subgradient of \eqref{eq:joint_slack} with respect to each parameter
$\theta_p$. This yields the following update rule for the $p$'th model:
\begin{equation}
  \label{eq:joint_update}
  \theta_p \leftarrow (1-\lambda)\theta_p +
  \begin{cases}
    0 & \textrm{ if } \sum_p \pscorei{y^i} \ge \sum_p \pthri + \ell^i, \\
    \nabla\pscorei{y^i} - \nabla\pthri & \textrm{ otherwise.}
  \end{cases}
\end{equation}
This update is identical to the original SC update with the exception
that we update each model individually only when the ensemble has made
a mistake {\em jointly}. Thus, learning to filter with the ensemble
requires only $P$ times as many resources as learning to filter with
any of the models individually.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 


==> text/nips2010/experiments.tex <==
\out{\begin{table}
  \label{tab:ensemble}
  \centering
  \small
  \begin{tabular}{|c|cc|cc|}
    \hline
    & \multicolumn{2}{|c|}{\em Pixel Err. at 50\% Efficiency} & \multicolumn{2}{|c|}{\em Pixel Err. at 90\% Efficiency}  \\
    \hline
    Model & Torso & Torso+Arms & Torso & Torso+Arms \\    
    \hline
    Torso   &34.5 $\pm$ 35.3 &26.8 $\pm$ 33.8 & 64.6 $\pm$ 70.2 &57.8 $\pm$ 62.5 \\
    L. Arm &50.1 $\pm$ 51.4 &36.5 $\pm$ 45.9 & 85.0 $\pm$ 87.2 &74.7 $\pm$ 75.8 \\
    R. Arm &28.3 $\pm$ 20.9 & {\bf 18.4 $\pm$ 21.3} & 52.0 $\pm$ 64.4 &45.1 $\pm$ 57.1 \\
    Ensemble & {\bf 20.4 $\pm$ 41.3} & 21.0 $\pm$ 33.3 & {\bf 35.1 $\pm$ 70.6} & {\bf 40.8 $\pm$ 60.2} \\
    \hline
  \end{tabular}
  \caption{\small Decomposition ensemble results on Buffy dataset. Shown is the minimum pixel distance from 
    the true joint location to an unfiltered state in the grid for each joint.
    ``Model'' indicates which temporal dependency was included in the model.}
\end{table}
}
\section{Experiments}
\label{sec:results}

We evaluated structured ensemble cascades in two experiments. First,
we analyzed the ``best-case'' filtering performance of the summed
max-marginal approximation to the true marginals on a synthetic image
segmentation task, assuming the true scoring function $\score{y}$ is
available for inference. Second, we evaluated the real-world accuracy
of our approach on a difficult, real-world human pose dataset
(VideoPose). In both experiments, the max-marginal ensemble outperforms
state-of-the-art baselines.

%     Model & L. Arm & R. Arm & Torso & All & L. Arm & R. Arm & Torso & All \\    
%     \hline
%     Torso  & 17.1 $\pm$ 31.7 &22.2 $\pm$ 36.5 &34.5 $\pm$ 35.3 &26.8 $\pm$ 33.8 & 36.8 $\pm$ 58.3 &49.7 $\pm$ 65.5 &64.6 $\pm$ 70.2 &57.8 $\pm$ 62.5 \\
%     L. Arm & 21.9 $\pm$ 41.5 &27.1 $\pm$ 41.2 &50.1 $\pm$ 51.4 &36.5 $\pm$ 45.9 & 59.0 $\pm$ 85.2 &55.5 $\pm$ 70.9 &85.0 $\pm$ 87.2 &74.7 $\pm$ 75.8 \\
%     R. Arm & 8.4 $\pm$ 12.3 &13.1 $\pm$ 21.8 &28.3 $\pm$ 20.9 &18.4 $\pm$ 21.3 & 29.0 $\pm$ 55.3 &33.8 $\pm$ 58.6 &52.0 $\pm$ 64.4 &45.1 $\pm$ 57.1 \\
%     Ensemble &17.6 $\pm$ 34.1 &16.8 $\pm$ 31.2 &20.4 $\pm$ 41.3 &21.0 $\pm$ 33.3 & 30.3 $\pm$ 69.1 &32.0 $\pm$ 61.2 &35.1 $\pm$ 70.6 &40.8 $\pm$ 60.2 \\

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 


==> text/nips2010/intro.tex <==
% !TEX root =  ../paper.tex

\section{Introduction}

% NOTES:
% Emphasize problem
% Emphasize DBN


We address the problem of prediction in graphical models
that are computationally challenging because of both high-treewidth
and large state-spaces.  A primary example where intractable, large state-space models typically arise is in dynamic state estimation problems, including tracking articulated objects or multiple targets~\cite{sigal2004tracking,bwu}.  The complexity stems from interactions of multiple degrees-of-freedom
(state variables) and fine-level resolution at which states need to be estimated.  Another typical example arises in pixel-labeling problems where the model topology is typically a 2D grid and the number of classes is large~\cite{MSRC-21}.  In this work, we propose a novel, principled framework called Structured Ensemble Cascades for handling state complexity while learning complex models, extending our previous work on structured cascades for low-treewidth models~\cite{weiss10}.

\begin{figure}[t!]
\centering
\includegraphics[width=0.98\textwidth]{figs/big_schematic+example.pdf}
\caption{\small \label{fig:overview} \textbf{(a)} Schematic overview of structured
  ensemble cascades. The $m$'th level of the cascade takes as input a
  sparse set of states $\mcal{Y}^m$ for each variable $y_j$. The full
  model is decomposed into constituent sub-models (above, the three
  tree models used in the pose tracking experiment) and sparse
  inference is run. Next, the max marginals of the sub-models are
  summed to produce a single max marginal for each variable
  assignment: $\mmarg{y_j} = \sum_p \pmmarg{y_j}$. Note that each
  level and each constituent model will have different parameters as a result of the learning
  process. Finally, the state spaces are thresholded based on the
  max-marginal scores and low-scoring states are filtered. Each state
  is then refined according to a state hierarchy (e.g., spatial
  resolution, or semantic categories) and passed to the next level of
  the cascade. This process can be repeated as many times as desired. In \textbf{(b)}, we illustrate two consecutive levels of the ensemble cascade on real data, showing the filtered hypotheses left for a single video example.}
\end{figure}


%we use a novel generalization of the Structured
%Prediction Cascades (SC) framework, first proposed by %\cite{weiss10},
%to intractable models.
The basic idea of structured cascades is to learn a sequence of coarse-to-fine
models that are optimized to safely filter and refine the structured output state space,
speeding up both learning and inference. While we previously assumed
(sparse) exact inference is possible throughout the
cascade~\cite{weiss10}, in this work, we apply and extend the
structured cascade framework to {\em intractable} high-treewidth
models. To avoid intractable inference, we decompose the desired model
into an ensemble of tractable sub-models for each level of the
cascade. For example, in the problem of tracking articulated human
pose, each sub-model includes temporal dependency for a single body
joint only. To maintain efficiency, inference in the sub-models of
the ensemble is uncoupled (unlike in dual
decomposition~\cite{komodakis2007dualdecomp}), but the decision to
filter states depends on the \emph{sum} of the max-marginals of the
constituent models (see Figure~\ref{fig:overview}).  We derive a
convex loss function for joint estimation of sub-models in each
ensemble, which provably balances accuracy and efficiency, and we
propose a simple stochastic subgradient algorithm for training.

The novel contributions of this work are as follows. First, we provide
a principled and practical generalization of structured cascades to intractable models. Second, we present generalization bounds on the performance of the ensemble.
Third, we introduce a challenging VideoPose dataset, culled from TV videos,
for evaluating pose estimation and tracking.
%for the purposes of establishing a new avenue of research.
\out{Third, we propose and implement a
``coarse-to-fine'' localization cascade, which we use as an
initial pre-processing step to determine a set of potential locations
for actors in an image in order to practically solve the VideoPose
problem. To learn this localization cascade, we introduce two further
generalizations to the SC framework to allow for training of filters
with multiple outputs per image and to handle features at differing
resolutions than the coarse-level state resolutions.
}
Finally, we present an evaluation of our approach on synthetic data and
the VideoPose dataset. We find that our joint training of an ensemble
method outperforms several competing baselines on this difficult tracking problem.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:




==> text/nips2010/localizer.tex <==
\begin{table}
  \centering
  \small 
  \begin{tabular}{|ccccc|ccc|}
    \hline
    \multicolumn{5}{|c|}{\em Filt. Err. at 75\% Efficiency ($10 \times 10$)}&   \multicolumn{3}{|c|}{\em Coarse-to-fine Cascade ($\alpha = 0.2$)}\\
    % & & & & & & &1 \\
    {\bf Method} & {\bf Buffy} & {\bf Lost} & {\bf Friends} & {\bf Mean} &  {\bf Grid Size} & {\bf Pixel Err.} & {\bf Sparsity (\%)} \\
    \hline 
    $\alpha=0$ &1.90 &0.52 &0.98 &1.13 $\pm$ 0.70&    10 $\times$ 10  & 0.00 $\pm$ 0.00    & 60.58 $\pm$ 2.64 \\
    $\alpha=0.2$ &1.32 &1.17 &0.63 &1.04 $\pm$ 0.37&    20 $\times$ 10  & 1.27 $\pm$ 0.73  & 29.43 $\pm$ 2.14 \\
    $\alpha=0.4$ &1.15 &1.69 &0.44 &1.10 $\pm$ 0.63&    20 $\times$ 20  & 5.89 $\pm$ 1.40  & 16.22 $\pm$ 1.41 \\ 
    $\alpha=0.6$ &2.18 &1.11 &0.58 &1.29 $\pm$ 0.82&    40 $\times$ 20  & 10.28 $\pm$ 0.69 & 8.49 $\pm$ 0.58 \\
    $\alpha=0.8$ &2.59 &0.35 &0.58 &1.17 $\pm$ 1.23&    40 $\times$ 40  & 12.88 $\pm$ 0.84 & 4.64 $\pm$ 0.44 \\ 
    Boosting &12.51 &5.52 &5.92 &7.98 $\pm$ 3.92& & & \\
    \hline
  \end{tabular}
  \caption{\small Coarse-to-fine upper body localizer cascade results. Left: a comparison of our filter learning approach to an AdaBoost based approach on a 
    $10 \times 10$ grid. Numbers represent the \% of regions containing the center of a true bounding box that are incorrectly filtered with fixed 75\% efficiency. 
    Right: performance of the coarse-to-fine cascade. Each row was trained with $\alpha=0.2$, and filtered using $\alpha=0$. Shown is the grid size, pixel error, 
    sparsity of the total grid.}
  \label{tab:c2f}
\end{table}

\section{Learning to Localize via Filtering}
\label{sec:localizer}

Despite the ensemble learning method described in Section
\ref{sec:dbn}, inference in even the simplest models is
computationally infeasible due to the large number of possible
configurations in each frame. Because we consider a $40 \times 40$
grid of $(x,y)$ locations, there are $40^4 \approx 10^6$ possible
transitions from one frame to another for the torso, and more for
transitions between limbs that also include rotation in the
state. Therefore, we first apply a ``coarse to fine'' structured
prediction cascade on each frame individually, using exact inference
to produce a sparse set of torso and limb states that we will be used
for learning the ensemble. We start the cascade by modeling the upper
body alone at a coarse $10 \times 10$ grid; we then gradually increase
the resolution; finally, we finish the cascade with a PS graph model
run at the final $40 \times 40$ resolution.

However, the original SC framework cannot be applied directly to our
``coarse to fine'' problem for two reasons. First, the training
examples may contain multiple valid outputs per image. Second,
learning an upper body detector poses a ``chicken and egg'' problem:
to perform inference at a coarse scale, we compute scores at the
finest resolution and maximize over scores in a coarse
region. However, to learn a scoring function for filtering with SC, we
must already have max marginals of the coarse regions. In the next
sections we show how these issues can be easily addressed with minimal
conceptual changes to the SC framework.

\subsection{Handling Multiple Outputs}
\label{sec:multiple_outputs}

For the localization problem, we can have multiple actors in a given
image. Formally, assume without loss of generality that there are $B$
outputs (actors) in each image, and let $y^{i1}, \dots, y^{iB}$ denote
these outputs. We can incorporate multiple outputs into the SC filter
learning problem simply by introducing one additional constraint per
output: rather than require a single output $y^i$ to pass the
threshold, we require that every output $y^{ib}$ is above the
filtering threshold. Introducing one slack variable for each of these
constraints, we obtain the following minimization problem:
\begin{equation}
  \label{eq:mo_slack}
  \inf_\theta \frac{\lambda}{2}||\theta||^2 + \sum_{i,b} \xi^{ib} \suchthat \scorei{y^{ib}} \ge \thri + \ell^i - \xi^{ib}. % \quad \forall i = 1, \dots, n, \forall b = 1, \dots, B
\end{equation}
Again, since $\xi^{ip} \le \thri - \scorei{y^{ib}} + \ell^i$, we can remove
the constraints and get an equivalent unconstrained minimization
problem over a sum of $B$ hinge loss functions:
\begin{equation}
  \label{eq:mo_hinge}
  \inf_\theta \frac{\lambda}{2}||\theta||^2 + \sum_{i=1}^n\sum_{b=1}^B \hinge{\thri - \scorei{y^{ib}} + \ell^i}.
\end{equation}
Applying the sub-gradient method yields an algorithm that perform a
separate update for every output $y^{ib}$ that is not above
threshold. Thus, the additional complexity of solving this new problem
is linear in the number outputs and does not affect the complexity of
inference in the structured setting. Note also that as in the original SC filter
learning problem, the algorithm does not learn to score any desired
output above all others, but simply tries to avoid filtering out any 
of the correct outputs. % increasing the scores of only those outputs that incorrectly fall below threshold.

% Note that for the purposes of learning to filter, the relative scores
% of the different outputs $\score{y^{ib}}$ are not important; by
% posing the problem in terms of learning a filtering threshold, we
% avoid any interaction between the multiple outputs. As in the original
% SC filter learning problem, the goal is not to score the desired
% output above all others, but instead to simply avoid filtering them
% out. 
% If we one slack variable
% per output for each of these constraints, we Therefore we modify the
% SC learning problem in \eqref{eq:std_sc} as follows:
% \begin{equation}
%   \label{eq:multiple_outputs}
%   \inf_\theta \frac{\lambda}{2}||\theta||^2 \suchthat \scorei{y^{ib}} \ge \thri + \ell^i, \quad \forall i = 1, \dots, n, \forall b = 1, \dots, B
% \end{equation}

%  To see this, we introduce slack variables:
% which is simply a sum of the violations of the conservative filtering
% constraints for each of the multiple outputs. In section
% \ref{sec:approach}, we use a sub-gradient method to solve
% \eqref{eq:mo_hinge}. 

\subsection{Coarse-to-Fine Filtering for Single Variables}
\label{sec:coarse2fine}

The idea of coarse-to-fine inference is to gradually reduce a
candidate set of object locations by eliminating unlikely locations at
increasingly fine scales. In this section we show how to use SC to
learn a sequence of image filters to minimize the number of pruning
mistakes. For an image $x$ with $r$ rows and $c$ columns, we consider
outputs $y \in \{1, \dots, r\} \times \{1, \dots, c\}$, i.e., a
position in that image (note that by $y$ we do not mean the $y$-axis
but a single location $y = \ang{c,r}$.) We allow for multiple such outputs
as handled according to the previous section. For each location the
feature function $\bft(x,y)$ computes features on a patch exactracted
from image $x$ and centered at the location $y$.

For a desired level of coarseness, let $S_1, \dots, S_R \subseteq \cY$
be rectangular sets of locations that collectively cover the output
space $\cY$. We then define the max marginal over a set $S_r$ to be the
maximum score of any output $y \in S_r$: 
\begin{equation}
  \mmarg{S_r} \triangleq \max_{y' \in \cY} \;\; \{ \score{y'}: y' \in S_r\}.
\end{equation}
% \begin{equation}
%   \mmarg{S_r} \triangleq \max_{y' \in \cY} \;\; \{ \score{y'}: y'_c \in S_r\}.
% \end{equation}
We can then redefine the SC filtering threshold $\thr$ in terms of
these set-wise max marginals:
\begin{equation}
  \label{eq:groupmaxthr}
  \thr = \alpha\scoremax + (1-\alpha)/R \sum_{r=1}^R \mmarg{S_r}.
\end{equation}
Given an image patch scoring function $\theta$, we can then proceed
with our cascade as follows. With a coarse $10 \times 10$ grid of
rectangular regions, we compute the threshold \ref{eq:groupmaxthr} and
eliminate any region of points whose max marginal falls below
threshold. We then subdivide each surviving region in half and repeat
the filtering procedure. However, by plugging in the definition
\eqref{eq:groupmaxthr} to the multiple outputs SC problem in
\eqref{eq:mo_hinge}, we can learn scoring function over image patches
that is useful for filtering at any desired level of coarseness. Note
that in our coarse-to-fine filter, the features $\nabla \thr$ needed
to compute the update step are the average of the $R$ image patches
that maximize score according to the current $\theta$ within each
rectangular region.

There are several novel distinctions of this coarse-to-fine method of
training when compared to typical object detection methods. Typically,
image patches are harvested from training data according to a
bootstrapping process and the algorithm is trained to make binary
decisions \cite{hog}. Patches corresponding to the true labels are labelled
positive while all others are labelled negative. During training,
false positives from early stages of training are repeatedly added to
the training set to increase the discriminative power of the
classifier. In contrast, our coarse-to-fine approach does not learn to
make binary decisions at the level of image patches. Each image is
treated as a single example, and the scoring function learns to score the true
patch higher than the average of a set of hard false-positive patches extracted
automatically from the image based on the current parameters.

% The resulting coarse-to-fine method of training the initial object
% detection filter is outlined in Figure
% \ref{fig:detector_process}. There are several key distinctions of our
% method when compared to typical object detection methods. (1) During
% training, we treat each image as a single example. (2) Extracting
% patches of the image to learn from is performed automatically based on
% the current scoring function; the patches centered on each set max
% marginal location $\wit{S_i}$ are averaged together with the argmax
% image patch to compute features for the threshold. (3) Instead of
% learning to detect objects by scoring the exact true object lcoations
% greater than non-object patches, we learn to filter object locations
% by finding a threshold that distinguishes the true location only at
% the level of a coarse set of regions in the image.

% In the coarse-to-fine , we are interested in progressively refining
% the output space The coarse-to-fine approach is summarized as follows:
% In the coarse-to-fine approach,

% The final goal of the localization and tracking task is to identify
% objects of interest at the level of individual pixels. Previous
% approaches typically treat each pixel as a separate example of a
% binary classification problem [CITE]. There, the goal is to learn to
% predict whether or not a given pixel is the center of an object based
% on features computed from surrounding pixels, where $y = 1$ represents
% the presence of an object and $y = -1$ the absence. For training,
% positive and negative image patches are harvested from a database of
% images using an iterative process of training and data-gathering.

% In this work, we propose a novel approach to object localization using
% the modified SC learning problem above. For an image $x$ with $r$ rows
% and $c$ columns, we consider outputs $y \in \{1, \dots, r\} \times
% \{1, \dots, c\}$, i.e., a position in that image. If there are $B$
% objects present in an image $x$, then we have $B$ outputs $y^1, \dots,
% y^B$ corresponding to the centers of each of the objects. We then
% define a feature generating function $\bft: \cX \times \cY \mapsto
% \reals^d$, which extracts a vector of features from the image $x$
% based on the location defined by $y$ (in our experiments, we use
% histogram of gradients (HOG) [CITE] extracted from surrounding
% pixels). Given a vector of parameters $\theta$, we then solve
% \eqref{eq:mo_hinge} to find a scoring function that scores the true
% locations $y^1, \dots, y^B$ greater than the corresponding threshold
% $\thr$ for that image. Note that unlike previous object detection
% methods, which can be tuned only post-hoc, the learning problem we
% propose is tunable with the parameter $\alpha$: as $\alpha$ increases
% from $0$ to $1$, the threshold becomes tighter and the number of
% unfiltered locations decreases, trading off increasing precision (and
% thus computational efficiency in the cascade) for potentially
% decreasing recall (and thus the final accuracy of the cascade).

% We make one additional significant modification to the problem in
% \eqref{eq:mo_hinge}. As in \cite{weiss10}, we approach the goal of
% tracking at the pixel-level by learning a sequence of models that
% incrementally filter and refine the output space; although the
% original pixels are needed to compute the features $\bft$, the first
% level of the cascade filters at a coarse scale for increased
% efficiency. We do so by rephrasing the SC framework to reason about
% regions of the image with a desired level of coarseness. In general,
% we consider $R$ arbitrary {\em sets} of partial assignmen
% The benefit of this approach is that $R$ can be chosen independently
% of the size of the output space $\cY$ or the number of cliques or
% clique assignments. Furthermore, the set filtering problem is a
% relaxation of the original filtering problem in the following sense:
% At each stage of the cascade, any clique assignment $y_c$ in a region
% $S$ with $\mmarg{S} > \thr$ survives the filtering step, regardless of
% the value of the max marginal $\mmarg{y_c}$. Learning with set max
% marginals proceeds is the same procedure as the original SC problem
% but with the new threshold function \eqref{eq:groupmaxthr}.

% The use of set max marginals is critical to training the first step of
% the tracking cascade. The first model has only one variable $y$, the
% location of the object center in the image, and is essentially a very
% large multi-class decision problem. Applying the standard SC learning
% rule would require the true locations of the objects to be unfiltered
% at the finest scale. By defining a rectangular grid of regions $S_1,
% \dots, S_R$ that cover the full image and using a threshold defined
% as, we relax the requirement that the true locations of the objects
% fall in an unfiltered grid cell. During learning, computation of the
% sub-gradient step requires only $O(R)$ instead of $O(m)$ time, a
% significant speedup. Thus, we compute and learn features at the finest
% scale possible while performing inference at a coarse scale.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 


==> text/nips2010/patv.tex <==

% EXPAND THIS SECTION:
% -- divide bar y-charts by 480
% -- 

% \out{
% \begin{table}
%   \label{tab:ensemble}
%   \centering
%   \small
%   \begin{tabular}{lccccccccc}
%     \hline \\[-0.5em]
%     & \multicolumn{3}{c}{\em Pixel Err. (Decoding)}  & 
%     \multicolumn{3}{c}{\em Pixel Err. (K=4)} & 
%     \multicolumn{3}{c}{\em Pixel Err. (K=10)} \\
%     {\em Method} & Torso & U.Arm & L.Arm & Torso & U.Arm & L.Arm & Torso & U.Arm & L.Arm \\[1em]
%     Ferrari et al. \cite{ferrari08} & 123.4 & 155.51 & 298.04 & 116.48 & 121.54 & 211.22 & N/A & N/A & N/A \\
%     SC: Single Frame & {\bf 51.17} & 67.39 & 96.56 & {\bf 37.34} & 39.09 & 69.41 & {\bf 32.57} & 31.46 & {\bf 60.955} \\
%     SC: Torso Only & 79.42 & 98.15 & 131 & 73.69 & 82.24 & 105.16 & 73.69 & 63.38 & 83.05 \\
%     SC: Ensemble & 53.1 & {\bf 41.48} & {\bf 89.67} & 40.97 & {\bf 32.69} & {\bf 67.45} & 35.11 & {\bf 26.52} & 62.96 \\[0.5em]
%     \hline
%   \end{tabular}
%   \caption{\small Results on VideoPose dataset. 
%     Shown is the pixel error from the true joint endpoint location to the closet unfiltered location for the Ferrari et al. \cite{ferrari}
%     baseline and two structured cascade methods. (The endpoint error reflects errors in both position and angle.) ``Torso only'' - Cascade with a single tree modeling persistence of torso through time.
%     ``Ensemble'' uses marginals summed from each model in the decomposition (Figure \ref{fig:dbn}). We show errors when the 
%     methods are used to produce a single decoding (Left) or used as a filter to produce 4 possible locations for each joint (Right).}
% \end{table}
% }

%Top $K$ Error ($K=4$). Minimum (oracle) error
%  when 4 hypotheses are generated.
\begin{figure}
  \centering
  \subfigure[\small Decoding Error.]{
    \includegraphics[width=0.3\textwidth]{figs/top1_tracking_bars.png}
  }
  \hspace{-0.1in}
  \subfigure[\small Top $K=4$ Error.]{
    \includegraphics[width=0.3\textwidth]{figs/top4_tracking_bars.png}    
  } 
  \hspace{-0.1in}  
  \begin{minipage}{0.3\linewidth}
    \vspace{-1.05in}
    \scalebox{0.7}{
      \begin{tabular}{cccc}
        \hline \\[-0.5em]
        & {\em State } & $PCP_{0.25}$& {\em Efficiency } \\[0.5em]
        {\em Level} & {\em Dimensions } & {\em in top  K=4} & (\%)  \\[0.5em]
\hline \\[-0.5em]
        0 & $10 \times 10 \times 24$ & -- & -- \\ 
        2 & $20 \times 20 \times 24$ & 98.8& 87.5 \\     
        4 & $40 \times 40 \times 24$ & 93.8& 96.9 \\
        6 & $80 \times 80 \times 24$ & 84.6& 99.2 \\[0.5em]
        \hline
      \end{tabular}
    }
    \vspace{0.3in}
    \begin{center}
      {\small (c) Ensemble efficiency.}
    \end{center}
  \end{minipage}

  \caption{\small \label{fig:tracking} {\bf (a)},{\bf (b)}: Prediction
    error for VideoPose dataset. Reported errors are the average
    distance from a predicted joint location to the true joint for
    frames that lie in the [25,75] inter-quartile range (IQR) of
    errors. Error bars show standard errors computed with respect to
    clips. All SC models outperform \cite{ferrari08}; the ``torso
    only'' persistence cascade introduces additional error compared to
    a single-frame cascade, but adding arm dependencies in the
    ensemble yields the best performance. {\bf (c)}: Summary of test
    set filtering efficiency and accuracy for the ensemble
    cascade. $PCP_{0.25}$ measures Oracle \% of correctly matched limb
    locations given unfiltered states; see \cite{sapp10cascades} for
    more details.}
\end{figure}

\subsection{The VideoPose Dataset}
\label{sec:patv}

Our dataset consists of 34 video clips of approximately 50 frames
each. The clips were harvested from three popular TV shows: 3 from
{\em Buffy the Vampire Slayer}, 27 from {\em Friends}, and 4 from {\em
  LOST}. Clips were chosen to highlight a variety of situations and
and movements when the camera is largely focused on a single
actor.
% Examples
%were chosen by manual inspection. 
In our experiments, we use the {\em
  Buffy} and half of the {\em Friends} clips as training (17 clips),
and the remaining {\em Friends} and {\em LOST} clips for testing.  In total we test on 901 individual frames. The
{\em Friends} are split so no clips from the same episode are used for
both training and testing.  We further set aside 4 of the {\em
  Friends} test clips to use as a development set. Each frame of each
clip is hand-annotated with locations of joints of a full pose model:
torso, upper/lower arms for both right and left, and top and bottom of
head. For each joint, a binary tag indicating whether or not the joint
is occluded is also included, to be used in future
research.\footnote{The VideoPose dataset is available online at {\tt
    http://vision.grasp.upenn.edu/video/.}}
For simplicity, we use only the torso and upper arm annotations in
this work, as these have the strongest continuity across frames and
strong geometric relationships.

\paragraph{Articulated pose model.} All of the models we evaluated on
this dataset share the same basic structure: a variable for each
limb's $(x,y)$ location and angle rotation (torso, left arm, and right
arm) with edges between torso and arms to model pose geometry. We
refer to this basic model, evaluated independently on each frame, as
the ``Single Frame'' approach. For the VideoPose dataset, we augmented
this model by adding edges between limb states in adjacent frames
(Figure \ref{fig:overview}), forming an intractable, loopy model. \textbf{Features:} Our features in a single frame are the same as in the 
beginning levels of the pictorial structure cascade from \cite{sapp10cascades}: 
unary features are discretized Histogram of Gradient part detectors scores, and 
pairwise terms measure relative displacement in location and angle between 
neighboring parts.  Pairwise features connecting limbs across time also express 
geometric displacement, allowing our model to capture the fact that human limbs 
move smoothly over time.


\paragraph{Coarse-to-Fine Ensemble Cascade.} We learned a
coarse-to-fine structured cascade with six levels for tracking as
follows. The six levels use increasingly finer state spaces for joint 
locations, discretized into bins of resolution $10 \times 10$ up to $80 \times 
80$, with each stage doubling one of the state space dimensions in the 
refinement step.  All levels use an angular discretization of 24 bins.  For the
ensemble cascade, we learned three sub-models simultaneously (Figure
\ref{fig:overview}), with each sub-model accounting for temporal
consistency for a different limb by adding edges connecting the same limb in 
consecutive frames.  
\paragraph{Experimental Comparison. } A summary of results are
presented in Figure \ref{fig:tracking}. We compared the single-frame
cascade and the ensemble cascade to a state-of-the-art single-frame
pose detector (Ferrari et al. \cite{ferrari08}) and to one of the
individual sub-models, modeling torso consistency only (``Torso
Only'').  We evaluated the method from \cite{ferrari08} on only the first half of the test data due to computation time (taking approximately 7 minutes/frame).  We found that the ensemble cascade was the most accurate for
every joint in the model, that all cascades outperformed the
state-of-the-art baseline, and, interestingly, that the single-frame
cascade outperformed the torso-only cascade. We suspect that the poor
performance of the torso-only model may arise because propagating only
torso states through time leads to an over-reliance on the relatively
weak torso signal to determine the location of all the limbs. Sample
qualitative output from the ensemble is presented in Figure
\ref{fig:results-qualitative}.

\out{state-of-the-art boosting method (Table \ref{tab:c2f}, left.) Note
that in practice, we represented an output $y$ as a tuple
$\ang{r,c,s}$, i.e. row, column, and scale, but otherwise followed the
algorithm described in Section \ref{sec:localizer}. For the both the
boosting baseline and our method, we computed Histogram of Oriented
Gradients (HOG) features \cite{hog} at 9 orientations normalized in
square cells 8 pixels wide. These features were extracted from image
patches approximately 110 pixels wide and 130 pixels tall after
rescaling the image to each of the 6 scales. For the coarse-to-fine
filter, we discretized the value of each HOG feature into 10 bins, so
that we used only binary features in the sub-gradient update. For the
boosting method, we extracted training patches with a 3-stage
bootstrapping procedure; parameters for both methods were selected
using early stopping on a development set to avoid overfitting. We
trained both methods three times (using a dense $10 \times 10$ grid
for our localizing filter), holding out {\em Buffy}, {\em Lost}, and
{\em Friends} as test data. To compute the filtering performance of
each method, we computed the number of incorrectly filtered regions if
50\% of regions were passed to the next level of the cascade. While
there was no significant difference in filter error at 75\% efficiency
regardless of the value of $\alpha$ during training, our method
significantly outperformed the boosting baseline.

Next, we computed the effectiveness of the 5 levels of the
coarse-to-fine cascade as the resolution increased (Table 1,
right). As an error metric, we compute the average minimum distance
from the center of region containing the center of the true bounding
box to the center of any unfiltered region. We found that the cascade
was highly effective: with hardly any error (12 pixels, on average),
the coarse-to-fine cascade reduced the $40\times40\times6$ state space
by over 95\% to about only 450 states.

Finally, we evaluated our decomposition ensemble method using {\em
  Buffy} as a test set (Table \ref{tab:ensemble}). The features for
the ensemble were based on face detections using standard
face-detection tools and arm part detectors trained discriminatively
using a pose estimation dataset. We compared the ensemble to each of
the individual methods in the ensemble at multiple efficiencies and
found that the ensemble outperformed our other baselines. Finally, we
also compared the predictive accuracy using only the maximum scoring
state of each model; the ensemble had overall pixel error of $\approx
53$ pixels compared to $\approx 63$ pixels of the next best model or
$\approx 105$ pixels of model with no temporal dependencies.}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 


==> text/nips2010/related.tex <==
\out{Although the detection and tracking of humans (and other objects) is a
well-studied problem in the field of computer vision, the new
dataset we study in this paper poses unique and novel challenges. Our
dataset is comprised of clips from four popular TV shows, which we
refer here to as the
%``{\bf P}ose {\bf A}rticulation and {\bf T}racking in Tele{\bf v}ision'' (PATV)
VideoPose dataset.  Unlike datasets produced in a controlled,
laboratory setting, each clip contains video from a single camera
only, so we cannot take advantage of multiple views or sensors
(e.g.,~\cite{bregler1998tracking}).  Furthermore, the camera and actors in the
scene may move
independently and simultaneously in different directions, or not at
all. Therefore, unlike pedestrian detection and tracking from
surveillance cameras (e.g.,~\cite{andriluka2008people}) we cannot rely on a background
subtraction (\cite{bwu}) nor use motion information or optical flow
techniques (\cite{kratz-tracking}) to determine the location of actors in the
image. In many scenes, actors' movements are often very different from
those of pedestrians. For example, actors on the TV show {\em Friends}
often point, gesticulate, stand up, and sit down, in many cases while
also being tracked by the camera; we are interested in tracking the
limbs of a few individuals with high precision. Parsing pedestrian
scenes, by contrast, involves tracking individuals as they move from
one side of the video frame to another (\cite{pellegrini2009you}), where
occlusion and
crowds pose the most significant challenges.}


\out{combined state of multiple variables: torso position, arm
positions, arm rotation, etc. For a single image, we model the
appearance of a person given these states is modeled well using a
simple tree model (figure \ref{fig:ps_tree}) to model the appearance
and geometry of a primitive human figure. When treated as a generative
model with Gaussian distributions, this model is known as Pictorial
Structures [CITE?]; in contrast, we use the same graph structure to
for the feature generation function of a supervised structured
prediction. Furthermore, as we discretize all continuous features
(such as joint displacement or appearance model scores), we learn a
non-linear function of appearance and geometric features.}

%{\bf Cascaded Inference.}

%{\bf Model ensembles.} Ways of combining tractable models: dual
%decomposition, treerw?




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 


==> text/nips2010/sc.tex <==
\section{Structured Cascades}
\label{sec:sc}

% TODO: add slack penalty into objective/constraint etc.
% TODO: MAKE SURE TO ADD 1/n

%We adopt a notation similar to that used in \cite{weiss10} but
%with several improvements for readability. 
Given an input space $\cX$,
output space $\cY$, and a training set
$\{\ang{x^1,y^1},\dots,\ang{x^n,y^n}\}$ of $n$ 
%independent and identically-distributed ({i.i.d.}) random 
samples from a joint
distribution $D(X,Y)$, the standard supervised learning task is to
learn a hypothesis $h: \cX \mapsto \cY$ that minimizes the expected
loss $\E{D}{ \cL\left(h(x) , y\right)}$ for some non-negative loss
function $\cL : \cY \times \cY \rightarrow \reals^+$. In {\em structured prediction problems},
$Y$ is a $\ell$-vector of variables and $\cY = \cY_1 \times \dots \times
\cY_\ell$, and $\cY_i = \{1, \dots, K\}$. In many settings, the number
of random variables, $\ell$, differs depending on input $X$, but for
simplicity of notation, we assume a fixed $\ell$ here.  The
linear hypothesis class we consider is of the form $h(x) =
\argmax_{y\in\cY} \score{y}$, where the scoring function $\score{y}
\triangleq \theta^\top \bft(x,y)$ is the inner product of a vector of
parameters $\theta$ and a feature function $\bft:
\cX\times\cY\mapsto\reals^d$ mapping $(x,y)$ pairs to a set of $d$
real-valued features. We further assume that $\bft$ decomposes over a
set of cliques $\cC$ over inputs and outputs, so that $\score{y} =
\sum_{c \in \cC} \theta^\top\bft_c(x,y_c)$.  Above, $y_c$ is an
assignment to the subset of $Y$ variables in the clique $c$ and we
will use $\cY_c$ to refer to the set of all assignments to the clique. By
considering different cliques over $X$ and $Y$, $\bft$ can represent
arbitrary interactions between the components of $x$ and $y$. Evaluating 
$h(x)$ is tractable for low-treewidth (hyper)graphs but is NP-hard in general,
and typically, approximate inference is used when features are not low-treewidth.
%computational limiation 
%limit the expressiveness of the features that can be used.

%\subsection*{Structured Cascades}
In our prior work~\cite{weiss10}, we introduced the framework of
Structured Prediction Cascades (SPC) to handle problems with
low-treewidth $T$ but large node state-space $K$, which makes
complexity of $O(K^{T})$ prohibitive.  For example, for a 5-th order
linear chain model for handwriting recognition or part-of-speech
tagging, $K$ is about $50$, and exact inference is on the order
$50^{6} \approx 15$ billion times the length the sequence.  In
tree-structured models we have used for for human pose
estimation~\cite{sapp10cascades}, typical $K$ for each part includes
image location and orientation and is on the order of $250,000$, so
even $K^{2}$ in pairwise potentials is prohibitive. Rather than
learning a single monolithic model, a structured cascade is a
coarse-to-fine sequence of increasingly complex models, where model
complexity scales with Markov order in sequence models or
spatial/angular resolution in pose models, for example.  The goal of
each model is to filter out a large subset of assignments without
eliminating the correct one, so that the next level only has to
consider a much reduced state-space.  The filtering process is
feed-forward, and each stage uses inference to compute max-marginals
which are used to eliminate low-scoring node or clique assignments.
The parameters of each model in the cascade are learned using a loss
function which balances accuracy (not eliminating correct assignment)
and efficiency (eliminating as many other assignments as possible).


%each model receives as input a sparse set of possible clique assignments $y_c$,
%further filters this set, and then passes the reduced set as input to
%the next model. Each clique assignment $y_c$ is represented by its
More precisely, for each clique assignment $y_{c}$,  there is a {\em max marginal} $\mmarg{y_c}$, 
defined as the maximum score of any output $y$ that contains the clique assignment $y_c$:
\begin{equation}
  \label{eq:mmarg_def}
  \mmarg{y_c} \triangleq \max_{y'\in \cY} \;\;\{ \score{y'} : y'_c = y_c\}.
\end{equation}
For simplicitly, we will examine the case where the cliques that we
filter are defined only over single variables: $y_c = y_j$ (although
the model may also contain larger cliques). Clique assignments are
filtered by discarding any $y_j$ for which $\mmarg{y_j} \le t(x)$ for
a threshold $t(x)$. We define $\cY_j$ to be the set of possible states
for the $j$'th variable. The threshold proposed in \cite{weiss10} is a
``max mean-max'' function,
\begin{equation}
  \label{eq:meanmax}
  \thr = \alpha \scoremax + (1-\alpha)\frac{1}{\sum_{j=1}^\ell |\cY_j|}\sum_{j=1}^\ell\sum_{y_j \in \cY_j} \mmarg{y_j}.
\end{equation}
Filtering max marginals in this fashion can be learned because of the
``safe filtering'' property: ensuring that $\scorei{y^i} > \thri$ is
sufficient (although not necessary) to guarantee that no marginal
consistent with the true answer $y^i$ will be filtered. Thus, for
fixed $\alpha$, \cite{weiss10} proposed learning parameters $\theta$
to maximize the margin $\scorei{y^i}-\thri$ and therefore minimize
filtering errors:
\begin{equation}
  \label{eq:std_sc}
  \inf_{\theta, \xi\ge 0} \frac{\lambda}{2}||\theta||^2 + \frac{1}{n}\sum_i \xi^i \suchthat \scorei{y^i} \ge \thri + \ell^i - \xi^i, \quad \forall i = 1, \dots, n
\end{equation}
Above, $\xi^i$ are slack variables for the margin constraints, and $\ell^i$ is the size of the $i$'th example.
% Learning the parameters $\theta$ is done via the following sub-gradient update rule:
% \begin{equation}
%   \label{eq:sc_update}
%   \theta \leftarrow (1-\lambda)\theta +
%   \begin{cases}
%     0 & \textrm{ if } \scorei{y^i} \ge \thri + \ell^i, \\
%     \nabla\scorei{y^i} - \nabla\thri & \textrm{ otherwise},
%   \end{cases}
% \end{equation}
% where $\nabla\scorei{y^i}$ are the features $\bft(x^i,y^i)$ while
% $\nabla\thri$ is a weighted sum of features from each max marginal.
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 


==> text/nips2010/synthetic.tex <==
% TODO: Shrink this section some

\begin{figure}[t]
\begin{center}
  \subfigure[]{
  \input{figs/gridcomb.tex}
  \label{fig:gridcomb}}
  \subfigure[]{
    \includegraphics[width=0.3\textwidth]{figs/improvements.png}
    \label{fig:synth}
  }
\end{center}
\caption{\small \subref{fig:gridcomb} Example decomposition of a $3
  \times 3$ fully connected grid into all six constituent ``comb''
  trees. In general, a $n \times n$ grid yields $2n$ such
  trees. \subref{fig:synth} Improvement over Loopy BP and constituent
  tree-models on the synthetic segmentation task. Error bars show
  standard error.}
\end{figure}

\subsection{Asymptotic Filtering Accuracy}

We first evaluated the filtering accuracy of the max-marginal ensemble
on a synthetic 8-class segmentation task. For this experiment, we
removed variability due to parameter estimation and focused our
analysis on accuracy of inference. We compared our approach to Loopy
Belief Propagation (Loopy BP) \cite{koller}, a state-of-the-art method
for approximate inference, on a $11 \times 11$ two-dimensional grid
MRF.\footnote{\tiny We used the UGM Matlab Toolbox by Mark Schmidt for
  the Loopy BP and Gibbs MCMC sections of this experiment.  Publicly
  available at: {\tt
    http://people.cs.ubc.ca/~schmidtm/Software/UGM.html}} For the
ensemble, we used 22 unique ``comb'' tree structures to approximate the
full grid model (i.e. Figure \ref{fig:gridcomb}). To generate a
synthetic instance, we generated unary potentials $\omega_i(k)$
uniformly on $[0,1]$ and pairwise potentials log-uniformly:
$\omega_{ij}(k,k') = \exp -v$, where $v \sim \mcal{U}[-25,25]$ was
sampled independently for every edge and every pair of classes. (Note
that for the ensemble, we normalized unary and edge potentials by
dividing by the number of times that each potential was included in
any model.) It is well known that inference for such grid MRFs is
extremely difficult \cite{koller}, and we observed that Loopy BP
failed to converge for at least a few variables on most examples we
generated.

\paragraph{Ensemble outperforms Loopy BP.} We evaluted our approach on
100 synthetic grid MRF instances. For each instance, we computed the
accuracy of filtering using marginals from Loopy BP, the ensemble, and
each individual sub-model. We determined error rates by counting the
number of times ``ground truth'' was incorrectly filtered if the top
$K$ states were kept for each variable, where we sampled 1000 ``ground
truth'' examples from the true joint distribution using Gibbs
sampling. To obtain a good estimate of the true marginals, we
restarted the chain for each sample and allowed 1000 iterations of
mixing time.  The result is presented in Figure \ref{fig:synth} for
all possible values of $K$ (filter aggressiveness.) We found that the
ensemble outperformed Loopy BP and the individual sub-models by a
significant margin for all $K$.

\paragraph{Effect of sub-model agreement.} We next investigated the
question of whether or not the ensembles were most accurate on
variables for which the sub-models tended to agree. For each variable
$y_{ij}$ in each instance, we computed the mean pairwise Spearman
correlation between the ranking of the 8 classes induced by the max
marginals of each of the 22 sub-models. We found that complete
agreement between all sub-models never occured (the median correlation
was 0.38). We found that sub-model agreement was significantly
correlated ($p < 10^{-15}$) with the error of the ensemble for all
values of $K$, peaking at $\rho = -0.143$ at $K=5$. Thus, increased
agreement predicted a decrease in error of the ensemble. We then asked
the question: Does the effect of model agreement explain the {\em
  improvement} of the ensemble over Loopy BP?  In fact, the
improvement in error compared to Loopy BP was {\em not} correlated
with sub-model agreement for any $K$ (maximum $\rho = 0.0185$, $p <
0.05$). Thus, sub-model agreement does {\em not} explain the
improvement over Loopy BP, indicating that sub-model disagreement is
not related to the difficulty in inference problems that causes Loopy
BP to underperform relative to the ensembles (e.g., due to convergence
failure.)

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 

